Enzyme economy and metabolic control

The metabolic state of a cell, comprising fluxes, metabolite concentrations and enzyme levels, is shaped by a compromise between metabolic benefit and enzyme cost. This hypothesis and its consequences can be studied by computational models and using a theory of metabolic value. In optimal metabolic states, any increase of an enzyme level must improve the metabolic performance to justify its own cost, so each active enzyme must contribute to the cell's benefit by producing valuable products. This principle of value production leads to variation rules that relate metabolic fluxes and reaction elasticities to enzyme costs. Metabolic value theory provides a language to describe this. It postulates a balance of local values, which I derive here from concepts of metabolic control theory. Economic state variables, called economic potentials and loads, describe how metabolites, reactions, and enzymes contribute to metabolic performance. Economic potentials describe the indirect value of metabolite production, while economic loads describe the indirect value of metabolite concentrations. These economic variables, and others, are linked by local balance equations. These laws for optimal metabolic states define conditions for metabolic fluxes that hold for a wide range of rate laws. To produce metabolic value, fluxes run from lower to higher economic potentials, must be free of futile cycles, and satisfy a principle of minimal weighted fluxes. Given an economical flux mode, one can systematically construct kinetic models in which all enzymes have positive effects on metabolic performance.

==> files/mySIsettings.tex <==
\renewcommand{\thesection} {S\arabic{section}}
\renewcommand{\thefigure}  {S\arabic{figure}}
\renewcommand{\thetable}   {S\arabic{table}}
\renewcommand{\theequation}{S\arabic{equation}}


==> files/mysettings_arxiv.tex <==
% ------------------------------------------
% this is like in ``mysettings.tex''

\usepackage{setspace} 
\onehalfspacing
\renewcommand{\familydefault}{\sfdefault}

\usepackage{wrapfig}
\usepackage{enumitem}
\usepackage{xr}
\usepackage{color}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{colortbl}
\usepackage{url}

\definecolor{grey}{rgb}{0.9, 0.9, 0.9}

\newcommand{\remember}[1]{\marginpar{\tiny #1}}
\newcommand{\myparagraph}[1]{\vspace{-3mm}\paragraph{#1}}

\newenvironment{myitemize}{\vspace{-4pt}\begin{itemize}[leftmargin=5mm]\itemsep -2pt}{\end{itemize}}

\newtheorem{mydefinition}{Definition}
\newtheorem{mytheorem}{Theorem}
\newtheorem{mycorollary}{Corollary}

\setlength{\parindent}     {0cm}
\setlength{\parskip}       {0.2cm}
\setlength{\textwidth}     {16.5cm}
\setlength{\textheight}    {25cm}

\newcommand{\mybox}[1]{\fbox{\parbox{16.5cm}{\begin{center}\parbox{15.5cm}{#1}\end{center}}}}

% ------------------------------------------
% this is different from mysettings.tex

\newcommand{\coout}[1]{}
\newcommand{\co}   [1]{}
\newcommand{\todo} [1]{}
\newcommand{\wolf} [1]{}

\setlength{\headsep}       {-2cm}
\setlength{\oddsidemargin} {-0.3cm}
\setlength{\evensidemargin}{-0.3cm}

% \setlength{\textwidth}     {15.5cm}
% \setlength{\textheight}    {22cm}
% \setlength{\oddsidemargin} {0.3cm}
% \setlength{\evensidemargin}{0.3cm}

\pdfoutput=1
\usepackage{hyperref}
\hypersetup{colorlinks = true, allcolors = {blue}}



==> files/mysettings_arxiv_nohyperref.tex <==
% ------------------------------------------
% this is like in ``mysettings.tex''

\usepackage{setspace} 
\onehalfspacing
\renewcommand{\familydefault}{\sfdefault}

\usepackage{wrapfig}
\usepackage{enumitem}
\usepackage{xr}
\usepackage{color}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{colortbl}
\usepackage{url}

\definecolor{grey}{rgb}{0.9, 0.9, 0.9}

\newcommand{\remember}[1]{\marginpar{\tiny #1}}
\newcommand{\myparagraph}[1]{\vspace{-3mm}\paragraph{#1}}

\newenvironment{myitemize}{\vspace{-4pt}\begin{itemize}[leftmargin=5mm]\itemsep -2pt}{\end{itemize}}

\newtheorem{mydefinition}{Definition}
\newtheorem{mytheorem}{Theorem}
\newtheorem{mycorollary}{Corollary}

\setlength{\parindent}     {0cm}
\setlength{\parskip}       {0.2cm}
\setlength{\textwidth}     {16.5cm}
\setlength{\textheight}    {25cm}

\newcommand{\mybox}[1]{\fbox{\parbox{16.5cm}{\begin{center}\parbox{15.5cm}{#1}\end{center}}}}

% ------------------------------------------
% this is different from mysettings.tex

\newcommand{\coout}[1]{}
\newcommand{\co}   [1]{}
\newcommand{\todo} [1]{}
\newcommand{\wolf} [1]{}

\setlength{\headsep}       {-2cm}
\setlength{\oddsidemargin} {-0.3cm}
\setlength{\evensidemargin}{-0.3cm}

% \setlength{\textwidth}     {15.5cm}
% \setlength{\textheight}    {22cm}
% \setlength{\oddsidemargin} {0.3cm}
% \setlength{\evensidemargin}{0.3cm}


==> files/symbols_trivial_names.tex <==
\renewcommand{\cintv}{\cv}
\renewcommand{\cextv}{\sv}
\renewcommand{\Next}{\Smat}
\renewcommand{\Nint}{\Nmat}
\renewcommand{\NR}{\Nmat_{\rm R}}


==> sec_definitions_cba_kinetic.tex <==
\subsection{Metabolic models}

\coout{The cost-benefit balance entails various constraints on the
  steady state of kinetic models, in particular, on their stationary
  {\flow}s. The following theorems state that: (i) the
  cost-benefit balance equation (\ref{eq:fitnessbalanceeq}) is
  equivalent to the {\gain} conditions (\ref{eq:fitnessbalance2}) and
  (\ref{eq:fitnessbalance3}); (ii) the economic balance equation
  (\ref{eq:reactionbalanceeq}) is equivalent to the absence of futile
  modes; (iii) the absence of futile submodes is equivalent to weighted
  flux minimisation.}

\myparagraph{\ \\Kinetic models} A kinetic metabolic model is defined by its
stoichiometric matrix and by reversible rate laws of the form
\begin{eqnarray}
  \label{eq.kineticlaw} v_{l} = \rate_{l}(\uv,\cv,\cextv) = u_{l} \,
  \ratelaw_{l}(\cv,\cextv).  
\end{eqnarray} 
We assume that each reaction is catalysed by a specific enzyme, whose
activity $u_{l}$ (concentration of the active form) appears as a
prefactor\footnote{The symbols $u_{l}$ and $\cextj$ (instead of
  symbols $e_{l}$ and $c^{\rm ext}$ used in other articel) emphasise
  that the important distinction is not between enzymes and external
  metabolites, but between controllable and non-controllable model
  parameters. The vectors $\uv$ and $\xv$ can also comprise other
  quantities: for instance, the growth rate could be another control
  parameter $u_l$ and the temperature could be another external
  parameter $\cext_j$.}.  The kinetic rate laws -- e.g.~mass-action or
Michaelis-Menten kinetics -- must be reversible and thermodynamically
correct (see \cite{liuk:10}), and the kinetic constants must satisfy the
Wegscheider conditions and Haldane relations \cite{liuk:10}.
Allosteric regulation by metabolites is described by the rate
laws. Changes by covalent enzyme modifications (e.g.~a
phosphorylation) that change enzyme activity) are incorporated into
the variables $u_{l}$.  We consider only models with a stable steady
state. The steady-state concentrations
$\cint_{i}=\csteady_{i}(\uv,\cextv)$ and fluxes
$v_{l}=\vsteady_{l}(\uv,\cextv) =
\rate_{l}(\cvsteady(\uv,\cextv),\cextv)$ are functions of the model
parameters, i.e.~enzyme levels $u_{l}$ and external concentrations
$\cextj$.  For a list of variables in kinetic models, see Table
\ref{tab:listofsymbols}. Economic state variables, used to describe
optimal states, are listed in Table \ref{tab:listofsymbols2}.

\myparagraph{Stationary {\flow}s and conserved moieties} The
stoichiometric matrix $\Nint$ for internal metabolites contains information about  the
stationary fluxes and conserved moieties.  It defines a
right-kernel matrix $\Kint$ (satisfying $\Nint\,\Kint=0$) and a link
matrix $\Lmat$. The columns of the right-kernel matrix ${\Kint}$
describe stationary fluxes.  If $\Nint$ does not have full row rank,
we can choose a set of independent internal metabolites and split the
stoichiometric matrix into $\Nint = \Lmat\, \NR$ where the rows of
$\NR$ refer to independent metabolites.  \coout{zweites beispiel
  zeigen?: branch point mit conc {\gain} -1?  enz cost 2 1 1;}
\coout{was ist mit inaktiven reakt?  koennte hv definiert sein? ist
  ein problem: am rand des S-polytops sind die ableitungen nur
  einseitig definiert!  und es fehlt noch ein term um ungleichung zu
  ermoeglichen} Moiety conservation (e.g.~the fact that the sum of
concentrations [ATP] + [ADP] + [AMP] is a constant) can make some metabolite concentrations
linearly dependent.  The rows of the left-kernel matrix $\Gmat$
describe conserved moieties.  In models with moiety conservation,
$\Nint$ can be split into a product $\Lmat\,\NR$, where the rows of
$\NR$ (reduced stoichiometric matrix) belong to independent
metabolites and are linearly independent. $\Lmat$ is called link
matrix. In models without moiety conservation, $\Lmat$ is an identity
matrix, $\NR=\Nint$, and $\Gmat$ is empty.

\myparagraph{Elasticities and control coefficients} We define the
unscaled elasticities $ \Eunvlci =
\partial v_l / \partial \cint_i$
for internal metabolites and the unscaled enzyme elasticities
$\Eunul = v_{l}/u_{l}$.  Scaled elasticities for internal metabolites
are defined by
$\Escvlci = \frac{\partial \ln |v_l|}{\partial \ln \cint_i} =
\frac{\cint_i}{v_l} \frac{\partial v_l}{\partial \cint_i}$.
In these definitions, metabolite and enzyme levels are independent
parameters, i.e.~the reaction is considered in isolation.  The
response and control coefficients, in contrast, are derivatives of the
global steady-state concentrations $\csteady_i$ and fluxes
$\vsteady_l$.

\myparagraph{Flux cost minimisation} Classical FBA is  a linear
optimality problem of the form
$\vv = \argmax_{\vv'}\; \bvtot \cdot\,\vv'$ with the constraints
$\Nint\;\vv'=0$ and $\vv^{\rm min} \le \vv' \le \vv^{\rm max}$.  A
flux cost minimisation (FCM) problem is an optimisation problem of the
form
\begin{eqnarray}
\label{sec:generalpmfoptimality2}
\vv = \argmin_{\vv'}  \acostv(\vv') \quad \mbox{subject to} 
 \quad \bvtot\cdot \vv = b, \quad \quad \Nint\;\vv=0, 
 \quad \mbox{and} \quad \vv^{\rm min} \le \vv \le \vv^{\rm max},
\end{eqnarray}
with a possibly non-linear flux cost function $\acostv(\vv)$.  The
flux cost function $\acostv(\vv)$ must have positive scaled
derivatives $(\partial \acostv(\vv)/ \partial v_l)\,v_l$ whenever
$v_l\ne 0$, implying that there is a single minimum, $v_{l}=0$.  FCM
problems with cost functions
$\acostv(v_{l}) = \sum_{l} \acostvlweight \,|v_{l}|$ and positive flux
cost weights $\acostvlweight$ are called \emph{weighted flux
  minimisation problems}.  An FCM problem is called
\emph{flux-enforcing} if its flux bounds exclude the thermodynamic
equilibrium state (i.e.~if $v^{\rm min}_{l} > 0$ or
$v^{\rm max}_{l} < 0$).

\subsection{Optimal states and economic variables}

In kinetic metabolic models, optimal states are defined by optiming a
fitness function with respect to control variables (typically, enzyme
levels).

\begin{mydefinition} 
  \textbf{(Conditions for enzyme-optimal states)} A kinetic model with
  a fitness function Eq.~(\ref{eq:fitness}) is called
  \emph{enzyme-balanced} if it is in a stable steady state and if all
  active enzymes satisfy a cost-benefit balance equation
  (\ref{eq:fitnessbalanceeq}). If, additionally,  all reactions are enzyme-catalysed  and
  active, the model is  called
  \emph{completely enzyme-balanced}. 
\end{mydefinition}

\begin{mydefinition} 
  \textbf{(Flux conditions in enzyme-optimal models)} States of
  economic enzyme usage must satisfy a number of (decreasingly strict) conditions: 

\begin{enumerate}[leftmargin=5mm] 
\item \textbf{Enzyme-optimal} A {\flow} $\vv$ is called
  \emph{enzyme-optimal} if it can be realised by an enzyme-optimal
  kinetic model. Such a model must satisfy four conditions: (i) the
  rate laws are reversible with kinetic constants satisfying Wegscheider
  conditions and Haldane relationships \cite{liuk:10}; (ii) the model
  has a steady state with {\flow} $\vv$; (iii) this steady state is
  stable, i.e.~all eigenvalues of the Jacobian matrix have negative
  real parts; (iv) the state is economically stable, that is, the
  enzyme levels represent a local maximum of the fitness
  function. This means (if inactive reactions are ignored): the
  fitness gradient $\fu$ must vanish and the fitness curvature matrix
  $\Fuu$ must be negative definite.

\item \textbf{Enzyme-balanced} A {\flow} is called \emph{enzyme-balanced}
  if it can be realised by  a kinetic model that satisfies conditions (i) and (ii)
  as well as the cost-benefit balance (\ref{eq:fitnessbalanceeq}). The
  steady state may be unstable, and the enzyme levels must represent
  an extremum of the fitness function (i.e.~$\fu=0$), but not
  necessarily a maximum (e.g.~the fitness curvature matrix $\Fuu$ can have positive
  eigenvalues). Enzyme-balanced flux modes satisfy the conditions
(\ref{eq:fitnessbalance2}) and
(\ref{eq:fitnessbalance3}) and the economic balance equations
  (\ref{eq:reactionbalanceeq}) and
  (\ref{eq:metabolitebalanceequation}).

\item \textbf{Enzyme-beneficial} A {\flow} is called
  \emph{enzyme-beneficial} if it stems from a kinetic model in which
  each enzyme has a positive influence (i.e.~a positive control
  coefficient) on the {\metabolicobjective}.

\item \textbf{Economical} A {\flow} is called \emph{economical} if this
  {\flow}, reduced to its active region, satisfies the
  {\summationcondition} (\ref{eq:fitnessbalance2}) with a
  positive cost vector $\hudot$. According to Theorems
  \ref{th:theoremfutile} and \ref{th:theoremPMF1}, this is equivalent
  to the following (equivalent) conditions: (i) $\vv$ satisfies the
  flux benefit balance (\ref{eq:reactionbalanceeq}) for some choice of
  the economic potentials $\winti$ and positive {{\enzymecost}}s
  $\hudotl$; (ii) $\vv$ is free of {\futile} submodes; (iii) $\vv$ is
  the solution of a (non-flux-enforcing) flux cost
  minimisation problem.
\end{enumerate}
\end{mydefinition}

\begin{mydefinition} \textbf{(Economical metabolic {\flow})} Consider a
  metabolic network formed by enzymatic reactions and with flux
  {\gain} vector $\bvtot$. A {\flow} $\vv$ in this network is called
  \emph{economical} if after removing all active reactions from the
  network, this {\flow} can satisfy the variation condition
  (\ref{eq:fitnessbalance2}) with a positive vector $\hudot$. Models
  with non-enzymatic reactions are discussed in SI
  \ref{sec:nonenzymatic}.
\end{mydefinition} 

\begin{mydefinition} \textbf{(Flux variations and {\nonbeneficial}
    submodes)} Let $\vv$ be the {\flow} in question and let $\modevector$
  be a conformal test mode of $\vv$ (i.e.~a non-vanishing {\flow} within
  the active region of $\vv$ and conformal with $vv$, i.e.~if all
  fluxes on the support of $\modevector$ have the same directions as
  in $\vv$). The vector $\modevector$ can be used as a flux variation
  of $vv$.  Let $\bvtot$ be a vector of {\fluxgain}s.  If
  $\modevector$ is {\futile} , their shared sign pattern is called a
  \emph{{\futile} submode in $\vv$} with respect to
  $\bvtot$. Likewise, if $\modevector$ is {\wasteful}, their shared
  sign pattern is called a \emph{{\wasteful} submode}. Flux modes that
  are {\futile} or {\wasteful} are also called \emph{\nonbeneficial}.
\end{mydefinition} 

\begin{mydefinition} \textbf{(Economic potential)} Consider an
  enzyme-balanced kinetic model with a {\metabolicobjective} function
  $\gplus(\uv,\cextv,\virtphiindv)$. The virtual exchange flux
  vector $\virtphiindv$, for independent metabolites, defines
  a virtual exchange flux vector $\virtphiv = \Lmat\,\virtphiindv$ for
  all internal metabolites. The economic potentials are defined
  as {\gain}s $\wextj =\bpsij$ (for external metabolites),
  $\winti = \frac{\partial \gplus}{\partial \virtphiindi}$ (for
  independent internal metabolites), and $\winti = 0$ (for dependent
  internal metabolites).
\end{mydefinition}

\emph{Remark.}  In models with moiety conservation, there is
arbitrariness in the choice of the independent metabolites, which
leads to arbitrariness (or rather, gauge freedom) in the definition of
economic potentials.  Economic potentials with a different gauging can
be obtained by replacing
$\wint \rightarrow \wint + \Gmat\trans\,\wvsymbol_{\rm cm}$, where
$\Gmat$ is a left-kernel matrix of $\Nint$, and the vector
$\wvsymbol_{\rm cm}$, containing the economic potentials of the
conserved moieties themselves, can be freely chosen.

\begin{mydefinition} \textbf{(Economic load)} In an enzyme-balanced
  kinetic model, we apply a small virtual variation of an internal
  metabolite concentration (replacing
  $\cint_i \rightarrow \cint_i + c^{\rm pert}_{i}$) and then let the
  system evolve to steady state. If metabolite $i$ is not involved in
  moiety conservation, the system will return to its previous steady
  state.  Instead, if it is involved in moiety conservation, the
  system will end up in a new state, and the {\metabolicobjective} is a function
  $\gplus(\uv,\cextv,c^{\rm pert}_{i})$ of the concentration variation
  $c^{\rm pert}_{i}$.  The economic loads are now defined as
  $\loadj = \frac{\partial \gplus}{\partial \cextj}$ (for external
  metabolites) and as
  $\loadint = \frac{\partial \gplus}{\partial c^{\rm pert}_{i}} -
  \frac{\partial \bbenefit}{\partial \cv}$ (for internal metabolites)
  with the concentration {\price}s
  $\hci = \partial \metcost/\partial \cint_i$.  Loads associated with  other
  (external or internal) model variables can be defined similarly as for
  (external or internal) metabolite concentrations.
\end{mydefinition}

\subsection{Conditions for optimal states} \label{sec:SIpropositions}

Enzyme-balanced states satisfy a number of mathematical conditions
which follow from the necessary optimality conditions.

\begin{proposition}
  \label{th:theorem1} \textbf{({\Summationconnectivitycondition})} If
  a kinetic model is  enzyme-balanced and all reactions are
  enzyme-catalysed and active, the cost-benefit balance
  Eq.~(\ref{eq:fitnessbalanceeq}) is equivalent to the variation
  conditions (Proof in SI
  \ref{sec:proofequivalenceoptimalitytheorems}):
 \begin{eqnarray}
\label{eq:fitnessbalance2}
{\Kint}\trans \bvtot &=&  \quad\;\;  {\Kint}\trans \diag(\hudot)\, \vv\inv\\
\label{eq:fitnessbalance3}
 \Lmat\trans\,\hc &=&   \Lmat\trans {\Eunint}\trans\, \diag(\hudot)\,\vv\inv,
 \end{eqnarray} 
 with the kernel matrix $\Kmat$ and the link matrix $\Lmat$. These
 conditions can also be written in the form 
 \begin{eqnarray}
(\bvtot - \acostv)  \cdot \deltapar \vv &=&  0 \nonumber\\
(\hc - {\Eunint}\trans\, \acostv)  \cdot \deltapar \cv &=& 0, \nonumber
 \end{eqnarray}
 which must hold for any proper (i.e.~stationary) flux variation
 $\deltapar \vv$ and proper (i.e.~moiety-conserving) concentration
 variation $\deltapar \cv$.  The \summationconnectivitycondition refer to active,
 enzyme-catalysed reactions only: before applying them, all inactive
 reactions (where $v_{l}=0$) must be removed from the model. There are
 also \summationconnectivitycondition for models with non-enzymatic reactions
 (see SI \ref{sec:nonenzymatic}).
\end{proposition}

\begin{proposition}
 \label{th:theoremtestmode}
 \textbf{(Flux variation criterion)} If $\vv$ is an economical
 metabolic {\flow} and $\modevector$ is a test mode of $\vv$,
 the following holds: if
 $\modevector$ is beneficial ($\bvtot \cdot \modevector>0$), then
 $\vv$ and $\modevector$ share some  reaction with the same flux
 directions; if $\modevector$ is wasteful
 ($\bvtot\cdot \modevector<0$), they share reaction with the opposite flux
 directions; and if $\modevector$ is {\futile}
 ($\bvtot\cdot \modevector=0$), they share some reactions of both sorts.
\end{proposition}

\emph{Remark:} The proof (see SI \ref{sec:prooftheoremtestmode} and
\ref{sec:prooftheoremfutile}) starts from the {\summationcondition}
(\ref{eq:fitnessbalance2}). Without loss of generality, $\vv$ is
assumed to cover the entire network. If $\vv$ is economical, there
must be some positive vector $\hudot$ that satisfies the condition
$\modevector \cdot \bvtot = \modevector\trans \diag(\hudot)\, \vv\inv$
for any flux variation $\modevector$. If a flux variation
$\modevector$ is {\futile}, the left-hand side will vanish, and so
the right side must vanish as well. In order for positive and negative
summands to cancel out, $\modevector$ and $\vv\inv$ (or equivalently
$\vv$) must contain at least one reaction with equal signs and another
reaction with opposite signs. Analogous arguments hold for beneficial
test modes (positive right-hand side: at least one reaction with
positive signs) and {\wasteful} flux variations (negative right-hand
side: at least one reaction with negative signs). Similar to  
Beard's thermodynamic  feasiblity criteria based on oriented matroids
\cite{bbcq:04}, we can state equivalently that the sign patterns of an
economical {\flow} $\vv$ and arbitrary {\nonbeneficial} {\flow}s $\kv$ must satisfy
$|\langle \sign(\kv), \sign(\vv) \rangle| < |\langle \sign(\kv),
\sign(\kv) \rangle|$.

\begin{proposition}
 \label{th:theoremfutile}
 \textbf{(Criteria for economical metabolic {\flow}s)} For a {\flow}
 $\vv$ (containing only enzyme-catalysed reactions), the following
 statements are equivalent: (i) $\vv$ is economical (i.e.~it satisfies
 the {\summationcondition} with positive {{\enzymecost}}s); (ii) $\vv$
 satisfies the flux benefit balance (\ref{eq:reactionbalanceeq}) with some
 choice of internal economic potentials $\winti$ and positive enzyme
 costs $\hudotl$; (iii) $\vv$ does not contain any {\nonbeneficial} submodes (Proof SI
 \ref{sec:prooftheoremfutile} and \ref{sec:proofecoblanacesummation}).
\end{proposition}
\emph{Remarks} (i) Economical metabolic {\flow}s must be beneficial.
This is easy to see: each {\flow} can be used as its own test mode; thus,
if a {\flow} $\vv$ is not beneficial ($\bvtot\cdot \vv \le 0$), it
contains a {\nonbeneficial} submode, and so it cannot be economical.  (ii)
There is another equivalent criterion for economical metabolic {\flow}s:
$\vv$ and $\bvtot$ can be realised by a kinetic model in an
enzyme-balanced state. The proof direction ``economical $\rightarrow$
realisable'' follows from the algorithm for model construction
(in section \ref{sec:reconstruction}).

\begin{proposition}
\label{th:theoremPMF1}
\textbf{(Flux cost minimisation and economic {\flow}s, ``Nocturno
  principle'')} (a) If a {\flow} $\vv$ is the solution of a
non-flux-enforcing FCM problem with {\metabolicobjective} function
$\fluxbene(\vv) = \bvtot\cdot \vv$, it is economical with
respect to $\bvtot$.  Also the opposite holds: (b) If a {\flow} is
pervasive and economical for $\bvtot$, it would solve some weighted FCM
problem with benefit function $\fluxbene(\vv) = \bvtot\cdot \vv$ and
flux {\price}s $\acostvl = \frac{\hul\, u_{l}}{v_{l}}$.  Moreover, it will
also solve \emph{any other} FCM problems with the same benefit
function and the same cost derivatives
$\partial \acost/\partial v_{l}$ in the optimal state (proof SI
\ref{sec:proofFBAmsf}).
\end{proposition}

\coout{Remark: ?? The Lagrange multipliers (related to the
  stationarity constraint in an FCM problem) can be seen as economic
  potentials.  cite REF}

\begin{proposition}
 \label{th:theoremloadForce}
 \textbf{(Load-potential balance)} Consider a kinetic model with a 
 given metabolic objective.  The load of a metabolite is linked to  the {\fluxvalue}s
 of the surrounding reactions (i.e.~reactions directly influenced by
 it) by the \loadbalance
\begin{eqnarray}
  \label{eq:loadfluxvalueequationApp}
 \loadi = \sum_{l}  \gvtotl\,\Eunvlci = \sum_{l}  [\Deltar \wtotl + \bvdirl]\,\Eunvlci.
\end{eqnarray}
The reactions can involve  non-enzymatic or dilution
reactions. Analogous balance equations hold for the load of external metabolites
and for the load  associated with other  variables $q_r$ that directly
affect the reaction rates (e.g.~temperature).
\end{proposition}

\begin{proposition}
 \label{th:theorembalance}
 \textbf{(Economic balance equations)} In  kinetic models in enzyme-balanced states,
 all active enzymatic reactions satisfy the
 flux benefit balance (Proof in SI \ref{sec:proofeconomicalternative})
 \begin{eqnarray*}
 [\Deltar \wtotl + \bvdirl]\,  v_{l} = \hul \,u_{l} 
 \end{eqnarray*}
 between economic potentials $\wtoti$, positive enzyme
 {\price}s $\hul$, and enzyme levels $u_{l}$.  Furthermore, all internal
 metabolites  satisfy the  metabolite balance
 (Proof SI
 \ref{sec:proofinvestmentbalance})
 \begin{eqnarray*}
 \loadi\, \cint_{i} &=& \sum_{l}\,\hudotl \, \Escvlci
 \end{eqnarray*}
 between economic loads $\loadi$ and scaled reaction elasticities
 $\Escvlci$. Similar balance equations hold for external metabolites and for
 any quantities that directly affect the reaction rates.
\end{proposition}
\emph{Remark} (1) In models with non-enzymatic reactions, the 
metabolite  balance reads
\begin{eqnarray}
\label{eq:qloadinternal3}
\loadi\,\cint_{i}&=& \sum_{l \in {\rm enz}} \hudotl \, \Escvlci
+ \sum_{l \in {\rm non}} \fudotl \,\Escvlci
\end{eqnarray}
where ``enz'' and ``non'' denote enzymatic and non-enzymatic
reactions.  The economic stress
$\fudotl=[\Deltar \wtotl + \bvdirl]\,v_{l}$ in a non-enzymatic
reaction can be seen as the benefit of a virtual enzyme with a level
$u_{l}=1$ (proof in SI \ref{sec:proofinvestmentbalancenonenzymatic}).
(2) The balance equations can also be written in terms of {\price}s
and {\myvalue}s (instead of costs and benefits):
 \begin{eqnarray*}
 \Deltar \wtotl + \bvdirl &=& \hul \,\frac{u_{l}}{v_{l}} = \hvl \\
 \loadi\,  &=& \sum_{l} \,\hvl \, \Eunvlci.
 \end{eqnarray*}



==> sec_proofs_cba_kinetic.tex <==
\section{Metabolic control coefficients}

\subsection{Control matrix $\Ccmat_\gamma$}
\label{sec:ProofsimplegammaControl}

The control matrix $\Cmat^{\rm S}_{\gamma}$ describes the long-term- effects of metabolic perturbations. It can be derived as follows.
After a perturbation $\delta \virtgammav$, moiety conservation implies that
$\Gmat\,\delta \cv = \Gmat\,\delta \virtgammav$. Furthermore, there are
stationarity conditions $0=\NR\,\rate(\cv^{\rm init})$ before the
perturbation and $0=\NR\,\rate(\cv^{\rm init} + \delta \cv)$ in the
final state. By taking the difference and using a linear expansion for
$\rate$, we obtain $0 = \NR \,\Eunint\,\delta \cv$. Together, our two
conditions yield
\begin{eqnarray}
{\Gmat \choose \NR\,\Eunint}\,\delta \cv = {\Gmat \choose 0}  \delta \virtgammav
\quad \Rightarrow \quad
\delta \cv = \underbrace{{\Gmat \choose \NR\,\Eunint}\inv \,{\Gmat \choose 0}}_{\Cmat^{\rm S}_{\gamma}}  \delta \virtgammav.
\end{eqnarray}
 The control matrix  $\Cmat^{\rm S}_{\gamma}$ can
 be rewritten as
\begin{eqnarray}
\label{eq:simplegammaControl}
\Cmat^{\rm S}_{\gamma} = \Imat -
\Lmat\,(\NR\,\Eunint\,\Lmat)\inv\,\NR\,\Eunint = \Imat + \Cmat^{\rm S}\,\Eunint.
\end{eqnarray}
To prove this, we
note that
 \begin{eqnarray} 
\Imat - \Lmat\,(\NR\,\Eunint\,\Lmat)\inv\,\NR\,\Eunint &=& {\Gmat \choose
       \NR\,\Eunint}\inv \,{\Imat \choose 0} \,\Gmat\nonumber
     \\ {\Gmat \choose \NR\,\Eunint} [ \Imat -
       \Lmat\,(\NR\,\Eunint\,\Lmat)\inv\,\NR\,\Eunint] &=& {\Gmat
       \choose 0}.
\end{eqnarray}
Since $\Gmat\,\Lmat=0$, this holds true.


\subsection{Theorems of metabolic control theory for kinetic models with dilution}
\label{sec:SIproofMCAwithDilution}

 In a growing cell, all compounds are constantly diluted.  To apply
 metabolic economics to models of growing cells, we need metabolic
 control coefficients for such models. Dilution  resembles a
 non-enzymatic degradation and can  be described by dilution
 fluxes $v^{\rm dil}_{i} = \lambda \,c_{i}$ proportional to  metabolite
 concentrations $c_{i}$ and the growth rate $\lambda$.  Given the
 dilution fluxes in a steady state, the concentrations must satisfy
 $\cv=\frac{1}{\lambda}\,\Nint\,\vv$;
 the Jacobian matrix contains an extra term
 $-\lambda\,\Imat$, and the control matrices read
\begin{eqnarray}
\label{eq:controlWithDilution}
\Ccmat &=& - \Lmat\,(\Mmat-\lambda\,\Imat)\inv\,\NR \nonumber \\
\Cvmat &=& \Imat + \Eunint\,\Ccmat,
\end{eqnarray}
where $\Mmat=\NR\,\Eunint\,\Lmat$ is the usual Jacobian for
independent metabolites and the Jacobian $\Mmat_{\lambda} = \Mmat -
\lambda\,\Imat$ includes the effects of metabolite dilution.  The
control matrices with respect to virtual exchange fluxes (for
independent metabolites) are given by $\Ccmat_{\virtphiind} = -
\Lmat\,{\Mmat_{\lambda}}\inv$ and $\Cvmat_{\virtphiind} = \Eunint\,
\Ccmat_{\virtphiind}$ (see SI
\ref{sec:proofenzymebenefitmetabolitevalue}).  The summation and
connectivity theorems  read (proof see below)
\begin{eqnarray}
 \label{eq:theoremsdilution}
 \Ccmat\, {\Kint} &=& 0 \nonumber \\
 \Cvmat\, {\Kint} &=& {\Kint} \nonumber\\
 \Ccmat\, \Eunint\, \Lmat &=& - \Lmat\,(\Imat + \lambda\,{\Mmat_{\lambda}}\inv)
 \nonumber \\
 \Cvmat\, \Eunint\, \Lmat &=& - \lambda\,\Eunint\,
\Lmat\,{\Mmat_{\lambda}}\inv.
\end{eqnarray}
These theorems cover  enzymatic and non-enzymatic reactions. With
the unscaled parameter elasticity matrix $\Eun_{\rm P}$, the response
matrices read
\begin{eqnarray}
 \Rcmat=\frac{\partial \cvsteady}{\partial \pv} =\Ccmat\, \Eun_{\rm P} \quad
\mbox{and} \quad
 \Rvmat=\frac{\partial \vvsteady}{\partial \pv} =\Cvmat\, \Eun_{\rm P}.
\end{eqnarray}
 If the growth rate $\lambda$ is treated as a parameter,
its  response coefficients form the  vectors
\begin{eqnarray}
 \Rcmat_{\lambda} = \frac{\partial \cvsteady}{\partial \lambda} = - \Ccmat_{\virtphi}\, \cv, \qquad
 \Rvmat_{\lambda} = \frac{\partial \vvsteady}{\partial \lambda} = - \Cvmat_{\virtphi}\, \cv,
\end{eqnarray}
where $\Ccmat_{\virtphi} = \Ccmat_{\virtphiind} \Lmatplus$ and
$\Cvmat_{\virtphi} = \Cvmat_{\virtphiind} \Lmatplus$. The matrix
$\Lmatplus$, the projector from internal metabolites to
independent internal metabolites,  is obtained from an identity
matrix $\Imat$ (with a size given by the number of internal metabolites)
by selecting the rows that correspond to \emph{independent} internal
metabolites.

\paragraph{Proof: Summation and connectivity theorems with dilution}
\label{sec:proofconnectdilution}

The summation and connectivity theorems (\ref{eq:theoremsdilution}) can
be derived as follows. To derive the summation theorems,
 we multiply the control matrices
(\ref{eq:controlWithDilution}) by $\Kmat$, note that
$\NR\,\Kmat=0$, and obtain
\begin{eqnarray}
  \Ccmat\,\Kmat &=& 0 \nonumber  \\
 \Cvmat\,\Kmat &=& \Kmat.
\end{eqnarray}
To derive the connectivity theorems, we first compute
\begin{eqnarray}
 \label{eq:prooftheoremsdilution}
 \Ccmat\, \Eunint\, \Lmat - \lambda\,\Ccmat_{\virtphiind}&=&
 -\Lmat\,(\Mmat-\lambda \Imat)\inv\Nint\, \Eunint\, \Lmat 
+ \lambda\,\Lmat \,(\Mmat-\lambda \Imat)\inv \nonumber \\
&=&
 -\Lmat\,(\Mmat-\lambda \Imat)\inv\Mmat
+ \Lmat \,(\Mmat-\lambda \Imat)\inv \lambda\,\Imat \nonumber \\
&=&
 - \Lmat\, (\Mmat-\lambda \Imat)\inv(\Mmat - \lambda\,\Imat) = -\Lmat.
\end{eqnarray}
This yields  (with $\Mmat_{\lambda} = \Mmat-\lambda\,\Imat$)
\begin{eqnarray}
 \label{eq:prooftheoremsdilution2}
 \Ccmat\, \Eunint\, \Lmat &=& -\Lmat + \lambda\,\Ccmat_{\virtphiind}
= - \Lmat - \lambda\,\Lmat\,(\Mmat-\lambda\,\Imat)\inv 
= - \Lmat \,(\Imat + \lambda\, {\Mmat_{\lambda}}\inv) \\
 \Cvmat\, \Eunint\, \Lmat &=& (\Imat + \Eunint\,\Ccmat)\, \Eunint\, \Lmat
= \Eunint\, \Lmat + \Eunint\,\Ccmat\, \Eunint\, \Lmat 
= \Eunint\, \Lmat - \Eunint\,\Lmat \left[ \Imat + \lambda\,{\Mmat_{\lambda}}\inv \right] \nonumber \\
&=& \Eunint\, \Lmat \left[ \Imat -  \left[ \Imat + \lambda\,{\Mmat_{\lambda}}\inv \right]\right]
= - \lambda\,\Eunint\, \Lmat  \,{\Mmat_{\lambda}}\inv.
\end{eqnarray}
Together, the theorems read
\begin{eqnarray}
 \label{eq:mcatheoremsdilCOPY}
 {\Cvmat \choose \Ccmat} ( \Kint |\Eunint\,\Lmat) &=& 
 \left(
 \begin{array}{ll}
  \Kint & - \lambda \,\Eunint\, \Lmat \,{\Mmat_{\lambda}}\inv \\
      0 & -\Lmat [\Imat + \lambda\,{\Mmat_{\lambda}}\inv]
 \end{array}
 \right).
\end{eqnarray}


\section{{\Summationconnectivitycondition}}
\label{sec:proofSummationConnectivity}

\subsection{{\Summationconnectivitycondition}  (Proposition \ref{th:theorem1})}
\label{sec:proofequivalenceoptimalitytheorems}

\coout{possibly, replace dg(y) vinv by av for simplicity? auch in p2.2}

\coout{Make sure everything is ok with row vectors, transposed
  vectors, diag around right vectors etc} The cost-benefit balance
Eq.~(\ref{eq:fitnessbalanceeq}) is equivalent to the summation and
{\connectivitycondition}s Eq.~(\ref{eq:fitnessbalance2}) and
(\ref{eq:fitnessbalance3}) whenever the Jacobian $\Mmat=\NR\,\Eunint\,\Lmat$ is invertible (i.e.~$\Eunint$ has full rank).  To show this, we rewrite
Eq.~(\ref{eq:fitnessbalanceeq}), noting that  $\gvtot\trans = \Cmat^{\rm g}_{\rm v}$:
\begin{eqnarray}
\label{eq:fitnessbalancea1}
 \frac{\partial h}{\partial \uv} = 
\frac{\partial \gplus}{\partial \uv} &=& 
\diag\left(\frac{\vv}{\uv}\right)\,{\gvtot} =
\diag\left(\frac{\vv}{\uv}\right)\,({\bvtot}\trans\, \CJmat+ {(-\hc)}\trans\,\CSmat )\trans \nonumber \\
\Leftrightarrow \qquad 
{\Cvmat \choose \Ccmat}\trans {\bvtot \choose (-\hc)}
 &=& \diag\left(\frac{\uv}{\vv}\right) \frac{\partial h}{\partial \uv}
= \diag(\hudot)\,\vv\inv.
\end{eqnarray}
Now we use the summation and connectivity theorems of metabolic
control theory  \cite{Heinrich1996}
\begin{eqnarray}
 \label{eq:mcatheorems}
 {\Cvmat \choose \Ccmat} ({\Kint} |\Eunint\,\Lmat) &=& \left(\begin{array}{ll}{\Kint}&0\\0&-\Lmat\end{array}\right),
\end{eqnarray}
where the matrix $\Eunint$ contains the unscaled reaction elasticities
for internal metabolites. We left-multiply
Eq.~(\ref{eq:fitnessbalancea1}) with $({\Kint}|\Eunint\,\Lmat)\trans$,
apply the theorems, and obtain
\begin{eqnarray}
\label{eq:fitnessbalancea2}
\left(\begin{array}{ll}{\Kint}\trans&0\\0&-\Lmat\trans\end{array}\right) {\bvtot \choose (-\hc)}
 &=& {{\Kint}\trans \choose \Lmat\trans\, \Eunint\trans}\,
 \diag(\hudot)\,\vv\inv.
\end{eqnarray}
These are the {\summationconnectivitycondition}
(\ref{eq:fitnessbalance2}) and (\ref{eq:fitnessbalance3}). To show that 
they do not
only \emph{follow} from the cost-benefit balance (\ref{eq:fitnessbalanceeq}),
but are \emph{equivalent} to it, we note that the matrix
$({\Kint}|\Eunint\,\Lmat)$ is quadratic and has full rank, and 
is therefore invertible;  multiplying with it is an equivalence
transformation. The fact that $({\Kint}|\Eunint\,\Lmat)$ is quadratic
can be seen as follows: if the internal stoichiometric matrix $\Nint$
has size $n_{m} \times n_{r}$ and rank $r$, then ${\Kint}$ has
$n_{r}-r$ columns, and $\Lmat$ has $r$ columns.  Accordingly, $\Mmat =
({\Kint}|\Eunint \Lmat)$ is an $n_{r} \times n_{r}$ matrix. To see
that $({\Kint}|\Eunint\,\Lmat)$ has full rank, we left-multiply it
with ${\Kint\trans \choose \NR}$, which yields a matrix with full
rank (because $\NR\,\Eunint\,\Lmat$ has full rank by assumption).


\co{Continuation:}

To derive  Eqs (\ref{eq:fitnessbalance2x}) and (\ref{eq:fitnessbalance3x}), we start from 
the \emph{{\summationcondition}} and
\emph{{\connectivitycondition}} of metabolic economics
in the form 
\begin{eqnarray}
  \label{eq:fitnessbalance2}
{\Kint}\trans \bvtot &=&  \quad\;\; {\Kint}\trans\, (\hudot \oslashs  \vv) \\
  \label{eq:fitnessbalance3} 
 \Lmat\trans \hc &=& (\Eunint\,\Lmat)\trans\, (\hudot \oslashs  \vv),
\end{eqnarray} 
The kernel
matrix $\Kmat$, the link matrix $\Lmat$, and the elasticity matrix
$\Eunint$ are commonly used in {\MCA} and are explained in the
appendix\footnote{ In Eq.~(\ref{eq:fitnessbalance2}), the kernel
  matrix $\Kmat$ can be replaced by any stationary flux distribution
  $\kv$. By inserting the flux vector $\vv$ itself, we obtain the
  equation
  $\bvtot \cdot \vv = \sum_{l} \hudotl = \sum_{l} \hul\,u_{l}$,
  stating that total {{\fluxbenefit}} and total {{\enzymecost}} must
  be equal.}. The vector $\hudot$ contains the {{\enzymecost}}s
$\hudotl = \hul\,u_{l}$. The  short notation $\hudot \oslashs \vv$ represents 
 the component-wise (Hadamard) division of the two vectors.  To
apply these formulae to a given metabolic state, all reactions must be
active (otherwise some fluxes would vanish, and there would be a
division by zero). If a state contains inactive reactions, these
reactions must be omitted from the model before the analysis.  A
similar {\summationcondition} for models with non-enzymatic reactions
is described in SI \ref{sec:proofnonenzymatic}. 
\co{In models without conserved moieties, the link matrix is given by
  $\Lmat=\Imat$, and the {\connectivitycondition} simply reads
  $\hc =\Eunint\trans\, \acostv$.}  
By defining the  defined the {{\enzymecost}}s
$\hudotl = \hul\,u_{l}$ and the {\fluxburden}s
$\acostvl=\hudotl / v_{l}$, we obtain the form
\begin{eqnarray}
  \label{eq:fitnessbalance2xpre}
\Kmat\trans (\bvtot -\acostv)&=&0  \\
  \label{eq:fitnessbalance3xpre} 
\Lmat\trans (\hc- \Eunint\trans\, \acostv)&=&0.
\end{eqnarray}
The column of $\Kmat$ and $\Lmat$ (and their linear combinations,
respectively), represent the sets of all proper flux variations
$\deltapar \vv$ and concentration variations $\deltapar \cv$.


\subsection{{\Summationconnectivitycondition} for models with dilution}
\label{sec:demandDilution}

For models with dilution (growth rate $\lambda$, Jacobian
$\Mmat_{\lambda} = \NR\,\Eunint\,\Lmat-\lambda\,\Imat$, all reactions
assumed to be enzyme-catalysed), we obtain the summation and connectivity
conditions
\begin{eqnarray}
\label{eq:SIsummationConnectivity}
 \Kint\trans \,\bvtot &=& \Kint\trans\, \diag(\hudot) \vv\inv \nonumber \\
 -\Lmat\trans\, ((-\hc)-\lambda\,\wint)
 &=& (\Eunint\,\Lmat)\trans \, \diag(\hudot)\vv\inv.
\end{eqnarray}

\textbf{Proof} The proof resembles the proof in
\ref{sec:proofequivalenceoptimalitytheorems}.  We just replace the
usual summation and connectivity theorems Eq.~(\ref{eq:mcatheorems})
by the summation and connectivity theorems for models with dilution
(see \ref{sec:proofconnectdilution}),
\begin{eqnarray}
 \label{eq:mcatheoremsdilfinal}
 {\Cvmat \choose \Ccmat} ( \Kint |\Eunint\,\Lmat) &=& 
 \left(
 \begin{array}{ll}
  \Kint &   - \lambda\, \Eunint\, \Lmat\, {\Mmat_{\lambda}}\inv \\
  0 &  - \Lmat [\Imat + \lambda\,{\Mmat_{\lambda}}\inv]
 \end{array}
 \right).
\end{eqnarray}
We proceed as in \ref{sec:proofequivalenceoptimalitytheorems} and
obtain
\begin{eqnarray}
\label{eq:fitnessbalancea2dil}
 \left(
 \begin{array}{ll}
 {\Kint}\trans &  0
 \\ 
 (- \lambda\, \Eunint\, \Lmat\, {\Mmat_{\lambda}}\inv)\trans &
   (-\Lmat [\Imat + \lambda\,{\Mmat_{\lambda}}\inv])\trans 
 \end{array}
 \right)
 {\bvtot \choose -\hc}
 &=& {{\Kint}\trans \choose (\Eunint\,\Lmat)\trans}\,\, \diag(\hudot)\,\vv\inv,
\end{eqnarray}
which can be written as
\begin{eqnarray}
\label{eq:fitnessbalancea2dil2}
 \Kint\trans \,\bvtot 
 &=& \Kint\trans\, \diag(\hudot) \vv\inv \nonumber \\
 - \lambda\,({\Mmat_{\lambda}}\inv)\trans\,\Lmat\trans \,{\Eunint}\trans
 \,\bvtot
 - [\Imat + \lambda\,{\Mmat_{\lambda}}\inv]\trans\, \Lmat\trans\, (-\hc)
 &=& (\Eunint\,\Lmat)\trans\, \diag(\hudot)\vv\inv.
\end{eqnarray}
The last equation can also be written as 
\begin{eqnarray}
\Lmat\trans\, \hc + \lambda\,({\Mmat_{\lambda}}\inv)\trans \,\Lmat\trans\,\hctot
 &=& (\Eunint\,\Lmat)\trans\, \diag(\hudot)\vv\inv
\end{eqnarray}
with $\hctot = \hc - \Eunint\trans\,\bvtot$.  Thus, the summation
condition remains unaffected by dilutioin, while the {\connectivitycondition}
takes up an extra term $\lambda\,({\Mmat_{\lambda}}\inv)\trans \,\Lmat\trans\,\hctot$. 
As shown in section
\ref{sec:SIProofsolveForEcoPot}, this term can be written as $\lambda \,{\wint}'
= \lambda \,\Lmat\trans\,\wint$. We therefore obtain the connectivity
condition:
\begin{eqnarray}
 \Lmat\trans\, (\hc + \lambda \,\wint) =
  \Lmat\trans\, {\Eunint}\trans \, \diag(\hudot)\vv\inv.
\end{eqnarray}

\myparagraph{A second {\summationcondition}} In the {\summationcondition}
Eq.~(\ref{eq:SIsummationConnectivity}), the columns of the matrix
$\Kmat$ represent nullvectors of $\Nint$, i.e.~flows $\kv$ that are
stationary on the network without dilution. Now, instead, we consider
vectors $\kv_{\rm dil}$ (``dilution {\flow}s'') that are stationary in
the system \emph{with} dilution. With a  concentration vector
$\cv$, such {\flow}s must satisfy the stationarity condition
$\Nint\,\kv_{\rm dil} = \lambda\, \cv$. If $\kv_{\rm dil}$ is a
dilution {\flow}, then any vector $\kv_{\rm dil} + \kv$ (with a usual stationary
 {\flow} $\kv$) is also a dilution {\flow}. We 
obtain a {\summationcondition}
\begin{eqnarray}
\label{eq:SIsummationCondDilution1}
 \kv_{\rm dil}\trans \,\bvtot + \lambda\,\wint\cdot \cv&=& \kv_{\rm dil}\trans\, \diag(\hudot) \vv\inv,
\end{eqnarray}
 where the vectors $\wint$ and $\cv$, respectively, 
 contain the economic potentials
 and concentrations of the internal metabolites.

\textbf{Proof of \ref{eq:SIsummationCondDilution1}} We first derive
summation theorems for dilution {\flow}s. Since $\NR\, \kv_{\rm dil} =
\lambda\,\cv'$, we obtain
\begin{eqnarray}
 \CSmat\,\kv_{\rm dil} &=& -\Lmat\,\Mmat_\lambda\inv\,\NR\,\kv_{\rm dil} = -\lambda\,\Lmat\,\Mmat_\lambda\inv\,\cv' \nonumber \\
 \CJmat\,\kv_{\rm dil} &=& (\Eunint\,\CSmat+\Imat)\,\kv_{\rm dil} = -\lambda\,\Eunint\,\Lmat\,\Mmat_\lambda\inv\,\cv' + \kv_{\rm dil}.
\end{eqnarray}
Therefore, 
\begin{eqnarray}
\gvtot \cdot \kv_{\rm dil} &=& [-\hc\trans \,\CSmat + \bvtot\trans\,\CJmat]\, \kv_{\rm dil}  \nonumber \\
 &=&   \hc\trans\,\lambda\,\Lmat\,\Mmat_\lambda\inv\,\cv'
   - \bvtot\trans \,\lambda\,\Eunint\,\Lmat\,\Mmat_\lambda\inv\,\cv' + \bvtot\trans \, \kv_{\rm dil} \nonumber \\
 &=&  - \lambda\,[-\hc\trans + \bvtot\trans\,\Eunint]\,\Lmat\,
        \Mmat_\lambda\inv\,\cv' + \bvtot\trans \, \kv_{\rm dil} \nonumber \\
 &=&  \lambda\,{\wint}' \cdot \cv' + \bvtot\trans \, \kv_{\rm dil}
\end{eqnarray}
For the last line, we used Eq.~(\ref{eq:SIwIndep}).  According to our
standard definition, dependent metabolites have vanishing economic
potentials. Therefore, we can replace ${\wint}' \cdot \cv' = \wint \cdot
\cv$, and obtain the left-hand side of the {\summationcondition}
Eq.~(\ref{eq:SIsummationCondDilution1}). For the left-hand side, we
note that $\gvtot=\diag(\hudot)\,\vv\inv$ as usually.

\subsection{{\Summationconnectivitycondition} for models with inactive or 
 non-enzymatic reactions}
\label{sec:proofnonenzymatic}

To derive {\summationconnectivitycondition} for models with
non-enzymatic reactions, we split the {\flow} $\vv$ into
subvectors $\vv_{\rm enz}$ (active enzymatic reactions) and $\vv_{\rm
  non}$ (inactive or non-enzymatic reactions); the stationary test
vector $\kv$ is split in the same way. The resulting flux and
concentration {\summationconnectivitycondition} read (proof below)
\begin{eqnarray}
\label{eq:demandConditionsNonEnzyProof1}
\kv_{\rm enz}\cdot \bvtot^{\rm, enz} - \kv_{\rm non} \cdot \Delta {\wint}^{\rm , non}
&=& \kv_{\rm enz}\trans \diag(\hudotenz) \,\vv_{\rm enz}\inv. \nonumber \\
\Lmat\trans\,\hc \,  - (\Eunint\,\Lmat)_{{\rm non}}\trans\, \gvnon &=& 
((\Eunint\,\Lmat)_{{\rm enz}})\trans
 \diag(\hudotenz) {\vv_{\rm enz}\inv}.
\end{eqnarray}
where $\gvnon = \Delta \wvsymbol_{\rm non} + {\bvdir}_{\rm non}$.
As a check, we can apply these formulae to models with dilution,
where we 
formally treat the dilution reactions as non-enzymatic
reactions. Setting $k^{\rm dil}_{i} = \lambda\,c_{i}$, $\Delta
\wtoti^{\rm dil} = -\wtoti$, $w^{\rm v, dil}_i=0$ and $\bar E^{\rm
  dil} = \lambda$, the extra terms  read
\begin{eqnarray}
- \kv_{\rm non} \cdot \Delta {\wint}^{\rm , non} &=& \lambda \sum_{i} c_{i}\, \winti
\nonumber  \\
- (\Eunint\,\Lmat)_{{\rm non},i }\trans\, {\gvnon}_{,i} &=&  - \lambda\,(-{\winti}') =  \lambda\,{\winti}'.
\end{eqnarray}
where the prime indicates  independent
internal metabolites.  Using ${\wint}' = \Lmat\trans\,\wint$ (see
section \ref{sec:SIProofsolveForEcoPot}), we obtain the summation and
{\connectivitycondition}s
\begin{eqnarray}
\label{eq:demandConditionsNonEnzyProof2}
\kv_{\rm enz}\cdot \bvtot^{\rm, enz} + \lambda\,\cv \cdot  \wint
&=& \kv_{\rm enz}\trans \diag(\hudotenz) \,\vv_{\rm enz}\inv. \nonumber \\
\Lmat\trans\,(\lambda \, \wint +\hc) &=& ((\Eunint\,\Lmat)_{{\rm enz}})\trans
 \diag(\hudotenz) {\vv_{\rm enz}\inv},
\end{eqnarray}
which should correspond to the equations from the previous section.
The first formula appears to be different.  In the previous section,
however, vectors $\kv$ referred to test modes that would be stationary
on the enzymatic reactions without dilution (even though the system
under study showed dilution); in the present formulae, the vector
$\kv$ is stationary on the entire system \emph{with} dilution, and
$\kv_{\rm enz}$ is the subvector for enzymatic reactions (which,
without the dilution fluxes, would be non-stationary).

\textbf{Proof of Eqs (\ref{eq:demandConditionsNonEnzyProof1})} The
cost-benefit balance for active enzymatic reactions reads (compare
Eq.~\ref{eq:fitnessbalancea1})
\begin{eqnarray}
\label{eq:nonenz1}
\huenz = \guenz = \diag\left(\frac{\vv_{\rm enz}}{\uv_{\rm enz}}\right)\,\gvenz
\quad \Rightarrow \quad 
\gvenz = \diag(\uv_{\rm enz})\diag(\huenz)\, \vv_{\rm enz}\inv
= \diag(\hudotenz)\, \vv_{\rm enz}\inv
\end{eqnarray}
Now let $\kv$ be a test mode, i.e, a stationary mode on the active
subnetwork of  $\vv$. The product $ \kv \cdot \gvtot$  can be split  into
\begin{eqnarray}
 \kv \cdot \gvtot =  \kv_{\rm enz} \cdot \gvenz +  \kv_{\rm non} \cdot \gvnon.
\end{eqnarray}
 Since $\gvtot = \Delta \wint + \bvtot$  and $\Delta \wint\cdot\kv=0$,
we obtain
\begin{eqnarray}
 \kv \cdot \bvtot = \kv \cdot [\gvtot - \Delta \wint] =  \kv \cdot \gvtot 
= \kv_{\rm enz} \cdot \gvenz +  \kv_{\rm non} \cdot \gvnon.
\end{eqnarray}
After inserting Eq.~(\ref{eq:nonenz1}) and rearranging, we obtain the {\summationcondition}
\begin{eqnarray}
 \kv\cdot \bvtot - \kv_{\rm non} \cdot \gvnon
&=& \kv_{\rm enz}\trans \diag(\hudotenz) \,\vv_{\rm enz}\inv.
\end{eqnarray}
This equation can be rewritten as 
\begin{eqnarray}
 \kv_{\rm enz}\cdot \bvtot^{\rm , enz} + \kv_{\rm non}\cdot \bvtot^{\rm , non} 
 - \kv_{\rm non} \cdot \gvnon
&=& \kv_{\rm enz}\trans \diag(\hudotenz) \,\vv_{\rm enz}\inv \nonumber \\
 \kv_{\rm enz}\cdot \bvtot^{\rm , enz} + \kv_{\rm non} (\bvtot^{\rm , non} 
 -  \gvnon)
&=& \kv_{\rm enz}\trans \diag(\hudotenz) \,\vv_{\rm enz}\inv \nonumber \\
 \kv_{\rm enz}\cdot \bvtot^{\rm , enz} - \kv_{\rm non} \cdot \Delta {\wint}^{\rm, non}
&=& \kv_{\rm enz}\trans \diag(\hudotenz) \,\vv_{\rm enz}\inv,
\end{eqnarray}
the desired {\summationcondition}.
Next, to derive the {\connectivitycondition}, we start from 
\begin{eqnarray}
{\gvtot}\trans\, \Eunint\,\Lmat = 
[-\hc\trans \Ccmat + \bvtot\trans \Cvmat]\, \Eunint\,\Lmat = \hc\trans\,\Lmat.
\end{eqnarray}
where we used the connectivity theorem. The left-hand side can  be split into 
\begin{eqnarray}
{\gvtot}\trans\, \Eunint\,\Lmat = 
\gvenz\trans\, (\Eunint\,\Lmat)_{{\rm enz}}
+\gvnon\trans\, (\Eunint\,\Lmat)_{{\rm non}}.
\end{eqnarray}
By equating the tqo equations, we obtain
\begin{eqnarray}
\label{eq:nonenz1y}
 \hc\trans \, \Lmat ={\gvenz}\trans \,(\Eunint\,\Lmat)_{{\rm enz}} 
 + {\gvnon}\trans \,(\Eunint\,\Lmat)_{{\rm non}}.
\end{eqnarray}
By inserting Eq.~(\ref{eq:nonenz1}) and taking the transpose, we obtain
the connectivity  condition
\begin{eqnarray}
\label{eq:nonenz1z}
\Lmat\trans\,\hc \,  &=& 
((\Eunint\,\Lmat)_{{\rm enz}})\trans
\diag(\hudotenz)\,{\vv_{\rm enz}\inv}
 + (\Eunint\,\Lmat)_{{\rm non}}\trans\, \gvnon.
\end{eqnarray}


\subsection{Enzyme cost, flux gain, and flux direction uniquely determine the
 fluxes}
\label{sec:UniquenessProof}

If the enzyme costs, flux gains, and flux directions in an
enzyme-balanced state are given, the {\flow} is uniquely
determined. 

\myparagraph{Proof:} To show
that there is only one solution with given signs, we assume two
solutions $\vv$ and $\wv$ with the same signs (positive signs, without
loss of generality) and show that these solution must be
identical. According to the {\summationcondition}, the solutions $\vv$
and $\wv$  solve the equations
\begin{eqnarray}
\vv\trans\,\diag(\hudot)\,\vv\inv &=& \vv\cdot \bvtot \nonumber \\
\vv\trans\,\diag(\hudot)\,\wv\inv &=& \vv\cdot \bvtot \nonumber \\
\wv\trans\,\diag(\hudot)\,\vv\inv &=& \wv\cdot \bvtot \nonumber \\
\wv\trans\,\diag(\hudot)\,\wv\inv &=& \wv\cdot \bvtot,
\end{eqnarray}
where we considered the  {\summationcondition}s for both solutions and
 inserted the solutions themselves as instances of $\kv$. By
taking differences between these 
equations, we obtain
\begin{eqnarray}
\vv\trans\,\diag(\hudot)\,[\vv\inv - \wv\inv] = 0 \nonumber \\
\wv\trans\,\diag(\hudot)\,[\vv\inv - \wv\inv] = 0.
\end{eqnarray}
By taking  the difference again, we obtain (now written in sum form)
\begin{eqnarray}
\sum_l [v_l - w_l] \trans\,\hudotl\,[\frac{1}{v_l} -\frac{1}{w_l}] = 0.
\end{eqnarray}
Now assume that all elements of $\vv$ and $\wv$ are positive, but  that
some of them differ between $\vv$ and $wv$.
If an element $w_l$ is larger than the corresponding element
$v_l$, the resulting sum element will be negative; if an element $w_l$
is smaller than the corresponding element $v_l$, the resulting sum
element will also be negative. There are no positive sum elements that
could compensate for such negative elements. Therefore, in order for the 
sum to vanish, $\vv$ and $\wv$ must be  identical.

\section{Economical {\flow}s}

\subsection{Test mode criterion (Proposition \ref{th:theoremtestmode})}
\label{sec:prooftheoremtestmode}

Let $\vv$ be a {\complete} {\flow} and $\modevector$ be a {\futile}
test mode of $\vv$ (i.e.~a test mode satisfying $\modevector \cdot
\bvtot=0$). To be economical, $\vv$ must satisfy the summation
condition Eq.~(\ref{eq:fitnessbalance2}) with some positive enzyme
cost vector $\hudot$:

\begin{eqnarray}
\label{app:testmode1}
0 =  \modevector\trans \diag(\hudot) \vv\inv.
\end{eqnarray}
All elements $\hudotl$ are positive, all elements $v_{l}$ are non-zero
and at least some of the elements $t_{l}$ are non-zero. Since
$\vv\inv$ and $\vv$ have the same sign patterns, Eq.~(\ref{app:testmode1}) can
only hold if $t_{l}\,v_{l}>0$ for some index $l$ and $t_{j}\,v_{j}<0$
for some other index $j$.

\coout{\textbf{Alternative proof:} Let $\vv$ be a \co{pervasive} {\flow}
 and $\modevector$ be a {\futile} test mode satisfying $\modevector \ne 0$,
 $\Nint\,\modevector=0$ and $\bvtot\trans\,\modevector=0$. We want to test $\vv$ for
 being economical. According to the  {\summationcondition} Eq.~(\ref{eq:fitnessbalance2}), there
 must be a positive vector $\hudot$ such that \co{links und rechts vertauschen ueberall}

\begin{eqnarray}
 \modevector\trans \diag(\hudot) \vv\inv = 0.
\end{eqnarray}
As $\hudot$ is positive, none of the $v_{l}$ is zero, and at least some
of the $k_{l}$ are non-zero, this can only hold true if
$k_{l}\,v_{l}>0$ for at least some index $l$, and $k_{l'}\,v_{l'}<0$
for some other index $l'$.

Analogy to BEARD: Hence, $\modevector$ and $\vv$ are strictly
 sign-orthogonal. If, on the other hand, $\modevector$ vanishes completely,
 then the supports $\modevector$ and $\vv$ have no indices in common, so
 $\modevector$ and $\vv$ are also strictly sign-orthogonal.}


\subsection{Non-beneficial submodes and the existence of economic potentials}
\label{sec:prooftheoremfutile}

We prove the
following lemma for use in Proposition \ref{th:theoremfutile}:

\textbf{Lemma.}  (a) If a {\complete} {\flow} $\vv$ satisfies the
flux benefit balance (\ref{eq:reactionbalanceeq}) with positive enzyme
costs $\hudotl$, it is free of {\futile} submodes. (b) If a flux
profile $\vv$ is {\complete} and free of {\futile} submodes, it
satisfies the flux benefit balance Eq.~(\ref{eq:reactionbalanceeq}) with
positive enzyme costs $\hudotl$.

For the proof, we recall Gordan's theorem \cite{gord:73}. Let $\Amat$
be a real $m \times n$ matrix and ${\bf 1} = (1, 1, . . . , 1)\trans
\in \Rset^{m}$. Gordan's theorem states that either the inequality
system $\Amat\, \xv > 0$ has a solution $\xv \in \Rset^{n}$ or the
system $\Amat\trans\, \yv = 0, \yv \ge 0$, ${\bf 1}\trans \yv > 0$ has
a solution $\yv \in \Rset^{m}$, but never both. 

\textbf{Proof for direction (a): If $\vv$ satisfies the flux benefit
  balance with a {\fluxgain} vector $\bvtot$ and positive enzyme costs
  $\hudotl$, $\vv$ is free of {\futile} submodes.} We consider a
pervasive flux distribution $\vv$ (without loss of generality, 
 all fluxes $v_{l}$ are positive). If $\vv$
contains a {\futile} submode, there exists a {\futile} test mode
$\modevector$, so
${ \bvtot\trans \choose \Nint} \modevector=0$, $\modevector\ge 0$, and ${\bf 1}\trans
\modevector > 0$. On the contrary, if $\vv$ satisfies the flux benefit balance
\begin{eqnarray}
 \Delta \wintl + \bvtotl &=& \hudotl/v_{l} > 0, \nonumber
\end{eqnarray}
the inequality $(\bvtot | {\Nint}\trans) \, {1\choose \wint}>0$ will
have a solution ${1 \choose \wint}$. According to Gordan's theorem,
only one of these two statements can hold. Thus, whenever the flux
benefit balance holds, $\vv$ cannot contain any {\futile} submodes.

\textbf{Proof for direction (b): If $\vv$ is beneficial ($\bvtot\cdot
  \vv>0$) and free of {\futile} submodes with respect to $\bvtot$,
  it will satisfy a flux benefit balance with flux gain vector
  $\bvtot$ and positive enzyme costs.} If $\vv$ is free of
{\futile} submodes, the inequality system ${\bvtot\trans \choose
  \Nint} \modevector=0, \modevector \ge 0, {\bf 1}\trans \modevector >0$ has no solution
$\modevector$. Thus, according to Gordan's theorem, there must be a solution
$\xv$ to the inequality system ${\bvtot\trans \choose
  \Nint}\trans\,\xv>0$.  Without loss of generality, we can assume
that the first element of $\xv$ is either -1, 0, or 1, and we can
identify the rest of the vector with $\wint$. Thus, one of the
following inequalities must have a solution (for all $l$):
\begin{eqnarray}
\Delta \wintl + \bvtotl > 0 \nonumber\\
\Delta \wintl > 0 \nonumber\\
\Delta \wintl - \bvtotl > 0. \nonumber
\end{eqnarray}
If we multiply the left-hand sides
 with the fluxes $v_{l}$ and sum over all reactions, the term $\sum_{l}
v_{l} \Delta \wintl$ drops out and we obtain the  
 three possible inequalities
\begin{eqnarray}
 \bvtot \trans \vv > 0 \nonumber\\
0 > 0 \nonumber\\
 - \bvtot \trans \vv > 0 \nonumber.
\end{eqnarray}
Since $\vv$ is known to be beneficial ($\bvtot \cdot \vv >0$), it is
the first inequality that holds. Therefore $\Delta \wintl + \bvtotl >
0$ must also hold, and positive enzyme costs will be given by $\hudotl
= [\Delta \wintl + \bvtotl]\,v_{l}$.

\subsection{Criteria for economical {\flow}s  (Proposition  \ref{th:theoremfutile})}
\label{sec:proofecoblanacesummation}

\textbf{Proposition} For pervasive, beneficial {\flow}s $\vv$, the
following statements are equivalent: (i) $\vv$ is economical; (ii)
$\vv$ is beneficial and free of {\futile} submodes; (iii) $\vv$
satisfies the flux benefit balance Eq.~(\ref{eq:reactionbalanceeq}) with
 internal economic potentials $\winti$ and  positive enzyme
costs $\hudotl$.

\textbf{Proof:} To prove the equivalence, we show that each condition
implies the following one in a circle (note that ``being economical'',
by definition, means ``agrees with the {\summationcondition}''):

\textbf{(i $\Rightarrow$ ii) A pervasive, economical {\flow} is
  beneficial and free of {\futile} submodes} The absence of futile
modes follows from the test mode criterion. It implies that the {\flow}
is beneficial and free of {\futile} submodels.

\textbf{(ii $\Rightarrow$ iii) A {\complete} {\flow} that is
  beneficial and free of {\futile} submodes solves the flux benefit
  balance} This was shown in section \ref{sec:prooftheoremfutile}.

\textbf{(iii $\Rightarrow$ i) A {\complete} {\flow} that satisfies
  the flux benefit balance is economical} We start from the flux
benefit balance in the form $ [\Delta \wintl + \bvtotl] =
\hudotl/v_{l}$, multiply it by a test mode $\modevector$, and obtain
\begin{eqnarray}
 \Rightarrow \modevector\trans\,[{\Nint}\trans \wint + \bvtot] &=& \modevector\trans\, \diag(\vv)\inv\, \hudot \nonumber \\
 \Rightarrow \modevector\trans\,\bvtot &=& \modevector\trans\,\diag(\hudot)\, v\inv,
\end{eqnarray}
where we used $\modevector\trans\,{\Nint}\trans = 0$. If this holds for any stationary
flux mode $\modevector$, it will also hold for the kernel matrix $\Kint$.


% --------------------------------------------------------------------

\subsection{Flux cost minimisation and economic flux modes (Proposition \ref{th:theoremPMF1})}
\label{sec:proofFBAmsf}

\paragraph{Proposition} If a metabolic {\flow} $\vv$  solves  a
non-flux-enforcing flux cost minimisation problem
\begin{eqnarray}
\label{eq:SIfcmProof2}
\mbox{Minimise} \quad \acostv(\vv)\quad \mbox{subject to} \quad \Nint \, \vv = 0,  \quad  \bvtotweight \cdot \vv = b,
\end{eqnarray}
then $\vv$ is economical and satisfies a flux benefit balance of the form
\begin{eqnarray}
\label{eq:ReactionBalanceCopyProof}
 [\bvtotweightl + \Delta \wintl]\,v_l = \hudotl
\end{eqnarray}
for all active reactions (where $v_l \ne 0$), with positive values $\hudotl$
and  $\sum_l \hudotl = \sum_l \bvtotweightl\,v_l = b$. With an
appropriate scaling of $\acostv$, we can define $\hudotl =
\frac{\partial \acostv}{\partial v_l}\,v_l$, and the $\wintl$ will be 
given by the Lagrange multipliers associated with the stationarity
condition.

\textbf{Proof 1:} The necessary optimality condition of the  FCM problem reads
\begin{eqnarray}
\label{eq:FCMoptimalitycondition1}
0 = \frac{\partial \acostv}{\partial v_l} - \sum_i \alpha_i\,n_{il}
 - \beta \,\bvtotweightl
\end{eqnarray}
with Lagrange multipliers 
$\alpha_i$ (for the stationarity constraints)
and $\beta$ (for the benefit constraint). Without loss of
generality, we assume that all flux directions are positive (reactions
without flux are omitted,   reaction orientations
 can be redefined). Then, all
derivatives $\frac{\partial \acostv}{\partial v_l}$ must be
positive.  Now we multiply 
Eq.~(\ref{eq:FCMoptimalitycondition1}) with $v_l$ and  obtain
\begin{eqnarray}
\label{eq:FCMoptimalitycondition2}
0 =  \frac{\partial \acostv}{\partial v_l}\,v_l 
 - \sum_{i} \alpha_i\,n_{il}\,v_l  -  \beta \,\bvtotweightl\,v_l.
\end{eqnarray}
With the definitions $\hudotl = \frac{1}{\beta} \frac{\partial
  \acostv}{\partial v_l}\,v_l$ and $\winti = \alpha_i/\beta$, we obtain
\begin{eqnarray}
\label{eq:FCMoptimalitycondition20}
0 =  \hudotl  -  \bvtotweightl\,v_l - \sum_{i} \winti\,n_{il}\,v_l,
\end{eqnarray}
which yields the flux benefit balance
(\ref{eq:ReactionBalanceCopyProof}). Summing over the reactions leads
to $\sum_l \hudotl = \sum_l \bvtotweightl\,v_l = b$ because the sum
$\sum_{il} \winti\,n_{il}\,v_l$ vanishes.  If $\vv$ solves an FCM
problem, it also solves all FCM problems with positively rescaled flux
cost functions. With an appropriate scaling of $\acostv$, we can
ensure that $\beta=1$ (since $b$ is a lower bound, and thus $\beta>0$).

 \textbf{Proof 2: The solutions of FCM problems are free of
   {\futile} submodes} Here is an alternative proof that does not
 involve Lagrange multipliers. I show that {\complete} {\flow}s that
 solve Eq.~(\ref{eq:SIfcmProof2}) are free of {\futile} submodes (as
 we saw before, this implies that these {\flow}s also solve a flux
 benefit balance).  The proof consists of three steps:
\begin{enumerate}[leftmargin=5mm]
\item If $\vv$ has a {\futile} submode (defined by a test mode $\modevector$
  conformal with $\vv$), any linear combination
  $\vv - \varepsilon\, \modevector$ (for small $\varepsilon>0$) violates the
  FBA inequality constraints.  

\textbf{Proof:} Since ${\Nint}\trans
  \modevector =0$ and ${\bvtotweight}\, \trans \modevector = 0$, $\vv - \varepsilon\, \modevector$ is
  stationary and has the same FBA benefit as $\vv$. Moreover,
 it satisfies $|\vv - \varepsilon\, \modevector|_{1} < |\vv|_{1}$
  (for a non-weighted flux minimisation problem) or $\acostv(\vv -
  \varepsilon\, \modevector) < \acostv(\vv)$ (for any FCM problem, where
  $\acostv(\cdot)$ is the flux cost function).  Therefore, $\vv$
  cannot be an optimum of the FCM problem unless $\vv - \varepsilon\,
  \modevector$ violates the inequality constraints.
\item If $\vv - \varepsilon\, \modevector$ violates the inequality constraints
  for arbitrarily small $\varepsilon>0$, the inequality constraints
  must contain some bounds $v^{\rm min}_l>0$ or $v^{\rm max}_l<0$.

  \textbf{Proof:} Assume that $\vv - \varepsilon\, \modevector$ (for any small
  $\varepsilon>0$) violates the lower flux bound for the $l^{\rm th}$
  reaction ($v_{l} - \varepsilon\, k_{l} < v^{\rm min}_{l}$).  Since
  $\vv$ itself satisfies this constraint, the constraint must be
  active, i.e.~$v_{l}=v^{\rm min}_{l}$, and $v^{\rm min}_{l}$ and
  $k_{l}$ share the same signs. Since subtracting $\varepsilon\, k_{l}$
  decreases the flux, this sign must be positive, so $v^{\rm
    min}_l>0$. A similar argument holds for $v^{\rm max}_l<0$.
\item The bounds proven in step 2 would contradict our assumption of a
  non-flux-enforcing FCM problem (where $v^{\rm min}_l \le 0$ and
  $v^{\rm max}_l \ge 0$); therefore, we have ruled out our initial
  assumption that an FCM solution $\vv$  can contain {\futile}
  modes.  This argument can be extended to {\flow}s with inactive reactions: if
  such a {\flow} $\vv$ solves a non-flux-enforcing FCM problem, the
  subvector of active fluxes $\vv_{\rm act}$ will solve a
  corresponding FCM problem on the network's active region. Therefore,
  the active {\flow}, and also $\vv$ itself, must be free of
  {\futile} submodes.

\end{enumerate}

\textbf{Proposition}: If $\vv$ is an economical flux
distribution, satisfying the flux benefit balance
\begin{eqnarray}
\label{eq:SIfcmProof2abc}
 [\bvtotl + \Delta \wintl]\,v_l = \hudotl,
\end{eqnarray}
it is also a solution of the flux cost minimisation problem
\begin{eqnarray}
\label{eq:SIfcmProof2x}
\mbox{Minimise} \quad \acostv(\vv')\quad \mbox{subject to} \quad
 \bvtot \cdot \vv = b, \quad \Nint \, \vv = 0
\end{eqnarray}
with $\acostv(\vv')= \sum_l \frac{\hudotl}{v_l} |v'_l|$.  The
Lagrange multipliers associated with the stationarity condition are
given by the economic potentials $\wintl$ (except for a possible
regauging of conserved moieties), and it holds that $b = \sum_l
\bvtotl\,v_l = \sum_l \hudotl$.

\textbf{Proof for {\complete} {\flow}s:} \coout{LOGIK KLAR? was ist,
  wenn die loesung des FCM-problems nicht eindeutig ist? kann es sein,
  dass die notwendige bedingung erfuellt ist, aber es trotzdem keine
  loesung ist?} Since the FCM problem has no maxima or saddle points,
any {\flow} that satisfies the necessary optimality condition
(\ref{eq:FCMoptimalitycondition1}) will be a flux cost minimum. Thus, we
need to find values of the Lagrange multipliers $\alpha_i$ and $\beta$
that satisfy Eq.~(\ref{eq:FCMoptimalitycondition1}) for all reactions
with $v_l \ne 0$. We can do this by setting 
$\alpha_i=\winti$ and $\beta=1$.  With this choice, the optimality condition 
reads
\begin{eqnarray}
0 \stackrel{!}{=} \hudotl/v_l - \sum_i \alpha_i\,n_{il}  - \bvtotl.
\end{eqnarray}
This is equivalent to the balance equation, which holds true by
assumption.

\textbf{Proof for {\flow}s with inactive reactions:} The proof
can be extended to {\flow}s with inactive reactions: if a flux
profile $\vv$ with inactive reactions is economical, the same {\flow},
restricted to its active region, is {\complete} and economical, and must
 be the solution of an FCM problem on the active region. Based on
this FCM problem, we can now construct an FCM problem for the entire
network, in which fluxes in the inactive region have very large
costs. If these costs are large enough, these fluxes will remain
inactive while the fluxes on the active region will be identical to
our previous solution.

\section{Economic potentials and loads}

\subsection{Economic potentials defined by Lagrange multipliers or by {\MCA} are equivalent}
\label{sec:ProofsPotentialsAreIdentical}

\coout{is it understandable? put reference in main text}

Economic potentials can be defined in several  ways. Here 
I define them by Lagrange multipliers for stationarity
constraints. An alternative definition is based on the metabolic
control coefficients of virtual exchange fluxes 
\cite{lieb:14b}. For the same kinetic model with the same cost and
benefit functions, both  definitions yield the same values and are therefore equivalent.  This is no
surprise because virtual fluxes describe violations of the
stationarity constraints. To formally show this, we first
note that both definitions lead to the same  {\fluxbenefitbalance} equation
\begin{eqnarray*}
\diag(\vv)\,[\bvdir + {\Next}\trans \,\wext  
 + {\Nint}\trans\,\Imat_{\rm R}\trans\,\wind] =\hudot,
\end{eqnarray*}
where $\bvdir$, $\wext$, and $\hudot$ are defined in the same
way. Without loss of generality, we assume that all reactions are
active (i.e.~that $\vv$ covers the entire network). The balance
equation has a unique solution for the independent internal economic
potentials $\windi$. To show this, we note that $
{\Nint}\trans\,\Imat_{\rm R}\trans = {\NR}\trans$ and rearrange the
equation:
\begin{eqnarray*}
 {\NR}\trans\,\wind = \diag(\vv)\inv \,\hudot - [\bvdir + {\Next}\trans \,\wext].
\end{eqnarray*}
Since the right-hand side is fully determined, and since $\NR$ has
full row rank by definition, there can only be one solution for
$\wind$.  This proves that both definitions yield the same numerical
values

\subsection{Adaptive and non-adaptive economic potentials and loads}
\label{sec:proofadaptive}

The economic potentials describe how small virtual exchange fluxes
affect the metabolic benefit in steady state. In their definition, we
assume that enzyme levels stay fixed. If the enzyme levels could be
adapted, this could further increase the benefit. Allowing for such an
adaptation, we would obtain an alternative definition of ``adaptive''
economic potentials. In enzyme-balanced states, however, the
additional benefit is a second-order effect, and adaptive and
non-adaptive economic potentials in such states will thus be
identical.  Thus, as long as we focus on enzyme-balanced states,
adaptive and non-adaptive economic variables need not be
distinguished.

\textbf{Proof.} The non-adaptive economic potentials for
 internal metabolites are defined as
\begin{eqnarray}
 \label{eq:nonadaptintvalueoptcompwind}
 \wind &=& \frac{\partial \gplus}{\partial \virtphiindv} 
 = \frac{\partial z}{\partial \sv} \frac{\partial \sv}{\partial \virtphiindv} 
\end{eqnarray}
where the state vector $\sv(\uv,\xv,\virtphiindv) =
{\vvsteady(\uv,\xv,\virtphiindv) \choose \cvsteady(\uv,\xv,\virtphiindv)}$
contains the steady-sate fluxes and concentrations , $\bbenefit(\sv)$ is the
metabolic objective, and $\gplus(\uv,\cextv,\virtphiindv) =
\bbenefit(\sv(\uv,\cextv,\Lmat \,\virtphiindv))$ is the metabolic benefit
function. For defining adaptive economic potentials, we first
define the adapted enzyme levels $\uv^{\rm opt}$ and the adaptive
fitness function
\begin{eqnarray}
 \label{eq:nonadaptintvalueoptcompwind2}
 \uv_{\frak a}(\cextv,\virtphiindv) &=& \mbox{argmax}_{\uv} \left[\gplus(\uv,\cextv,\virtphiindv) - \hminus(\uv)\right] \nonumber \\
 \ffit_{\frak a}(\cextv,\virtphiindv) &=& \ffit(\uv_{\frak a}(\cextv,\virtphiindv),\cextv,\virtphiindv).
\end{eqnarray}
The adaptive economic potentials for internal metabolites, defined as
${\wind}_{\frak a} = \partial \ffit_{\frak a}/\partial \virtphiindv$, read
\begin{eqnarray}
 \label{eq:intvalueoptcompwind}
 {\wind}_{\frak a} &=& \frac{\partial \ffit_{\frak a}}{\partial \virtphiindv} 
 = \frac{\partial z}{\partial \sv} 
 \left[\frac{\partial \sv}{\partial \virtphiindv} 
 + \frac{\partial \sv}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \virtphiindv} \right] - \frac{\partial \hminus}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \virtphiindv} \nonumber \\
&=&
 \frac{\partial z}{\partial \sv} 
 \frac{\partial \sv}{\partial \virtphiindv} 
 + \left[\frac{\partial z}{\partial \sv} 
 \frac{\partial \sv}{\partial \uv} \right] \frac{\partial \uv_{\frak a}}{\partial \virtphiindv}
- \frac{\partial \hminus}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \virtphiindv}
=\wind + [\gu-\hu]\,\frac{\partial \uv_{\frak a}}{\partial \virtphiindv}.
\end{eqnarray}
In  enzyme-balanced states, the term $[\gu-\hu]$ vanishes, so 
${\wind}_{\frak a} = \wind$. The identidy  for economic
loads can be proven in the same way. We first consider external
metabolites.  If we differentiate $\ffit_{\frak a}$ by $\cextv$
instead of $\virtphiindv$, we obtain
\begin{eqnarray}
 \label{eq:extvalues}
{\loadext}_{\frak a} &=& \frac{\partial \gplus_{\frak a}}{\partial \cextv} 
 = \frac{\partial z}{\partial \sv} 
 \left[\frac{\partial \sv}{\partial \cextv} 
 + \frac{\partial \sv}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \cextv} \right]
 - \frac{\partial \hminus}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \cextv}
= \loadext + [\gu-\hu]\,\frac{\partial \uv_{\frak a}}{\partial \cextv}.
\end{eqnarray}
The proof for internal metabolites is as follows: 
\begin{eqnarray}
 \label{eq:extvaluesProof2}
{\loadint}_{\frak a} &=& {\gc}_{\frak a} + \hc 
= \bvtot\trans  \frac{\partial \vvsteady_{\frak a}}{\partial \gammav} + (-\bc)\trans  \frac{\partial \cvsteady_{\frak a}}{\partial \gammav} 
- \frac{\partial \hminus}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \gammav}
+ \hc  \nonumber \\
&=& \bvtot\trans  [ \frac{\partial \vvsteady}{\partial \gammav} + \frac{\partial \vvsteady}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \gammav}] 
+ (-\bc)\trans  [ \frac{\partial \cvsteady}{\partial \gammav} + \frac{\partial \cvsteady}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \gammav}] 
- \frac{\partial \hminus}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \gammav}
 + \hc \nonumber \\
&=& 
[\bvtot\trans \frac{\partial \vvsteady}{\partial \gammav} 
- \hc\trans  \frac{\partial \cvsteady}{\partial \gammav}  + \hc ]
+ [\bvtot\trans \frac{\partial \vvsteady}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \gammav}
+ (-\hc)\trans \frac{\partial \cvsteady}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \gammav}] 
- \frac{\partial \hminus}{\partial \uv} \frac{\partial \uv_{\frak a}}{\partial \gammav}
\nonumber \\
&=& 
 \loadint + [\gu-\hu]\,\frac{\partial \uv_{\frak a}}{\partial \gammav}.
\end{eqnarray}

\subsection{The  flux prices form a  nullvector of $[\Imat - {\CJmat}]\trans$}
\label{sec:SIproofsFluxPricesNullVector}

We consider a model with flux benefit, assume an enzyme-balanced
state, and omit all inactive reactions. Since the flux control matrix
is a projector matrix ($\CJmat = \CJmat\,\CJmat$), the {\fluxvalue}
vector $\gvtot = {\CJmat}\trans \bvtot$ can be seen as a projection of
$\bvtot$.  Applying the same projection again, we obtain the same
vector ${\CJmat}\trans \gvtot = \gvtot$. This means that
$[\Imat - {\CJmat}]\trans \gvtot = 0$ and, in an optimal state,
$[\Imat - {\CJmat}]\trans \hvv = [\Imat - {\CJmat}]\trans
\diag(\ratelawv)\inv\,\hu = [\Imat - {\CJmat}]\trans
\diag(\hu)\,\ratelawv\inv = 0$.

%\section{Economic loads and metabolite balance}

\subsection{Metabolite  rule}
\label{sec:loadproof}

\coout{schoenerer beweis mit hilfe von projektoreigenschaften?}  The
metabolite rule $\gc = -\hc + \loadint$ relates the total concentration
demands ($\gc = \partial \gplus/\partial \virtgammav$) of internal
metabolites to their concentration gains ($\hc = -\partial
\bbenefit/\partial \cv$) (i.e.~direct demand) plus and indirect
concentration demand called economic load (and defined as $\loadint=
\gc + \hc$). According to the metabolite rule, the loads are given by
$\loadi = \sum_l \gvtotl\,\Eunvlci$. To prove this rule, we
now show that ${\gc}\trans + \hc\trans = \gvtot\trans\,\Eunint$. We
first write the left-hand side as
\begin{eqnarray}
{\gc}\trans + \hc\trans = [-\hc\trans + \bvtot\trans\,\Eunint]\,
\Cmat^{\rm S}_\gamma + \hc\trans = [-\hc\trans +
  \bvtot\trans\,\Eunint]\, [\Cmat^{\rm S}_\gamma -\Imat + \Imat] + \hc\trans.
\end{eqnarray}
With $\Cmat^{\rm S}_\gamma = {\Gmat \choose \NR\,\Eunint}\inv {\Gmat \choose 0}$, we can set  
 $\Imat - \Cmat^{\rm S}_\gamma = {\Gmat \choose \NR\,\Eunint}\inv {0 \choose \NR\,\Eunint}$, and 
continue 
\begin{eqnarray}
 .. &=&  - [-\hc\trans + \bvtot\trans\,\Eunint]\, {\Gmat \choose \NR\,\Eunint}\inv {0 \choose \NR\,\Eunint} +
[-\hc\trans + \bvtot\trans\,\Eunint]  + \hc\trans \nonumber \\
&=&  - [-\hc\trans + \bvtot\trans\,\Eunint]\, {\Gmat \choose \NR\,\Eunint}\inv {0 \choose \NR\,\Eunint} +  \bvtot\trans\,\Eunint.
\end{eqnarray}
Now we compute the right-hand side:
\begin{eqnarray}
 \gvtot\trans\,\Eunint &=& [-\hc\trans \,\Cmat^{\rm S} + \bvtot\trans \,\Cmat^{\rm J}]\, \Eunint
= [-\hc\trans \,\Cmat^{\rm S} +  \bvtot\trans [\Imat - \Eunint \,\Cmat^{\rm S}] ]\, \Eunint\nonumber \\
&=& 
 -[-\hc\trans + \bvtot\trans\,\Eunint] \,\Lmat ( \NR\,\Eunint\,\Lmat)\inv\,\NR\, \Eunint
 + \bvtot\trans\, \Eunint.
\end{eqnarray}
 Both expressions are identical except for the central terms, whose identity still needs to be shown:
\begin{eqnarray}
{\Gmat \choose \NR\,\Eunint}\inv {0 \choose \NR\,\Eunint}
\stackrel{?}{=}\Lmat ( \NR\,\Eunint\,\Lmat)\inv\,\NR\, \Eunint.
\end{eqnarray}
To prove the identity, we left-multiply  with ${\Gmat \choose \NR\,\Eunint}$ and obtain
\begin{eqnarray}
 {0 \choose \NR\,\Eunint}
\stackrel{?}{=}{\Gmat \choose \NR\,\Eunint}\Lmat ( \NR\,\Eunint\,\Lmat)\inv\,\NR\, \Eunint.
\end{eqnarray}
Since $\Gmat \,\Lmat=0$, the right-hand side yields
${0 \choose \NR\,\Eunint\,\Lmat} ( \NR\,\Eunint\,\Lmat)\inv\,\NR\, \Eunint 
= {0 \choose \Imat } \NR\, \Eunint =  {0 \choose \NR\,\Eunint}$.



\subsection{Formula Eq.~(\ref{eq:solveForEcoPot}) for economic potentials}
\label{sec:SIProofsolveForEcoPot}

To derive Eq.~(\ref{eq:solveForEcoPot}) for the economic potentials,
we consider the metabolite rule in the form $\loadint =
\Eun\trans\,[\Delta \wint + \bvtot]$ (splitting the flux demand into
total flux gain $\bvtot$ and the internal economic potential balance
$\wint$).  In models without moiety conservation, we can replace
$\loadint = \hc$ and obtain $\hc = {\Eun}\trans\,{\Nint}\trans\, \wint
+ \Eun\trans\,\bvtot$. Solving for $\wint$ yields Eq.~(\ref{eq:solveForEcoPot}):

\[\wint = -((\Nint\,{\Eun})\trans)\inv\, [\Eun\trans\,\bvtot - \hc] = (\Mmat\trans)\inv\hctot.\]

In models with moiety conservation, we first note that
$\Lmatplus\,\Lmat = \Imat$ and ${\Lmatplus}\trans\,{\wint}'=\wint$ (the
standard definition of economic potentials, whereby dependent
metabolites have vanishing economic potentials), and thus
${\Lmat}\trans\,\wint={\Lmat}\trans\,{\Lmatplus}\trans\,{\wint}'=
{\wint}'$.  We now left-multiply the metabolite rule by $\Lmat\trans$ and
obtain
\[\Lmat\trans\,\loadint =
\Lmat\trans\,\Eun\trans [{\NR}\trans\,\Lmat\trans\, \wint + \bvtot].\]
 Replacing $\Lmat\trans \,\loadint = \Lmat\trans \,\hc$, we 
obtain
\begin{eqnarray}
\Lmat\trans\,\hc &=& \Lmat\trans\,\Eun\trans \,\bvtot +
  \Lmat\trans\,\Eun\trans\,{\NR}\trans\, {\wint}' \nonumber \\
 0 &=& \Lmat\trans\,[-\hc + \Eun\trans \,\bvtot] +
(\NR\,\Eun\,\Lmat)\trans \, {\wint}' \nonumber \\ 
 {\wint}' &=& - ((\NR\,\Eun\,\Lmat)\trans)\inv
\Lmat\trans\,[-\hc + \Eun\trans \,\bvtot],
\end{eqnarray}
and therefore
\begin{eqnarray}
\label{eq:SIwIndep}
\wint = {\Lmatplus}\trans\,{\wint}' 
= - {\Lmatplus}\trans\,((\NR\,\Eun\,\Lmat)\trans)\inv \Lmat\trans\,
[-\hc + \Eun\trans \,\bvtot] = \Lmatplus\trans\,(\Mmat\trans)\inv
\Lmat\trans\,\hctot.
\end{eqnarray}
Note the resemblance to the formula for control
coefficients, which also contains the inverse (but untransposed)
Jacobian \cite{rede:88}.

\paragraph{Example} As an illustration case for 
 Eq.~(\ref{eq:solveForEcoPot}), we consider the linear chain shown in
 Figure \ref{fig:unbranchedfluxART}, with a flux benefit.  Since there
 is no moiety conservation, $\Lmat$ and $\Lmatplus$ can be ignored and
 we can rewrite the equation as $\Mmat\trans\,\wint =
 -\Eunint\trans\,\bvtot.$ We assume a flux $\vv=(1,1,1)\trans$, a flux
 objective $\bbenefit = \bvtot \,\vv$ with $\bvtot = (0,0,7)\trans$,
 and internal economic potentials $\wint = (4,6)\trans$ (obtained from
 adding  the flux-specific enzyme costs along the pathway). With the
 stoichiometric matrix
 $N=\left(\begin{array}{rrr}1&-1&0\\0&1&-1\end{array}\right)$ and the
   elasticity matrix $\Eunint
   =\left(\begin{array}{rr}-1/2&0\\1&-1/2\\0&1\end{array}\right)$, the
     Jacobian matrix reads $\Mmat = \Nint\,\Eunint =
     \left(\begin{array}{rr}-3/2&1/2\\1&-3/2\end{array}\right)$.  With
       these numbers, our equation is satisfied.


\subsection{Enzyme point cost and enzymatic flux point cost are identical}

\co{note that there is another proof for this in cba theory}

Given a cost function $\hminus(\uv)$, the point cost of enzyme $l$ is
defined as $\hudotl = \frac{\partial h}{\partial u_l}\,u_l$. Based on
a kinetic model, we define a flux cost function called  enzymatic
flux cost $\fluxcost^{\rm enz}(\vv)$: for each flux distribution
$\vv$, we consider an enzyme profile $\uv^*(\vv)$ that realises this
flux distribution in our model (and possibly, under constraints on
enzyme and metabolite concentrations), at the lowest possible enzyme cost. The
flux distribution $\vv$ need not be stationary.  We define the
enzymatic flux cost as $\fluxcost^{\rm enz}(\vv) =
\hminus(\uv^*(\vv))$. With this definition, we obtain the equality
\begin{eqnarray}
\label{eq:fluxCostEnzymeCost}
 \frac{\partial \fluxcost^{\rm enz}}{\partial
  v_l}\, v_l = \frac{\partial \hminus}{\partial u_l} \,u_l,
\end{eqnarray}
and can therefore write $\hudotl = \frac{\partial \fluxcost^{\rm
    enz}}{\partial v_l} v_l$.  Eq.~(\ref{eq:fluxCostEnzymeCost}) can
be derived as follows. We compute the variation $\frac{\partial
  \fluxcost^{\rm enz}}{\partial v_l}\, \delta v_l=
\frac{\partial}{\partial v_l} \hminus(\uv^*(\vv)) \, \delta v_l =
\sum_j \frac{\partial \hminus}{\partial u_j} \frac{\partial
  u^*_j(\vv)}{\partial v_l} \, \delta v_l$. The last terms can be
expanded, to first order, as $\frac{\partial u^*_j(\vv)}{\partial v_l}
\, \delta v_l \approx \delta_{jl} \, u_l$.


\subsection{Economic potentials as control variables}
\label{se:SIEcPotControlVariables}

To treat the economic potentials themselves as model variables, the
{\metabolicobjective} function $g(\varphi)$ can be replaced by a transformed
{\metabolicobjective} function
$g'(\wint) = g(\varphi(\wint)) - \sum \varphi_i\,w_i$ with derivatives
$\partial g^*(\wint)/\partial \winti = -\varphi_i$.

\textbf{Proof:} With a {\metabolicobjective} function $g(\varphi)$ depending on
virtual influxes $\varphi_i$, the economic potentials of internal
metabolites are defined as
$\winti = \partial \gplus/\partial \varphi_i$.  The Legendre
transformation yields the transformed {\metabolicobjective} function
$\gplus'(\wint) = \gplus(\varphi(\wint)) - \sum_j \varphi_j(\wint)
\,\wintj$. The derivatives with respect to $\winti$ read
\[ \frac{\partial \gplus'}{\partial \winti} = \sum_j \frac{\partial \gplus}{\partial \varphi_j}
\frac{\partial \varphi_j}{\partial \winti} - \sum_j \frac{\partial
  \varphi_j}{\partial \winti}\,\wintj - \varphi_i(\wint) = -
\varphi_i.\] The enzyme-optimal state is a state in which all
$\varphi_i$ vanish. Therefore, $\partial \gplus'/\partial \winti=0$,
so $\gplus'(\wint)$ has a local extremum in this state.


\section{Economic balance equations}

\coout{
\subsection{Load-force relation Eq.~(\ref{eq:loadfluxvalueequation})}
\label{sec:proofloadfluxvalueequation}

\co{DIRECT Proof by thought experiment with compensated variation:
  (1) Assume an increase of a single metabolite concentration, compensated by
  virtual exchange fluxes for all directly affected reactions. The concentration
  increase $\md c_{i}$ yields immediate flux variations $\md v_{l}=\bar
  E^{v_{l}}_{c_{i}}\,\md c_{i}$, which have to be compensated by
  virtual exchange fluxes $\md \virtphiindm = - \sum_{l} n_{ml} \,\md v_{l} = -
  \sum_{l} n_{ml} \bar E^{v_{l}}_{c_{i}}\,\md c_{i}$. If the steady
  state is stable, then applying these virtual exchange fluxes will
  automatically yield the changes $\md c_{i}$ and $\md v_{l}$, but no
  other changes in the surrounding system. What is the economic
  balance of this change? On the one hand, the change of the metabolic
  benefit can be expressed via the virtual exchange fluxes and the economic
  potentials: $\md g = \sum_{m} {\wint}^{m}\,\md \virtphiindm$. On the
  other, we can express it by the direct effects of $\md c_{i}$ and
  $\md v_{l}$ as $\md g = -\hcm \,c_{m} + \sum_{l} \bvtotl\,v_{l}$. By
  equating both expressions, we obtain
 \begin{eqnarray}
 \label{eq:proofloadpotential1}
\md g &=& \sum_{m} \wintm\,\md \virtphiindm = -\hcm \,\md c_{m} + \sum_{l} \bvtotl\,\md v_{l}
\end{eqnarray}
and, by inserting the expressions for $\md \virtphiindm$ and $\md
v_{l}$ and dividing by $\md c_{i}$, this yields
\begin{eqnarray}
 \label{eq:proofloadpotential2}
 - \sum_{ml} \wintm n_{ml} \bar E^{v_{l}}_{c_{i}}
&=& -\hcm + \sum_{l} \bvtotl\,\bar E^{v_{l}}_{c_{i}} \nonumber \\
\Leftrightarrow \qquad + \hcm 
&=& \sum_{l}\left[\sum_{m}\wintm n_{ml} + \bvtotl\right] \bar E^{v_{l}}_{c_{i}} 
= \sum_{l}\left[\sum_{m}\wtotm n_{ml} + \gvtotl\right] \bar E^{v_{l}}_{c_{i}} 
\end{eqnarray}
}
}

\subsection{Flux benefit balance (Proposition \ref{th:theorembalance}) 
directly derived from cost-benefit balance}
\label{sec:proofeconomicalternative}

In the article, we defined the economic potentials based on supply
fluxes and showed that these potentials satisfy the flux benefit balance.
We can also show this in reverse: we start from the cost-benefit
balance (\ref{eq:fitnessbalanceeq}), derive a balance equation, and
interpret a term in this equation as the vector of economic
potentials:
\begin{eqnarray}
 \label{eq:balancealternativederivation1}
 \frac{\partial \hminus}{\partial \uv} = \frac{\partial \gplus}{\partial \uv}
 &=& \Cmat^{\rm g}\,\diag(\Eunu)
 =  [\bvtot\trans \Cvmat - \hc\trans \Ccmat ]\, \diag(\vv/\uv) \nonumber\\
 &=&[\bvtot\trans (\Imat - \Eunint\,\Lmat\, \Mmat\inv \NR) +\hc\trans \Lmat \, \Mmat\inv\NR]\, \diag(\vv/\uv) \nonumber\\
 &=&[\bvtot\trans - \underbrace{(\bvtot \trans \Eunint - \hc) \,\Lmat\, \Mmat\inv \Lmatplus}_{- \hat \wint \trans}\, \Nint] \, \diag(\vv/\uv).
\end{eqnarray}
With the \emph{definition} $\hat \wint = -(\bvtot \trans \Eunint - \hc)
\,\Lmat\, \Mmat\inv\, \Lmatplus$, we obtain 
\begin{eqnarray}
 \frac{\partial \hminus}{\partial \uv}
 &=& [\bvtot\trans + \hat \wint \trans\,\Nint]\,\diag(\vv/\uv).
\end{eqnarray}
In fact, our definition of $\hat \wint$ exactly matches the formula
Eq.~(\ref{eq:SIwIndep}), obtained from the usual definition of $\wint$.

\coout{can this also be seen in terms of loads??}  \coout{Whenever we
  can require a sign relation $\mbox{sign}(\Cy_{v_{l}})=
  \mbox{sign}(v_{l})$, we obtain a constraint relation analogous to
  the flux benefit balance.}

\subsection{Metabolite balance  (Proposition \ref{th:theorembalance})}
\label{sec:proofinvestmentbalance}

We now prove the metabolite balance Eq.~(\ref{eq:metabolitebalanceequation})
for external metabolite concentrations or model parameters.

\textbf{External metabolites.} For an external metabolite, the
economic load $\loadj$ is defined as $\loadj = \partial \gplus/
\partial \cextj$, where $\gplus(\uv,\xv)$ is the metabolic benefit in
steady state. The load can be written as
\begin{eqnarray}
\label{eq:qloadexternal}
 \loadj = \sum_{l} \gvtotl\, \Eunextlj
\end{eqnarray}
with unscaled elasticities $\Eunextlj$. According to the cost-benefit
balance (\ref{eq:fitnessbalanceeq}), the flux demand $\gvtotl$ must
be balanced with  the  {\fluxburden} $\hvl = \hul\,u_{l}/v_{l}$. By inserting this
into Eq.~(\ref{eq:qloadexternal}), we obtain 
 \begin{eqnarray}
\label{eq:qloadexternal2a}
 \loadj &=& \sum_{l}  \frac{\hul u_{l}}{v_{l}}\,\Eunextlj = 
\sum_{l}  \hvl\,\Eunextlj.
\end{eqnarray}
 Multiplying with the external concentration $\cext_{j}$, we obtain
 \begin{eqnarray}
\label{eq:qloadexternal2}
 x_{j}\, \loadj &=& \sum_{l}  \frac{\hul\, u_{l}\,x_{j}}{v_{l}}\,\Eunextlj
 = \sum_{l} \hul\, u_{l}\, \Escextlj  = \sum_{l} \hudotl\, \Escextlj
\end{eqnarray}
with  scaled elasticities $\Escextlj = \frac{x_j}{v_l}\Eunextlj$. 

\textbf{External parameters} For model parameters $q_r$ affecting
the rates, we can define economic loads $\loadsymbol^{\rm q}_r= \partial
\gplus/\partial q_r$ and obtain an analogous formulae
\begin{eqnarray}
\loadsymbol^{\rm q}_r &=& \sum_{l}  \frac{\hul u_{l}}{v_{l}} \Eunvlpr = 
\sum_{l}  \hvl\, \Eunvlpr \nonumber \\
q_r\, \loadsymbol^{\rm q}_r &=& \sum_{l}  \frac{\hul\,u_{l}\,q_r}{v_{l}} \Eunvlpr.
 = \sum \hudotl\, \Escvlpr.
\end{eqnarray}


\subsection{Metabolite balance with non-enzymatic reactions}
\label{sec:proofinvestmentbalancenonenzymatic}

A metabolite balance can also comprise
non-enzymatic reactions. 

\textbf{External metabolite} We first consider the metabolite rule for an
external metabolite. If we sum over enzymatic and non-enzymatic
reactions separately, Eq.~(\ref{eq:qloadexternal2}) reads
 \begin{eqnarray}
\label{eq:qloadexternal2a}
 x_{j}\, \loadj &=& \sum_{l \in {\rm enz}} \hul\,u_{l}\, \Escextlj
 + \sum_{l \in {\rm non}} \gvtotl \, \Escextlj\,v_{l}.
\end{eqnarray}
With enzyme costs $\hudotl = \hul\,u_{l}$ and flux point benefits $\vbenel = \gvtotl\,v_{l}$, this reads
 \begin{eqnarray}
\label{eq:qloadexternal2b}
 x_{j}\, \loadj &=& \sum_{l \in {\rm enz}} \hudotl\, \Escextlj
 + \sum_{l \in {\rm non}} \vbenel\, \Escextlj.
\end{eqnarray}
\textbf{Internal metabolite} For internal metabolites, we split the
metabolite rule into
\begin{eqnarray}
\label{eq:qloadinternal1a}
\loadi =  \sum_{l \in {\rm enz}, i} \hvl  \, \Eunvlci
 + \sum_{l \in {\rm non}} \gvtotl \, \Eunvlci,
\end{eqnarray}
and the final metabolite balance reads
\begin{eqnarray}
\label{eq:qloadinternal3b}
{\loadi}\,c_{i} &=& \sum_{l \in {\rm enz}, i} \hudotl \, \Escvlci
+ \sum_{l \in {\rm non}} \vbenel \,\Escvlci.
\end{eqnarray}
\textbf{Metabolite balance with dilution fluxes} Dilution in growing
cells can be described by dilution reactions with rates $v^{\rm
  dil}_{i} = \lambda\,c_{i}$. The economic potential difference in
such reactions reads $\Delta \winti = - \winti$.  With the unscaled
elasticities $\bar E^{\rm dil}_{ii} = \md v^{\rm dil}_{i}/\md c_{i} =
\lambda$, we obtain an additional term $-\winti\,\lambda\,c_{i}$ on
the right of the metabolite balance.  Bringing this term to the left, we
obtain the effective economic load ${\loadi}^{\rm , dil} = \loadi +
\winti\,\lambda\,c_{i}$.

\subsection{Closed formula for optimal states}
\label{sec:SIclosedFormula}

With homegeneous cost and benefit functions, and assuming an optimal
state, we can express the fitness as a function of the absolute cost
\begin{eqnarray}
\ffit &=& \gplus - \hminus = \frac{1}{\beta_{\rm v}}\,z_{\rm v} - \frac{1}{\beta_{\rm u}}\,y
      = \left[\frac{1}{\beta_{\rm v}} - \frac{1}{\beta_{\rm u}}\right]\,y = \left[\frac{\beta_{\rm u}}{\beta_{\rm v}}-1\right]\,\hminus,
\end{eqnarray}
where we used the fact that $z_{\rm v} = y$. It follows that
$\gplus = \ffit + \hminus = \frac{\beta_{\rm u}}{\beta_{\rm
    v}}\,\hminus$.

More generally, setting $g=\alpha_v\,u^{\beta_v}$ and
$h=\alpha_u\,u^{\beta_u}$, we can equate point benefit and cost yields
$\beta_v\,\alpha_v\,u^{\beta_v} = \beta_u\,\alpha_u\,u^{\beta_u}$ and
solve for the optimum enzyme level and the optimal fitness:
\begin{eqnarray}
u^{\rm opt} &=&
\left(\frac{\beta_u\,\alpha_u}{\beta_v\,\alpha_v}\right)^{\frac{1}{\beta_v-\beta_u}} \nonumber \\
f^{\rm opt} &=& \left[\frac{\beta_{\rm u}}{\beta_{\rm
      v}}-1\right]\,\hminus = \left[\frac{\beta_{\rm u}}{\beta_{\rm
      v}}-1\right]\,\alpha_u\,u_{\rm opt}^{\beta_u} =
\left[\frac{\beta_{\rm u}}{\beta_{\rm v}}-1\right]\,
\left(\frac{\beta_u\,\alpha_u^2}{\beta_v\,\alpha_v}\right)^{\frac{\beta_u}{\beta_v-\beta_u}}\nonumber  \\
\gplus^{\rm opt} &=& \left[\frac{\beta_{\rm u}}{\beta_{\rm v}}\right]\,
\left(\frac{\beta_u\,\alpha_u^2}{\beta_v\,\alpha_v}\right)^{\frac{\beta_u}{\beta_v-\beta_u}}.
\end{eqnarray}

\section{Construction of models in enzyme-optimal states}
\label{sec:realisekineticmodels}

%\subsection{Reconstruction algorithm}

A {\flow} is called enzyme-optimal if it can be realised by a kinetic
model with a enzyme-optimal stable steady state. To check whether a
given {\flow} is enzyme-optimal, we may attempt to construct such a
model: we first determine a {\flow}, then all other steady-state
variables, and finally the rate laws.  Some of these model variable
can be freely chosen (e.g.~based on experimental data), while others
are constrained or determined by previously chosen variables. The
simultaneous binding modular rate law is used because it provides
simple formulae for reaction elasticities \cite{liuk:10}.  By
construction, the model will be thermodynamically correct and
enzyme-balanced, but it may still be dynamically or economically
unstable. This needs to be checked in the end.

The model in Figure \ref{fig:reconstructed} in the article, for
example, has been constructed in this way.  The construction consists
of three phases.

\textbf{Steady-state phase} In the steady-state phase, we determine
fluxes $\vv$, concentrations $\cv$, chemical potentials $\muv$, and
economic potentials $\wtot$ representing an energetically and
economically feasible steady state. The following constraints must be
satisfied: (i) The fluxes must be stationary ($\Nint\,\vv=0$). (ii)
The flux directions must be energetically feasible (satisfying
$\mbox{sign}(\vv) = \mbox{sign}(-\Deltar \muv)$ where the chemical
potentials are given by $\mu_i = \mu^\circ_i + RT \ln c_i$ and the
reaction affinities by $-\Delta \muv$).  (iii) The flux benefit
balance must be satisfied with positive enzyme costs. In practice, we
can implement this as follows. Concentrations $\cv$ and equilibrium
constants $\kv^{\rm eq}$ together determine the vector of
thermodynamic driving forces, ${\boldsymbol \theta} = -\Delta {\bf
  G}/RT = \ln \kv^{\rm eq} - {\Ntot}\trans \log \cv$.  The equilibrium
constants must satisfy the Wegscheider conditions (${\Nint}\trans\,\ln
\kv^{\rm eq}=0$), and thermodynamic forces and fluxes must share the
same directions ($v_{l}\ne 0 \Rightarrow \mbox{sign}(\theta_{l}) =
\mbox{sign}(v_{l})$). Positive lower bounds on the reaction affinities
$\theta_{l}$ can be used to avoid extreme kinetic properties in later
steps of the algorithm.  Ways to determine such variables are
discussed in \cite{lieb:14b}. One may either compute all quantities
together (by mixed integer linear programming) or first compute
consistent fluxes; concentrations; equilibrium constants; from the
latter, the chemical potentials and thermodynamic driving forces; and,
finally, economic potentials and enzyme costs.  In any case, if the
flow $\vv$ contains inactive reactions, we restrict our model to the
active region. The inactive reactions can be justified by large enzyme
{\price} s or low catalytic constants. From here on, the flux profile
$\vv$ can be assumed to be pervasive.

\coout{Of course, these quantities may also be computed
  differently. The following quantities have to be determined,
  satisfying all relevant conditions: (i) Metabolic network: specify
  stoichiometric matrix $\Ntot$, external metabolites, irreversible
  reactions, controllable reactions (by their indices). (ii) metabolic
  objective: specify which reaction fluxes are directly scored, with
  first and second derivatives $\partial z/\partial v_{l}$ and
  $\partial^{2} z/(\partial v_{l}\,\partial v_{k})$. (iii) Cost
  function: specification of enzyme weights $\alpha_l$ (ones or
  protein lengths) and the first and second derivative $h'$ and
  $h''$. (iv) Choose a {\flow} $\vv$, which needs to be
  stationary ($\Nint\,\vv=0$). (v) Choose non-equilibrium ratios
  $\Gamma_i=c_i/c_i^{eq}$. (vi) Choose positive metabolite concentrations
  $c_i$. The fluxes need to be energetically feasible and
  consistent with the non-equilibrium ratios: $\diag(\vv) {\Ntot}\trans
  \hudot \le 0$, $v_l=0$ if $({\Ntot}\trans \hudot)_l=0$.} 

\coout{WO ?  metabolite balance
    Eq.~(\ref{eq:metabolitebalanceequation})in the form $0 =
    {\Escint}\trans\, \hudot - \loadint$}

\textbf{Kinetic phase} After the steady-state phase, fluxes
$v_{l}$, concentrations $c_{i}$, and chemical potential differences
$\Delta \mu_{l}$ have been fixed, the model has been restricted to
active reactions, and enzyme costs $\hudotl$ and economic potentials
$\wtoti$ have been determined in accordance with the reaction
balance. Now elasticities and economic loads need to be chosen (while 
satisfying
the metabolite balance).  In the kinetic phase, we
choose rate laws that agree with the previously chosen state:
the resulting elasticities must satisfy the metabolite balances
\begin{eqnarray}
\label{eq:reconconstraints}
 \loadi \,c_{i} = \sum_{l} \hudotl\, \Escvlci, \qquad
\loadj\,x_{j} = \sum_{li} \hudotl\, \Escextlj.
\end{eqnarray}
for external and internal metabolites.  In practice, we do this in
reverse: we first determine economic loads and reaction elasticities
that satisfy the metabolite balance and then compute the corresponding
kinetic constants.  Given $x_{j}$, $c_{i}$, and $\hudotl$ (known from
the stead-state phase), the equations
(\ref{eq:reconconstraints}) can be used as linear constraints for
$\loadj$, $\loadi$, and $\Escvlci$.  However, since these variable
have to satisfy more constraints, we express them, in turn, in terms
of other, independent variables.   This works as follows:

\begin{enumerate}[leftmargin=5mm]
\item \textbf{Express elasticities in terms of saturation values} For
  our metabolic state, we next construct the reaction elasticities. To
  choose them consistently, we already decide that eventually, our
  model is going to contain simultaneous binding modular rate laws
  \cite{liuk:10}, saturable rate laws whose scaled elasticities can be
  easily written in terms of thermodynamic forces (which we already
  know) and saturation values (which we are going to determine).  The
  saturation values $\beta^{\rm M}_{li}$, $\beta^{\rm A}_{li}$, and
  $\beta^{\rm I}_{li}$ describe the binding of reactants, allosteric
  activators, and allosteric inhibitors to enzymes in a metabolic
  state in question.  For ease of notation, we define $\alpha^{\rm
    A}_{li} = 1 - \beta^{\rm A}_{li}$. The scaled elasticities of the
  simultaneous binding modular rate law with complete allosteric
  regulation \cite{liuk:10} can be written in terms of thermodynamic
  forces and saturation values as
\begin{eqnarray}
\label{eq:modularelasticities3}
 \Escvlci = \Esctherm_{li} - \beta^{\rm M}_{li} m^{\rm M}_{li}  + \alpha^{\rm A}_{li}\, m^{\rm A}_{li} - \beta^{\rm I}_{li}\, m^{\rm I}_{li}
\end{eqnarray}
where $\Esctherm_{li} = \frac{\zeta_{l} m^{\rm S}_{li} - m^{\rm
    P}_{li}}{\zeta_{l} -1}$, $\zeta_{l} = \e^{- h_{l}\,\Delta
  \mu_{l}/RT}$, $m^{\rm S}_{li}$ and $m^{\rm P}_{li}$ are the
molecularities of substrates and products, and $m^{\rm M}_{li} =
m^{\rm S}_{li} + m^{\rm P}_{li}$. Of course, only relevant saturation
values (corresponding to non-zero values of $m^{\rm S}_{li}$,
$m^{\rm P}_{li}$, $m^{\rm A}_{li}$, or $m^{\rm I}_{li}$) need to be
considered. The coefficients $m^{\rm A}_{li}$ and $m^{\rm I}_{li}$
indicate allosteric regulation.  Formula (\ref{eq:modularelasticities3})
stems from Eqs (33), (34), (35), and (37) in \cite{liuk:10}. 
\coout{With
predefined values $\zeta_{l}$, \co{alle koeff umbenennen}
$m^{\pm}_{li}$, and $w^{\pm}_{li}$, the elasticity $\Escvlci$ depends
linearly on the saturation values.}

\item \textbf{Express internal loads in terms of conserved moiety
  loads} The vector of internal loads $\loadint$ needs to satisfy the
  constraint $\Lmat\trans\, \hc = \Lmat\trans\,\loadint$ (in model
  without moiety conservation, this simply means that 
 $\loadint = \hc$). To account for this constraint, we do not treat
  $\loadint$ as a free variable, but express it as
\begin{eqnarray}
\loadint =  \Gmat\trans\gv^{\rm cm} +\hc
\end{eqnarray}
 in terms of a conserved moiety vector $\gv^{\rm cm}$, which
 is treated as a free variable.

\item \textbf{Linear constraints} By combining the previous equations,
  we obtain the linear constraints for saturation values $\beta^{\rm
    M}_{li}, \beta^{\rm A}_{li}, \beta^{\rm I}_{li}$, conserved moiety
  loads $g^{\rm cm}_k$, and external metabolite loads $\loadj$:
\begin{eqnarray}
\label{eq:modelconstructioninvestment4result}
-\hci\,c_i + \sum_{l} \hudotl\,\Esctherm_{li}
&=&  
c_i\,\sum_k G_{ki}\, g_k^{\rm cm} + \sum_{l} (\hudotl\, m^{\rm M}_{li}) \,\beta^{\rm M}_{li} - (\hudotl\, m^{\rm A}_{li})\, \alpha^{\rm A}_{li} + (\hudotl\, m^{\rm I}_{li}) \,\beta^{\rm I}_{li} \nonumber \\
\label{eq:modelconstructioninvestment3result}
 \sum_{l} \hudotl\, \Esctherm_{lj}
 &=& x_{j}\,\loadj + \sum_{l} (\hudotl\, m^{\rm M}_{lj})\,\beta^{\rm M}_{lj} - \sum_{l} (\hudotl\, m^{\rm A}_{lj}) \,\alpha^{\rm A}_{l} + \sum_{l} (\hudotl\, m^{\rm I}_{lj}) \,\beta^{\rm I}_{lj}.
\end{eqnarray} 
For internal metabolites that are not involved in moiety conservation,
the constraints  read
\begin{eqnarray}
\label{eq:modelconstructioninvestment5result}
-\hci\,c_i + \sum_{l} \hudotl\,\Esctherm_{li}
&=& \sum_{l} (\hudotl\, m^{\rm M}_{li}) \,\beta^{\rm M}_{li} - (\hudotl\, m^{\rm A}_{li})\, \alpha^{\rm A}_{li} + (\hudotl\, m^{\rm I}_{li}) \,\beta^{\rm I}_{li}.
\end{eqnarray} 

\item \textbf{Bounds on saturation values and on external loads} The
  saturation values are constrained by $0 \le \beta_{li} \le 1$ (same
  for $\beta_{li}$), or by lower and upper bounds (e.g.~restrict
  saturation values to the range [0.05, 9.95] to avoid full
  saturation). For economic loads, sign constraints are not mandatory,
  but we can prescribe signs whenever this is plausible.  For
  example, the concentration of imported nutrients is likely to have
  a positive effect on fitness, while the extracellular concentration
  of exported waste products may have the opposite effect. In these
  cases, we may use sign constraints $\sign(\loadj) = -
  \sign\left(\sum_{l} n_{jl}\, v_{l}\right)$.  Similarly, we may
  predefine signs of conserved moiety loads (e.g.~we may require a positive
  load for the conserved moiety ATP+ADP to express the conviction that
  a concentration increase would improve the cell's fitness).
\item \textbf{Solution by sampling or optimisation} Given the linear
  constraints Eq.~(\ref{eq:modelconstructioninvestment3result}) and
  the bounds for the saturation values and conserved moiety loads, we
  can attempt to find solutions by uniform sampling of these variables. Alternatively, to
  obtain a unique solution, we may score the plausibility of certain
  values (e.g.~by assuming a Gaussian probability distribution)
 and use quadratic
  programming to find the constrained maximum. In models without
  conserved moieties, there are no conserved moiety loads, and the
  problem can be determined separately for each metabolite: we consider
  the metabolites one by one and determine for each of them, the
  associated parameters (saturation values $\alpha^{\rm X}_{li}$,
  $\beta^{\rm X}_{li}$ and economic loads $\loadi$ or $\loadj$). For
  problems with conserved moieties, variables belonging to a conserved
  moiety are coupled and must be  determined simultaneously.
\item \textbf{Correction of concentration gains} We first search for a
  solution using a predefined concentration {\price} vector $\hc$. If no
  solution exists, we repeat the search, but allow $\hc$ to deviate
  from its given value. For instance, we can replace $\hc$ in
  Eq.~(\ref{eq:modelconstructioninvestment4result}) by $\hc + \hc^{\rm
    mis}$, thus yielding an additional term $c_i\,{\hci}_{\rm mis}$ on
  the right.  The mismatch vector can be treated as a free variable to be
  minimised ($||\hc^h{\rm mis}|| \stackrel{!}{=}$min).
\item \textbf{Calculation of kinetic constants} Before we determine the
  kinetic constants, we choose enzyme levels $u_{l}$ in a physiologically
  sensible range (based on proteomics data or based on the previously 
chosen enzyme costs
  $\hudotl$ and assumed enzyme {\price} s $\hul$). Then we compute the
  $K_{\rm M}$ values and the activation and inhibition constants (from
  the saturation values and the metabolite concentrations). For each enzyme,
  there remains one unknown parameter $k^{\rm V}_{l}$, the geometric
  mean of forward and reverse catalytic constants. It needs to be
  chosen such that the reaction rates $r_{l}(\cv,\uv)$ from the rate
  laws match the predefined fluxes $v_{l}$. Given the previously
  determined kinetic constants, equilibrium constants, metabolite
  concentrations, enzyme levels, and fluxes $v_{l}$, we can directly
  solve for the constants $k^{\rm V}_{l}$.
\end{enumerate}

\textbf{3. Test for second-order conditions} By construction, our
model has now an enzyme-balanced steady state.  If the state is
dynamically and economically stable (which can be tested by inspecting
the Jacobian and the fitness curvature matrix), the {\flow} is called
enzyme-optimal.  \coout{For each constructed model, both considtions
  need to be checked, and unstable models have to be discarded.
  Moreover, the model, by construction, satisfies the \emph{necessary}
  optimality condition, i.e.~the slope of the fitness function will
  be zero. However, to guarantee a fitness optimum (in contrast to a
  saddle point), it also needs to satisfy the \emph{sufficient}
  condition of being economically stable: the curvature matrix of the
  fitness function, $\Fuu$ has to be negative definite.} We can
require this for all sampled models: if the Jacobian or the fitness
curvature matrix has positive eigenvalues, the sampled model will be
discarded. \coout{or be kept (if only \emph{enzyme extremality} is
  required)}.

%\textbf{Check stable steady state and fitness optimum} 

\coout{\item Compute the scaled concentration elasticities $\Escvlci =
 \frac{\partial v_{l}}{\partial c_{bi}}\frac{c_{m}}{v_{l}}$ (formula
 see \cite{liuk:10}).
\item Compute the internal economic potentials $\wintm$ and
 enzyme costs $\hudotl$ using the above formula. This involves a matrix
 inversion. If the matrix is not invertible, we may not be able to
 construct the model \co{Is this true?? or is it just a non-unique
  solution????} } \coout{Thus, we have $n_{\rm reaction} + n_{\rm
  int}$ linear equations for $n_{\rm reaction} + n_{\rm int}$
 unknowns (enzyme costs $\hudotl$ and internal economic potentials
 $\winti$ for internal metabolites). We can rewrite the equations in
 matrix form:
\begin{eqnarray}
 \label{eq:construction2}
 { \diag(\vv)\, \bvtot \choose \load}
= \left(
\begin{array}{ll}
I & - \diag(\vv) {\Nint}\trans \\
\Esc \trans & 0 
\end{array}
\right)
 { \hudot \choose \bar \wint}
\end{eqnarray}
where the vector $\bar \wint$ contains the economic potentials of the
internal metabolites only. The first matrix on the right has a square shape. If it is also invertible, we
obtain the unique solution:
\begin{eqnarray}
 \label{eq:construction3}
 { \hudot \choose \bar \wint}
= \left(
\begin{array}{ll}
I & - \diag(\vv) {\Nint}\trans \\
\Esc \trans & 0 
\end{array}
\right)\inv
 { \diag(\vv)\, \bvtot \choose \load}.
\end{eqnarray}

A solution $(\hudot, \bar \wint, \Esc\trans)$ can only exist if the
following two requirements are satisfied:
\begin{enumerate}[leftmargin=5mm]
\item 
 In order to be invertible, the square matrix needs to have full
 rank. \co{What otherwise? no solution? or multiple solutions?
 Will that happen if conservation relations hold?} This is
 guaranteed if (i) all $v_{l}$ are non-zero (which we assumed), (ii)
 each column of $\Nint$ has a non-zero entry, and (iii) the scaled
 elasticity matrix, restricted to internal metabolites, has full
 column rank. This means, in particular, that every internal
 metabolite must have a kinetic influence on at least one reaction
 and that the unscaled elasticities of different internal metabolites must not
 be proportional (i.e.~listing the same metabolite in duplicate
 would be a problem). For reasonable kinetic models, it is likely
 that these conditions can be satisfied.

\item The enzyme cost $\hudot$ must be strictly positive for every
 active reaction. Considering Eq.~(\ref{eq:construction2}), this
 implies in particular that $\Esc\trans\,\hudot=\load$ must have a
 solution for strictly positive $\hudot$, i.e.~that (setting
 $\hudot=\hudot'+\varepsilon$)
 \begin{eqnarray}
 \label{eq:construction2bla}
 \Esc\trans\, \hudot' &=& \load - \varepsilon\, \Esc\trans \hat 1 \nonumber \\
 \hudot' &\ge& 0
 \end{eqnarray}
 must have a solution $(\hudot', \bar \Esc\trans)$ for some small positive
 $\varepsilon$. If a matrix $\Esc\trans$ has already been
 predefined, this can be easily tested.
\end{enumerate}
}

%\section{Construction of kinetic models}

\coout{Changes: The solution is not found by linear programming, but
 by quadratic programming with prior values for saturation values and
 economic loads; it may be that predefined internal loads cannot be
 realised; in this case, they are adapted as part of quadratic
 programming; models with moiety conservation are not handled because
 that would entail constraints between elasticities associated with
 different metabolites; this would be possible, but more complicated
 to program and is therefore disregarded. Also mention that by
 increasing the thermodynamics forces (stretching the scale of
 chemical potentials, ET values become less extreme and therefore,
 solutions with zero adjustment of internal economic loads become
 more likely)}

\coout{Also, try to see if the loads for dependent internal
 metabolites can maybe be counted for each metabolite and not added
 for independent metabolites and set to zero for the others}



==> sec_supplement_cba_kinetic.tex <==
\co{WO?

  \includegraphics[width=12cm]{../additional_material/ps-files/backpropagation1.eps}\\
  \includegraphics[width=12cm]{../additional_material/ps-files/backpropagation2.eps}\\

}

\co{

  \begin{figure*}[t!]
  \begin{center}
    \includegraphics[width=14cm]{\psfileslabourvalues/costbenefitcurves2.eps}
  \end{center}
  \caption{\co{REF IN TEXT (gibt schon ref in main article)}
    Cost-benefit and {\myvalue}-{\price} balances for enzymes.  (a)
    Cost-benefit balance. In enzyme-optimal states, the slopes of
    {\metabolicobjective} $g$ and {{\investment}} $h$ as functions of $\ln u$,
    called {{\enzymebenefit}} and {{\enzymecost}}, must be
    balanced. Since enzyme costs are positive, enzymes must have
    positive benefits, i.e.~a positive control over the metabolic
    {\metabolicobjective}.  (b) The slopes of {\metabolicobjective} and {{\investment}}
    (as functions of $u$), called enzyme {\myvalue} and {\price}, must
    also be balanced. The two terms correspond to the two paths in
    Figure \ref{fig:costbenefitcurves1} (b)).  (c) If an enzyme
    {\myvalue} is always below the {{\enzymeprice}}, the enzyme must be
    inactive in optimal states.  (d) This holds, in particular, if the
    enzyme {\myvalue} is negative.}
    \label{fig:costbenefitcurves2}
\end{figure*}

}

\coout{sagen, dass $\Cmat^{\rm g} = - {\hctot}\trans\,\Ccmat$?}


\section{Perturbed metabolic states: description by control coefficients}

\co{this has newly arrived from CBA local; check the entire section!}

\co{anfangssatz: pertrubations of metabolic steady states described by perturbation parameters and control coefficients with respect to these parameters. Here overview of all relevant types of control coefficients and their usage to handle standard metablic models in  MVT.}

\co{refer back to basic model equations (in CBA kin SI? WO?)}

\myparagraph{Systems without moiety conservation} For simplicity, let us
first consider systems without conserved moieties.  In addition to its
dependence on $\esymbolv$ and $\xv$, the metabolic state also depends on
perturbation variables $\virtgamma_{i}$, $\virtnu_{l}$,
$\virtphi_{i}$: $\virtgamma_{i}$ is added to the concentration $c_{i}$
in rate laws or in the benefit function. \co{note that psi and phi
  only apply to independent metabolit concentrations!} $\virtnu_{l}$
is added to $v_{l}$ in mass balances or in the benefit function, and
$\virtphi_{i}$ adds directly to the mass balance of metabolite
$i$. Hence, we replace:
\begin{eqnarray}
  \vv \rightarrow  \vv = \hat \vv + \virtnuv, \qquad
 \cv^{\rm ind} \rightarrow  \cv^{\rm ind}
 = \hat \cv^{\rm ind} + \virtgammav, \qquad \dot \cv \rightarrow \hat{\dot{\cv}}
 = \dot \cv + \Lmat \,\virtphiindv_{\rm ind}
\end{eqnarray}
instead of the stationarity condition
\begin{eqnarray}
  \label{eq:ModelReal}
0 = \dot \cv = \Nint\, \vv = \Nint\, \rv(\cv)
\end{eqnarray}
we now obtain 
\begin{eqnarray}
  \label{eq:ModelVirtual}
0= \dot \cv = \Nint [\rv(\hat \cv + \virtgammav) + \virtnuv] + \Lmat \,{\virtphiv}_{\rm ind}
\end{eqnarray}

\myparagraph{Metabolic control coefficients} \co{note ``sensitivities:
  direct (elasticities) and indirect (control coefficients)} By taking
the derivatives with respect to $\virtgamma_{i}$, $\virtnu_{l}$,
$\virtphi_{i}$, we obtain the derivatives for metabolic state
variables
$c_{i} = \csteady_{i}(\esymbolv,\xv,\virtgammav,\virtphiindv,\virtnuv)$ and
$v_{l} = \vsteady_{l}(\esymbolv,\xv,\virtgammav,\virtphiindv,\virtnuv)$:
\co{first definintions as derivatives!}

They read

\parbox{5cm}{
\begin{eqnarray}
C^{\cvsteady}_{\virtgammav}   & = & 0  \nonumber\\
C^{\vvsteady}_{\virtgammav}   & = & 0 \nonumber
\end{eqnarray}
}
\parbox{5cm}{
\begin{eqnarray}
C^{\cvsteady}_{\virtphiindv}  & = & - (\Nint\,\Eunc)\inv \,\Lmat \nonumber\\
C^{\vvsteady}_{\virtphiindv}  & = & \Eunc\, C^{\cvsteady}_{\virtphiindv} \nonumber
\end{eqnarray}
}
\parbox{5cm}{
\begin{eqnarray}
C^{\cvsteady}_{\virtnuv}     & = &  - (\Nint\,\Eunc)\inv \,\Nint \nonumber\\
C^{\vvsteady}_{\virtnuv}     & = & \Imat + \Eunc\,C^{\cvsteady}_{\virtnuv}.
\end{eqnarray}
}
\co{shift equation number to the right?}

\co{FN. similar definition for other state variables $p_{m}$ with corresponding virtual 
variation parameters $\psi_{m}$}


\co{WO? Control matrices: (definition in CBA I; move graphics there?)

\parbox{8cm}{\includegraphics[width=5.5cm]{/home/wolfram/projekte/cba/zeichnungen/A58.jpg}}
\parbox{8cm}{
  \begin{eqnarray}
    C^{c}_{c} &=& -(N E)\inv\nonumber \\
    C^{c}_{v} &=& C^{c}_{c} N\nonumber \\
    C^{v}_{v} &=& I + E \,C^{c}_{c} N\nonumber \\
    C^{v}_{c} &=& E \,C^{c}_{c} N
  \end{eqnarray}  
}
}

\myparagraph{Systems with moiety conservation} In a model with
conserved moieties (i.e.~a model in which $\Nint$ does not have full
row rank), we split the stoichiometric matrix into
$\Nint = \Lmat\,\NR$ and there is a left-kernel matrix $\Gmat$
satisfying $\Gmat\,\Nint=0$ and accordingly $\Gmat\,\Lmat=0$.  Each
column of $\Lmat$ refers to an independent internal metabolite and
\todo{describes metabolite changes that can be attributed to changes
  of this metabolite}. Each row of $\Gmat$ describes a conserved
moiety. For instance, if there is a conserved moiety ATP + ADP =
const, and ATP is chosen as an independent metabolite, ADP will be
dependent and there can be a column $(1,-1,0,...)\trans$ in $\Lmat$
and a row $(1,1,0, ...)$ in $\Gmat$.  The matrix $(\Lmat|\Gmat\trans)$
is quadratic and invertible. The internal concentrations can be
written as
$\cv(t) = \Lmat\,\cv^{\rm ind}(t) + \Gmat\trans\,\cv^{\rm cm}$, where
the concentrations of the conserved moieties can be determined from
the initial conditions by
$\cv^{\rm cm} = \Gmat^{+} [ \cv(0) - \Lmat\,\cv^{\rm ind}(0)]$.

In system with moiety conservation, the stationarity condition with virtual 
perturbation variables reads 
\begin{eqnarray}
  \label{eq:ModelVirtual2}
  0 = \NR\, [\rv(\hat \cv + \virtgammav) + \virtnuv] + \virtphiindv,
\end{eqnarray}
and since a virtual change $\virtgammav$ will change the conserved
moieties by exactly $\Gmat\,\virtgammav$, we obtain the additional
condition
\begin{eqnarray}
  \label{eq:ModelVirtual3}
 \frac{\partial}{\partial \virtgammav} \Gmat\,\hat \cv = 0 
\end{eqnarray}
Furthermore, we consider state variables given by algebraic equations
$\pv = \pv(\cv)$, which can also appear in the rate laws (with
elasticities $\Emat_{\pv}$) we can perturb by virtual variation
variables $\virtpsiv$.  Some other possibilities in models are not
explicitly considered here because they are already, effectively, covered by our
approach: (i) state variables $\pv$ that depend on $\cv$ and $\vv$ can
effectively be written as dependent on $\cv$ only. (ii) State
variables that are not given by algebraic, but differential equations
can be effectively be written as metabolite concentrations (with a
virtual ``producing reaction'' representing the differential equation.
With these conditions, we obtain \co{C ueberall dick!!}
\begin{eqnarray}
C^{\cvsteady}_{\virtgammav } & = & - {\NR\,\Eunc \choose \Gmat}\inv {\NR\,\Eunc \choose 0} + \Imat
= {\NR\,\Eunc \choose \Gmat}\inv {0 \choose \Gmat}
\end{eqnarray}
and thus

\parbox{8cm}{
\begin{eqnarray}
C^{\cvsteady}_{\virtgammav } & = &  {\NR\,\Eunc \choose \Gmat}\inv {0 \choose \Gmat} \nonumber \\[1mm]
C^{\cvsteady}_{\virtphiindv} & = &  - \Lmat\, (\NR\,\Eunc\,\Lmat)\inv \nonumber \\[1mm]
C^{\cvsteady}_{\virtnuv    } & = &  - \Lmat\,(\NR\,\Eunc\,\Lmat)\inv \NR\nonumber \\[1mm]
C^{\cvsteady}_{\virtpsiv   } & = & - \Lmat\,(\NR\,\Eunc\,\Lmat)\inv \NR\,\Emat_{\pv} \nonumber
\end{eqnarray}
}
\parbox{4cm}{
\begin{eqnarray}
C^{\vvsteady}_{\virtgammav } & = & \Eunc \, C^{\cvsteady}_{\virtgammav }\nonumber \\[1mm]
C^{\vvsteady}_{\virtphiindv} & = &  \Eunc\, C^{\cvsteady}_{\virtphiindv}\nonumber \\[1mm]
C^{\vvsteady}_{\virtnuv    } & = & \Eunc\,C^{\cvsteady}_{\virtnuv    } + \Imat\nonumber \\[1mm]
C^{\vvsteady}_{\virtpsiv   } & = & \Emat_{\pv} + \Eunc\,C^{\cvsteady}_{\virtpsiv    } \nonumber
\end{eqnarray}
}
\parbox{5cm}{
\begin{eqnarray}
C^{\Pv}_{\virtgammav } & = & \Emat^{\Pv}_{\cv} \, C^{\cvsteady}_{\virtgammav} \nonumber \\[1mm]
C^{\Pv}_{\virtphiindv} & = &  \Emat^{\Pv}_{\cv} \, C^{\cvsteady}_{\virtphiindv} \nonumber \\[1mm]
C^{\Pv}_{\virtnuv    } & = & \Emat^{\Pv}_{\cv} \, C^{\cvsteady}_{\virtnuv} \nonumber \\[1mm]
C^{\Pv}_{\virtpsiv   } & = & \Emat^{\Pv}_{\cv} \, C^{\cvsteady}_{\virtpsiv} +\Imat\nonumber
\end{eqnarray}
}

The derivatives with respect to $\virtnuv$ are just the usual control
coefficients, and the derivatives with respect to $\virtpsiv$ are just
the usual parameter response coefficients. For convenience, we also
define the matrices
\begin{eqnarray}
C^{\rm S}_{\virtphiv} &=& C^{\rm S}_{\virtphiindv}\,\Imat\trans_{\rm R} \nonumber \\
C^{\rm J}_{\virtphiv} &=& C^{\rm J}_{\virtphiindv}\,\Imat\trans_{\rm R}
\end{eqnarray}
where $\Imat$ is obtained from a unit matrix (corresponding to the internal metabolites) by selecting the rows corresponding to independent metabolites, such that $\NR = \Imat_{\rm R}\,\Nint$. These matrices are related to the 
usual control matrices by 
\begin{eqnarray}
C^{\rm S} &=& C^{\rm S}_{\virtphiv}\,\Nint  \nonumber \\
C^{\rm J} &=& C^{\rm J}_{\virtphiv}\,\Nint
\end{eqnarray}


\myparagraph{Effect of virtual variations on general state variables}
Consider a state variable $a$ given as a function
$\fluxcost(\vvsteady(\esymbolv,\xv,..),\cvsteady(\esymbolv,\xv,..),\Pv(\esymbolv,\xv,..))$ of the steady-state
concentrations and fluxes. Its derivatives with respect to virtual
variation variables read
\begin{eqnarray}
C^{\rm a}_{\virtgammav } & = & 
{\av^{\rm c}}\trans\, C^{\cvsteady}_{\virtgammav } + 
{\av^{\rm v}}\trans\, C^{\vvsteady}_{\virtgammav }+ 
{\av^{\rm p}}\trans\, C^{\Pv}_{\virtgammav }
= [{\av^{\rm c}}\trans + {\av^{\rm v}}\trans\,\Eunc  + {\av^{\rm p}}\trans\,\Emat^{\Pv}_{\cv}]\, C^{\cvsteady}_{\virtgammav }  
\nonumber \\
C^{\rm a}_{\virtphiindv} & = & 
{\av^{\rm c}}\trans\, C^{\cvsteady}_{\virtphiindv } + 
{\av^{\rm v}}\trans\, C^{\vvsteady}_{\virtphiindv }+ 
{\av^{\rm p}}\trans\, C^{\Pv}_{\virtphiindv }
 = [{\av^{\rm c}}\trans + {\av^{\rm v}}\trans\,\Eunc + {\av^{\rm p}}\trans\,\Emat^{\Pv}_{\cv}]\, C^{\cvsteady}_{\virtphiindv }  
 \nonumber \\
C^{\rm a}_{\virtnuv    } & = &
{\av^{\rm c}}\trans\, C^{\cvsteady}_{\virtnuv } + 
{\av^{\rm v}}\trans\, C^{\vvsteady}_{\virtnuv }+ 
{\av^{\rm p}}\trans\, C^{\Pv}_{\virtnuv }
 = {\av^{\rm v}}\trans + [{\av^{\rm c}}\trans + {\av^{\rm v}}\trans\,\Eunc + {\av^{\rm p}}\trans\,\Emat^{\Pv}_{\cv}]\, C^{\cvsteady}_{\virtnuv }  
 \nonumber \\
C^{\rm a}_{\virtpsiv    } & = &
{\av^{\rm c}}\trans\, C^{\cvsteady}_{\virtpsiv } + 
{\av^{\rm v}}\trans\, C^{\vvsteady}_{\virtpsiv } + 
{\av^{\rm p}}\trans\, C^{\Pv}_{\virtpsiv }
 = {\av^{\rm p}}\trans + [{\av^{\rm c}}\trans + {\av^{\rm v}}\trans\,\Eunc + {\av^{\rm p}}\trans\,\Emat^{\Pv}_{\cv}]\, C^{\cvsteady}_{\virtpsiv }  
\end{eqnarray}
The differential can be written as
\begin{eqnarray}
 \delta a = C^{\rm a} \, {\virtnuv}\, \delta \virtnuv + 
C^{\rm a} \, {\virtphiv}\, \delta \virtphiv + 
C^{\rm a} \, {\virtgammav}\, \delta \virtgammav + 
C^{\rm a} \, {\virtpsiv}\, \delta \virtpsiv.
\end{eqnarray}

\co{WO? EXTRA-ABSCHNITT! TEXT zu duality von CBA field SI hierher!!


  To study compound-reaction duality, we can start from the dual equations
\begin{eqnarray}
\delta \dot{\vv} &=& \Eunc\,\delta \dot{\cv} + \Eune\,\dot{\esymbolv}  \nonumber\\
\delta \dot{\cv} &=& \Nint\,\delta \vv.
\end{eqnarray}

}

\subsection{The fitness  function and its direct derivatives}

\myparagraph{\ \\Basic concepts} Our economic variables (e.g.~values and
economic potentials) are defined as derivatives of the fitness
function. When computing with them, or to establish relations between
them, we need to consider that our benefit-cost calculation is built
around dynamic models of metabolism, and therefore we need to
distinguish between basic variables like our control variables
$\esymbol_{l}$, which can be directly controlled, and state variables, whose
values are obtained by solving the dynamic system, for instance, for a
steady state depending on the basic variables.  We can write
relationships in terms of derivatives. In general, we consider a
benefit function
\begin{eqnarray}
  f(\esymbolv,\xv,\virtphiind) = z(\sv(\esymbolv,\xv,\Lmat \,\virtphiind))) - h(\esymbolv),
\end{eqnarray}
where $h$ is convex and rises monotonically in each variable $\esymbol_{l}$
(or in its absolute value, if $\esymbol_{l}$ is complex).  In a specific
interpretation, $\esymbolv$ is a vector of static enzyme levels, $\xv$ is a
vector of external metabolite concentrations, $\virtphi$ is a vector of static
virtual supply fluxes, $\sv = {\cvsteady \choose \vvsteady}$ is the vector of
steady-state internal concentrations and fluxes.  In a more relatively
general interpretation, $\esymbolv$ can contain any control variables, $\xv$
contains any uncontrollable external variables, $\sv$ is a vector of
metabolic state variables, and $z$ and $h$ are functions scoring the
variables.

\myparagraph{Economic model with separate cost function} \co{include other
  state variables $\pv = \Pv(\esymbolv,\xv)$ (algebraic (depending on c and
  p) or differential (with time derivative depending on c and p); can
  appear in reaction rates, balance equations, and benefit function)} We
first introduce the economic state variables for models with a
separate cost function.  Assume a fitness function
\begin{eqnarray}  
 \ffit(\esymbolv,\xv) = \gplus(\esymbolv,\xv) - \hminus(\esymbolv) = \bbenefit(\sv(\esymbolv,\xv)) - \hminus(\esymbolv)
\end{eqnarray}
with external variables $\xv$, control variables $\esymbolv$, metabolic state $\sv$ (comprising concentrations $\cv = \cvsteady(\esymbolv,\xv)$ and fluxes $\vv = \vvsteady(\esymbolv, \xv)$).
We define some economic variables (in column vectors) by the following  derivatives:
\co{def bv = dq/dv; gc = -dq/dc} \co{fix all the ``b'' variables below: gplus! auch fix bc : -gc}

\begin{eqnarray}
\label{eq:SomeDerivatives}
  \mbox{Enzyme economic tension}\qquad \fu &=& \partial \ffit / \partial {\esymbolv} \nonumber \\
   \mbox{Enzyme value}\qquad   \gu    &=& \partial \gplus / \partial {\esymbolv}\, \nonumber \\
   \mbox{External parameter value}\quad   \gx    &=& \partial \gplus / \partial {\xv}\, \nonumber \\
   \mbox{Enzyme loss}\qquad    \hu    &=& \partial \hminus/ \partial {\esymbolv}\nonumber  \\
   \mbox{Concentration demand}\qquad    {\bf \bbenefit}^{\rm c}    &=& \partial \bbenefit / \partial {\cv}\nonumber  \\
   \mbox{Flux demand}\qquad    {\bf \bbenefit}^{\rm v}    &=& \partial \bbenefit / \partial {\vv}\nonumber  \\
   \mbox{Concentration/enzyme response}\qquad    R^{\rm S}_{\rm u} &=& \partial \cvsteady / \partial {\esymbolv} \nonumber \\
   \mbox{Flux/enzyme response}\qquad    R^{\rm J}_{\rm u} &=& \partial \vvsteady / \partial {\esymbolv}
\end{eqnarray}
Other derivatives can be  defined accordingly. We
obtain the formulae $\fu = \gu - \hu$ and $\gu = {{\bf \bbenefit}^{\rm
    \sv}}\trans\,R^{\rm \sv}_{\esymbolv}$. To define economic variables, we
also consider derivatives with respect to virtual variations:
\begin{eqnarray}
   \mbox{Production value}\quad    \gphi &=& \delta \gplus / \delta \virtphiindv \Imat_{\rm R}\nonumber \\
   \mbox{Flux value}\qquad         \gvtot &=& \delta \gplus / \delta \virtnuv \nonumber \\
   \mbox{Concentration value}\qquad \gc   &=& \delta \gplus / \delta \virtgammav\nonumber \\
   \mbox{Other variable value}\qquad \gp   &=& \delta \gplus / \delta \virtpsiv
\end{eqnarray}

\textbf{Comprehensive economic model} We can also consider fitness
functions that do not contain a separate {{\investment}} term, but in which benefit
and {{\investment}} are combined in a single function:
\begin{eqnarray}  
 \ffit(\esymbolv,\xv) = \bbenefit(\sv(\esymbolv,\xv),\esymbolv, \xv)
\end{eqnarray}
In this case, the enzyme gain and loss from
Eq.~(\ref{eq:SomeDerivatives}) need to be redefined: 
\begin{eqnarray}
   \mbox{Enzyme value}\qquad   \gu    &=& \frac{\partial \bbenefit}{\partial \sv}\,\frac{\partial \,\sv}{\partial{\esymbolv}} \nonumber \\
   \mbox{Enzyme loss}\qquad    \hu   &=& -\partial {\esymbolv} /  \partial \bbenefit.
\end{eqnarray}
Similar other derivatives are defined accordingly.


\subsection{Economic variables}

With the virtual variations of concentrations, production rates,
fluxes, and other state variable, we can define economic values for
all these quantities:
\begin{itemize}[leftmargin=5mm]
\item \textbf{Production value} The production gain of an independent
  internal metabolite is given by the derivative $\partial
  \gplus/\partial \virtphiind_{i}$ of the metabolic benefit with respect
  to the corresponding virtual supply flux. Setting the production gains of all 
other metabolites to 0, we obtain the value vector
 \begin{eqnarray}
{\bf \gplus^{\rm \virtphiind}}\trans = {\wint}\trans = \frac{\partial  \gplus}{\partial \virtphiindv} \,\Imat_{\rm R}
 \end{eqnarray}
which we also call internal economic potential vector.
\item \textbf{Flux value} Likewise, we define the flux gain of  reaction by the 
 derivative $\partial
  \gplus/\partial \virtnu_{l}$ of the metabolic benefit with respect
  to the  virtual flux. We can write the (transposed) flux gain vector as 
 \begin{eqnarray}
{\bf \gplus^{\rm v}}\trans =   \gvtot\trans = \frac{\partial  \gplus}{\partial \virtnuv} 
= \bvtot\trans\,C^{\rm J}_{\virtnu} + {\bc}\trans\,C^{\rm S}_{\virtnu}
= \underbrace{{\bvtot}\trans}_{{(\gvdir)}\trans}  
+ \underbrace{[{\bvtot}\trans\,\Eunc + {\bc}\trans]\,C^{\rm S}_{\virtnu}}_{{\gvind}\trans},
 \end{eqnarray}
thereby splitting it into  direct and indirect flux gains. 
\item \textbf{Concentration value} The concentration gain of an internal metabolite 
is obtained from the derivative $\partial
  \gplus/\partial \virtgamma_{i}$  with respect
  to the virtual concentration variations. The vector reads
  \begin{eqnarray}
{\bf \gplus^{\rm c}}\trans =      \frac{\partial  \gplus}{\partial \virtgammav} = 
\bvtot\trans\,C^{\rm J}_{\virtgamma} + \bc\trans\,C^{\rm S}_{\virtgamma} 
= \bc\trans + 
 \underbrace{[\bvtot\trans\,\Eunc  + \bc\trans] \,C^{\rm S}_{\virtgamma}}_{{\loadint}\trans}
  \end{eqnarray}
thereby splitting it into direct concentration gain (i.e.~concentration demand)
and indirect concentration  value (i.e.~the load). Without moiety conservation,  
$\frac{\partial  \gplus}{\partial \virtgammav} $ vanishes and $\loadint = -\bc $
\item \textbf{Value of general  state variables} For algebraic state
  variables $p_{r}$, the value is defined by the derivative $\partial
  \gplus/\partial \virtpsi_{r}$ with respect to the virtual
  perturbation. This yields
  \begin{eqnarray}
{\bf \gplus^{\rm p}}\trans =    \frac{\partial  \gplus}{\partial \virtpsiv} = 
\bvtot\trans\,C^{\rm J}_{\virtpsi} + \bc\trans\,C^{\rm S}_{\virtpsi} 
= \bc\trans + 
 \underbrace{[\bvtot\trans\,\Eunc  + \bc\trans] \,C^{\rm S}_{\virtpsi}}_{{\loadint}\trans}
  \end{eqnarray}
thereby splitting it into  direct and indirect flux gains. 
\end{itemize}
\co{fix the last one and include demands for p also in other formulae.}

\section{Economic variables, rules, and balance equations}

\co{anfangssatz, sagen dass jetzt alles nochmal verbal erklaert wird,
  und mit mehr details} \co{note that full definitions of all economic
  variables (through virtual variations) are given in the supplement
  of cba local; there is also another discussion of the control
  matrices.  are all relations between the control matrices fully
  explained? is there anything new i could to conclude from these
  relations?}

Metabolic systems in optimal states can be described by economic
variables and their balance equations. To obtain such equations, we
need to understand how local perturbations (e.g.~variations of enzyme
levels) influence steady states. Economic variables (such as economic
potentials $\wint$, {\fluxvalue}s $\gvtot$, concentration {\myvalue}s
$\gc$) can be written in terms of metabolic control coefficients.
Using the framework of Metabolic Control Theory, we can define the
economic potentials as metabolic control coefficients, with the
{\metabolicobjective} as the output variable.  An alternative definition,
described in \cite{lieb:18lagrange}, is based on Lagrange multipliers:
we solve the same optimality problem, but treat rate laws and
stationarity as explicit constraints. The economic potentials and flux
{\myvalue}s can then be defined as the Lagrange multipliers associated
with these constraints (proof in section
\ref{sec:ProofsPotentialsAreIdentical}).

\begin{figure*}[t!]
  \begin{center}
\begin{tabular}{ll}
(a) Tracing the fitness effects of an enzyme & (b) Economic state variables \\
    \includegraphics[width=8cm]{\psfileskinetic/backpropagation1b.eps} & 
    \includegraphics[width=7.5cm]{\psfileskinetic/costbenefitcurves3.eps}
\end{tabular}
  \end{center} 
  \caption{\co{WO? REF IN TEXT!}  \co{ODER: a ist ergaenzte version von abb 1 a!
      a schoen in den main text einbinden. sagen, dass wir nochmal das
      scheme aus abb 1 anschauen und die genauen kausalen wirkungne
      beschreiben; mit hilfe von kontrollkoeffizienten!}  Economic
    variables associated with enzyme levels. (a) Enzyme {\myvalue}s
    describe the fitness effects of enzymes, as mediated by the
    metabolic network.  The {\myvalue} of an enzyme tells us how
    strongly a virtual variation of the enzyme level would affect the
    {\metabolicobjective} function by changing the metabolic state.  To trace such
    indirect effects, we apply the chain rule and split the total
    derivative into a series of direct derivatives (symbolically
    written as ratios of differentials
    $\frac{\delta \gplus}{\delta u} = [\frac{\delta \gplus}{\delta
      \vv} \, \frac{\delta \vv}{\delta r} + \frac{\delta
      \gplus}{\delta \cintv} \, \frac{\delta \cintv}{\delta r}]
    \frac{\delta r}{\delta u}$).  The derivatives
    $\frac{\delta \vv}{\delta r}$ and $\frac{\delta \cintv}{\delta r}$
    of steady-state variations are metabolic control coefficients.
    Metabolic value theory extends the definition of {\myvalue}s from
    model parameters (such as enzyme levels) to all metabolites and
    reactions in the network. \co{say that this tracing can now be
      inverted!}  \coout{Show formulae in table? or ref to table in
      SI?}  (b) \co{wo werden im text die point variables usw gut
      eingefuehrt?  die abbildung dorthin tun} Economic variables. In
    metabolic value theory, the scaled derivatives between {\metabolicobjective} (or
    {{\investment}}, or fitness) and an enzyme level are called
    {{\enzymebenefit}}, enzyme cost, and economic imbalance. The usual
    derivatives are called enzyme {\myvalue}s (or {{\enzymeprice}}s,
    or enzyme stresses\co{opportunity cost? thanks to ron!}).  By
    dividing the scaled derivatives by the flux, we obtain economic
    variables called {\fluxvalue}, {\fluxburden}, and flux stress.  }
  \label{fig:costbenefitcurves1} 
\end{figure*}

\subsection{Economic potentials}
\label{sec:proofenzymebenefitmetabolitevalue}

\myparagraph{\ \\Economic variables and control matrices} Using
control matrices and the chain rule, \coout{supply fluxes must have
  the form $\Lmat\,\virtphiindv$ fix the notation} the internal
economic potentials can be written as (a row vector)
\begin{eqnarray}
\label{eq:SIdefWcint}
{\wint}\trans= \Cmat^{\rm  g}_{\virtphiindv} \Lmatplus =
 [{\bvtot}\trans \Cmat^{\rm  g}_{\virtphiindv} - \hc\trans \Cmat^{\rm  g}_{\virtphiindv}]\,\Lmatplus
= [\bvtot\trans \Cvmat_{\virtphiv} - \hc\trans \Ccmat_{\virtphiv}]\trans
\end{eqnarray}
and the flux and concentration {\myvalue}s can be written as
\begin{eqnarray}
\label{eq:defGV}
\gvtot\trans &=& \Cmat^{\rm  g} = {\bvtot}\trans \Cvmat - \hc\trans \Ccmat \nonumber \\
\gc\trans    &=& \Cmat^{\rm  g}_{\virtgamma} = {\bvtot}\trans \Cvmat_{\virtgamma} 
                               - \hc\trans \Ccmat_{\virtgamma}.
\end{eqnarray}


\myparagraph{Economic potentials and reaction rule} Based on the definition of 
economic potentials, we can now prove
the {\fluxbenefitbalance} equation. Using Eq.~(\ref{eq:SIdefWcint}),
we can compute the vector of economic potential differences
\begin{eqnarray}
\label{eq:controlandvirtual1}
\Deltar \wint 
&=&  {\Nint}\trans\, \wint 
=  [\bvtot\trans \Cvmat_{\virtphiv}\, {\Nint} 
  - \hc\trans \Ccmat_{\virtphiv}\, {\Nint}]\trans 
= [\bvtot\trans (\Cvmat - \Imat) - \hc\trans \Ccmat]\trans
= \gvtot - \bvtot
\end{eqnarray}
and obtain  the equalities
\begin{eqnarray}
\label{eq:controlandvirtual1aa}
 \gvtot &=& \Deltar \wint + \bvtot = \Deltar \wint + \Deltar \wext + \bvdir = \Deltar \wtot + \bvdir.
\end{eqnarray}
By inserting Eq.~(\ref{eq:controlbysupplyproof-1}) into
Eq.~(\ref{eq:SIdefWcint}), we obtain  explicit formulae for  the  economic 
potentials and their differences
\begin{eqnarray}
\label{eq:formulawint}
{\wint}\trans &=& -  [ \bvtot \trans \Eunint - \hc \trans] \,\Lmat\, \Mmat\inv \Lmatplus 
 =  [ \bvtot \trans \Eunint - \hc\trans] \,{\Ccmat_{\virtphi}}
= -{\hctot}\trans\,\Ccmat_{\virtphiv}\nonumber \\
\Deltar \wint &=& -{\hctot}\trans\,\Ccmat_{\virtphiv} \,\Nint=
- {\hctot}\trans\,\Ccmat.
\end{eqnarray}
with the effective concentration {\price}
$\hctot = \hc - \Eunint\trans \,\bvtot$.
  \coout{WEG? Accordingly: ${\wint}\trans =
  [\bvtot\trans \,\Cv_{\virtphiindv} - \hc\trans
    \,\Cc_{\virtphiindv}]\,\Imat_{\rm R} =
  -{\hctot}\trans\Cc_{\virtphiindv}\,\Lmatplus$} 
Thus the global economic variables can be computed from local {\gain}s and {\price}s as
 \begin{eqnarray}
 \label{eq:intvalueoptcompwind6a}
 {\wint}\trans &=& - (\bvtot\trans \Eunint - \hc\trans)\, \Lmat\,(\NR \Eunint\,\Lmat)\inv\,\Lmatplus \nonumber \\
 \Deltar {\wint}\trans &=& 
- (\bvtot\trans \Eunint - \hc\trans)\, \Lmat \,(\NR \Eunint\,\Lmat)\inv\,\NR.
 \end{eqnarray}
These formulae also apply to  models with non-enzymatic reactions and dilution.  
\coout{ We can now consider two special cases.  If the metabolic objective
 $\bbenefit(\vv)$ scores only fluxes, we obtain
 \begin{eqnarray}
 \label{eq:intvalueoptcompwind2}
 {\wint}\trans &=& \bvtot\trans \Cvmat_{\virtphi} = - \bvtot\trans \Eunint \Lmat\, (\NR \Eunint \Lmat)\inv\, \Lmatplus \nonumber \\
 \label{eq:intvalueoptcompwind3}
 \Deltar {\wtot}\trans &=& 
 {\wint}\trans \Nint 
 = - \bvtot\trans \Eunint \Lmat\, (\NR \Eunint \Lmat)\inv \NR 
 = \bvtot\trans (\Cvmat-\Imat) = \bvtot\trans \Cvmat - \bvtot\trans. 
 \end{eqnarray}
and if the metabolic objective $\bbenefit(\cintv)$ scores only internal
 concentrations, 
 \begin{eqnarray}
 \label{eq:intvalueoptcompwind4}
 {\wint}\trans &=& -\hc\trans \Ccmat_{\virtphi} =  \hc\trans \Lmat\, (\NR \Eunint \Lmat)\inv\,\Lmatplus \nonumber \\
 \label{eq:intvalueoptcompwind5}
 \Deltar {\wtot}\trans &=&  \hc\trans \Lmat(\NR \Eunint\,\Lmat)\inv \NR = -\hc\trans \Ccmat.
 \end{eqnarray}}


\myparagraph{Economic potentials in models with dilution} \co{Note
  that an example (small growing cell) is currently in CBA
  Lagrange. should this example be moved here? nee lieber referenz!}
To compute feasible economic potentials $\winti$ and flux demands
$g^{\rm v}_{l}$ for a given network model with dilution, we use the
reaction rule and the metabolite rule for models with dilution (but
without moiety conservation): 
\begin{eqnarray}
\label{eq:formulaForComcentrationValues0}
  \gvtot &=& {\Nint}\trans \wint + {\Next}\trans \wext + \bvdir\nonumber \\
\hc &=&\Eunc \trans \gvtot - \lambda \, \wint.
\end{eqnarray}
Given the external economic potentials and the growth rate $\lambda$,
we can solve for the internal economic potentials.  By combining the
rules Eq.~(\ref{eq:formulaForComcentrationValues0}), we obtain
 \begin{eqnarray}
\label{eq:formulaForComcentrationValues}
 0 &=& 
 -\hc +\Eunc \trans [{\Nint}\trans \wint + {\Next}\trans \wext + \bvdir]
  - \lambda \, \wint \nonumber \\
\Rightarrow \quad \wint
  &=& - 
 ((\Nint\Eunc - \lambda\, \Imat)\trans)\inv [-\hc+\Eunc\trans\,[{\Next}\trans \,{\wext + \bvdir]]} \nonumber \\
 &=& - (\underbrace{(\Nint\Eunc - \lambda\, \Imat}_{\Mmat_\lambda})\trans)\inv 
\underbrace{[ -\hc +\Eunc\trans\, \bvtot]}_{-\hc^{\rm eff}}.
 \end{eqnarray}
 For a solution to exist the system must be dynamically stable and the
 Jacobian matrix $\Mmat_\lambda$ must be invertible.

\myparagraph{Conserved moieties and the gauging of economic
  potentials}
\label{sec:conservedmoieties}
Depending on network structure, there can be conserved
moieties in a model. For instance, if ADP and ATP are only interconverted, but never
produced or consumed individually, their total concentration [ATP]+[ADP]
remains  constant in time.  Conserved moieties are associated with
left-kernel vectors of the internal stoichiometric matrix $\Nint$.
Metabolites that share a conserved moiety have dependent
concentrations. To account for this in our models, we can choose a set of independent
metabolites (concentration vector $\cintv'$) that uniquely determine all
metabolite concentrations. The concentration changes of all
metabolites can be written as
$\md \cintv /\md t = \Lmat\, \md \cintv' /\md t$, with a link matrix $\Lmat$
satisfying $\Nint = \Lmat \, \NR$.  Each conserved moiety is associated
with a vector $\gv_{\rm cm}$ satisfying
$\gv_{\rm cm}\trans \Nint = 0$. We can write such vectors as
$\gv_{\rm cm} = \Gmat\trans\,\qv$, with a left-kernel matrix $\Gmat$
satisfying $\Gmat\,\Nint=0$. For metabolic value theory, moiety
conservation has several consequences:
\begin{enumerate}[leftmargin=5mm]
\item To define the economic potentials of internal metabolites,
  we introduce virtual supply fluxes. In models with moiety
  conservation, the virtual supply fluxes must be chosen such that
   conserved
  moieties are not affected (otherwise, they would create a non-steady
  state).  To satisfy this condition, a vector of  virtual supply fluxes must have the
  form $\virtphiv = \Lmat\,\virtphiindv$, based on virtual supply
  fluxes $\virtphiindv$ for independent metabolites.  With these
  supply fluxes, we can define the economic potentials for independent
  internal metabolites, while the dependent internal metabolites are defined to have
  vanishing economic potentials.

\item To define the  economic potentials in a kinetic model, we need to refer
  to a specific choice of independent metabolites. This means that there is some freedom in the choice of economic potentials. In the flux benefit balance, economic potentials do
  never appear separately, but only in the form of differences $\Delta
  \wtot$. As a consequence, if metabolites form a conserved moiety,
  their economic potentials can be gauged: adding a conserved moiety
  vector $\gv_{\rm cm}$ to the internal economic potential vector ($\wint
  \rightarrow \wint+\gv_{\rm cm}$) does not change the economic
  balances\footnote{If we  define a conserved moiety vector
    $\gv_{\rm cm}$ among all (internal and external) metabolites,
    it will satisfy $\gv_{\rm cm}\trans \Ntot = 0$ and 
    ${\Ntot}\trans [\wtot+\gv_{\rm cm}] = {\Ntot}\trans \wtot$. However,
    adding such a conserved moiety vector will change the external
    economic potentials and thus, the assumed production {\gain}s of
    external metabolites.}  because ${\Nint}\trans [\wint+\gv_{\rm cm}] =
  {\Nint}\trans \wint$.  If metabolites do not participate in active
  reactions, their potentials are irrelevant and can be freely gauged.
  \coout{\item A similar thing holds for the economic loads in the
    compound balance. A compound balance exists for each independent
    metabolite; however, the dependent metabolites are not completely
    irrelevant, but appear in the equation of the metabolites on which
    they depend; both are connected, again, by the link matrix. Again,
    the balance equations do not determine the loads uniquely and
    there remains a gauge freedom $(\loadint \rightarrow \loadint +
    \gv)$ for the economic loads of metabolites forming conserved
    moieties.}
\end{enumerate}
When we estimate economic potentials from measured data, we need to 
remember this gauge freedom: for example, if ATP+ADP is a conserved
moiety, observed enzyme investments will never allow us to determine
the individual economic potentials of ATP and ADP, but only their
difference.  \coout{WIRKLICH? if a {\flow} consists of several
  disconnected parts (not connected by any internal nor external
  metabolites), the potentials within each part can also be regauged.}

\subsection{Economic potentials  derived from the flux variation condition}
\label{sec:FluxVariationConditionLeadsToEconomicPotentials}

In the article, the economic potentials were defined as control
coefficients, and the economic balance equations show that the
potentials, in optimal states, are equal to ``embodied values''
related to enzyme investments. But we can also get to a notion of
economic potentials directly, by starting from a very idea of embodied
values, and based solely on the flux variation condition.  In a linear
metabolic pathway, by summing all enzyme investments upstream of a
metabolite, we obtain the ``embodied enzyme investment'' in that
metabolite, and dividing this by metabolite production rate (i.e.~the
pathway flux), we obtain the ``embodied value'' of that
metabolite. However, this definition works only for linear chains,
where investments simply accumulate from reaction to reaction. But we
can generalise the notion of ``embodied values'' to metabolites in
general networks, with branched and cyclic fluxes. To do so, we
consider the flux variation condition and \co{also refer to more
  elegant proof (and the corresponding proof for
  {\connectivitycondition} and {\compoundbenefitbalance}) in
  \ref{sec:fromSumFormulaToLocal}} \todo{\co{besserer uebergang!
    lieber sagen: cumulative value von linearer kette auf anderes
    verallgemeinern!  nochmal sagen, wo wir tstarten, naemlich bei den
    var cond!}  Let me restate this less technically and show how we
  can get to the notion of economic potentials.} Intuitively, in the
{\summationcondition} we ``probe'' the system with stationary flux
variations and compare the changes in cost and benefit. For optimality
reasons, the two changes must be equal for any possible flux variation
(because they must be equal for any enzyme variation that might have
causes the flux variation). Can we apply this principle also to
non-stationary flux variations, e.g.~a flux variation in a single
reaction? And can we apply similar optimality conditions to other
network elements, to define a notion of ``value'' for metabolites,
instead of enzymes? The cumulative {\fluxvalue}s in Figure
\ref{fig:unbranchedfluxART}, an example of such values, can be
generalised from linear pathways to metabolic networks. Using the
{\summationcondition} Eq.~(\ref{eq:fitnessbalance2x}), we can express
the cost of each enzyme by a value difference between its substrates
and products.  Given $v_l$, $\hudotl$, and $\bvtotl$, we define the
economic potential differences
\begin{eqnarray}
\label{eq:defDeltaW}
  \Deltar \wintl = \hudotl/v_l-\bvtotl.
\end{eqnarray}
As suggested by the symbol, $\Deltar \wint$ is a difference
$\Deltar \wint = \sum_i n_{il}\, \winti$ of quantities $\winti$
associated with metabolites (where only \emph{internal} metabolites
are considered in the difference). We can prove this mathematically by
showing that $\kv\trans\,\Deltar \wint=0$ for all kernel vectors $\kv$
satisfying $\Nint\,\kv=0$; this follows directly from the
{\summationcondition}.  By rearranging Eq.~(\ref{eq:defDeltaW}), we
obtain 
\begin{eqnarray}
(\Deltar \wintl + \bvtotl)\,v_l= \hudotl.
\end{eqnarray}
To rewrite this in terms of economic potentials in general (not only
internal economic potentials), we use
Eq.~(\ref{eq:splitmarginalfluxbenefit}) to split $\bvtotl$ into
$\bvtotl = \Deltar \wextl + \bvdirl$ (where only external metabolites
are considered in $\Deltar \wextl$). By setting
$\Deltar \wtotl = \Deltar \wintl + \Deltar \wextl$ (where \emph{all}
metabolites are considered in $\Deltar \wtotl$), we obtain the
economic reaction balance
\begin{eqnarray}
\label{eq:FluxBenefitBalanceFirst}
(\Deltar \wtotl + \bvdirl)\,v_l= \hudotl.
\end{eqnarray}
The term in brackets, called {\fluxvalue} $\gvtotl$, represents the
total {\myvalue} for the reaction flux $v_l$. the formula shows that
it consists of a direct {\myvalue} $\bvdirl$, which directly scores
the flux, and an indirect {\myvalue} $\Deltar \wtotl$, which scores
the global fitness effects of this flux, as mediated through direct
production and consumption of reactants. This is the economic flux
rule. \co{these are the same economic potentials as those defined by
  control coefficients} \co{note that, in the same way, the economic
  loads can be derived (stimmt das? wie?)}

\co{ REF TO THIS, WO? Direct derivation of metabolite variation condition (and local metabolite balance) from connectivity theorem:

  \subsection{Economic potentials  derived from the metabolite  variation condition}
\label{sec:MetaboliteVariationConditionLeadsToMetaboliteBalance}

  Def Flux value ${w^{tot}}\trans = b_{v}\trans + (-g_{c}\trans + b_{v}\trans\,E_{c}) \,C^{c}$

  Connectivity theorem: $C^{c}\,E_{c}\,L =-L$

  Right-multiplying (1) by $E_{c}\L$ and usin gthe theorem yields
  
  ${w^{tot}}\trans\, E_{c}\,L= b_{v}\trans\, E_{c}\,L - (-g_{c}\trans + b_{v}\trans\,E_{c}) \,L = g_{c}\trans\,L$

  Since in optimal state, $w^{tot} = a_{v}$, we obtain the metabolite variation
  condition

  $(g_{c} + E_{c}\trans a_{v}) \,L= 0$

In models without moiety conservation (where $L=I$), this yields one separate equation for each metabolite. For models with moiety conservation, we can modify the condition, to obtain separate equations.
  
We  use the fact that $(L,G\trans)$ is invertible (since $L$ and $G\trans$ have orthogonal columns, and the right number of columns).

Then we can argue that
\begin{eqnarray}
  (g_{c} + E_{c}\trans a_{v})\, \perp \boldsymbol{\ell}= 0
\end{eqnarray}
for all ${\ell} \in span(N)$, i.e.~possible columns of $L$. Since $span(G\trans)\perp span(L)$, we
obtain
\begin{eqnarray}
  (g_{c} + E_{c}\trans a_{v})\, \in span(G\trans) \nonumber \\
  (g_{c} + E_{c}\trans a_{v}) + G\trans \,w_{cm} = 0
\end{eqnarray}
for a suitable chocie of $w_{cm}$. This yields a local equation for each metabolite!

ALSO refer to this in CBA lagrange (when referring back to (not really local)
optimality condition in CBA opt)
}



\subsection{Economic loads}

\myparagraph{\ \\Metabolite rule for models with conserved moieties} If
an internal metabolite concentration  is perturbed (by adding a certain amount
of the metabolite in one moment), a system may be able return to its
original state. However,  this is not always the case: if a conserved moiety
is affected, this perturbation cannot be undone by the system
dynamics. To describe this, we can split the original perturbation
into a ``controllable'' part that is cancelled and a
``non-controllable'' part that remains and leads to a change of 
 the metabolite  concentrations 
involved in conserved moieties.  By considering a small variation of
the metabolite concentrations (in a vector $\delta \virtgammav$) and tracing
its fate, we can derive the metabolite rule. Here are two possible
derivations.

\textbf{Metabolite rule (Derivation 1):}
The direct effect on 
reaction rates,  $\delta \vv = \Eun\, \delta\virtgammav$, would 
change the fitness by $\gvtot\trans\,\Eun\,\delta \virtgammav$ where
$\gvtot=\Deltar \wtot+\bvdir$.  The local fitness balance thus reads
\begin{eqnarray}
  \delta \gplus = -\hc\trans\,\delta \virtgammav + 
\gvtot\trans\,\Eun\,\delta \virtgammav.
\end{eqnarray}
The same fitness change can also be written in terms of the concentration {\myvalue}s
\begin{eqnarray}
  \delta\gplus = \gc \cdot \delta \virtgammav.
\end{eqnarray}
By equating both formulae and dividing by 
$\delta \virtgammav$, we obtain the metabolite rule
\begin{eqnarray}
{\gc}\trans  \hc\trans = \gvtot\trans\,\Eun.
\end{eqnarray}

\textbf{Metabolite rule (Derivation 2):}
\label{sec:proofecloadcongain}
In our second, alternative derivation, we consider a virtual initial
concentration variation $\delta \virtgamma_i$ of an internal
metabolite. Its marginal effect on the {\metabolicobjective} function $\gplus$
is given by $\gci = \frac{\partial \gplus}{\partial \virtgamma_{i}}$,
which defines the concentration {\myvalue} $\gci$.  In models without
moiety conservation, the system dynamics allows the metabolites to
return to their initial steady state concentrations. In models with
moiety conservation, perturbations of conserved moieties cannot be
undone, and they may permanently change the   {\metabolicobjective}. With the
control matrices $\Cvmat_{\virtgamma}$ and $\Ccmat_{\virtgamma}$ (see section
\ref{sec:SIvirtualVariations}), the
resulting concentration {\myvalue}s can be written as
\begin{eqnarray}
  \label{eq:economicLoad2}
{\gc}\trans = \bvtot\trans\, \Cvmat_{\virtgamma} - \hc\trans \, \Ccmat_{\virtgamma}
 = [\bvtot\trans\, \Eunint - \hc\trans] \, \Ccmat_{\virtgamma}
 = -{\hctot}\trans\, \Ccmat_{\virtgamma}.
\end{eqnarray}
By applying the connectivity theorem from {\MCA}, we can see that it satisfies
${\gc}\trans\Lmat=0$ (see \ref{sec:SIvirtualVariations}).  As shown in
SI \ref{sec:loadproof}, we can further split it into a sum
\begin{eqnarray}
  \label{eq:economicLoad2}
\gci =  -\hci + \sum_l C^{\rm g}_l\, \Eunvlci.
\end{eqnarray}

\myparagraph{The economic load} The \emph{indirect} concentration
value of an internal metabolite $i$, called its economic load
$\loadi$, is given by the total concentration {\myvalue} $\gci$ minus
the direct concentration value (i.e.~the negative metabolite {\price}
$\hci$), that is $\loadi = \gci + \hci$.  The economic load appears
like an effective concentration {\price} promoted by the system,
i.e.~by the fact that the metabolite concentration has a direct effect on
neighbouring reaction rates, and via these rates an effect on the
steady state and on the {\metabolicobjective}.  The metabolite
rule (\ref{eq:economicLoad2}) tells us that the load
$\loadi = \gci + \hci$ can also be written as
$\loadi = \sum_l \gvtotl\, \Eunvlci$.  The vector of internal loads is
therefore given by 
\begin{eqnarray}
  \label{eq:economicLoad}
{\loadint}\trans = \Cmat^{\rm g}\, \Eunint = \bvtot\trans \,\Cvmat \,\Eunint - \hc\trans \,\Ccmat \,\Eunint.
\end{eqnarray}
By multiplying the load vector with the link matrix $\Lmat$ and
applying the connectivity theorem, we obtain the equality
\begin{eqnarray}
\label{eq:proofecloadcongain1}
{\loadint}\trans\,\Lmat = [\bvtot\trans\,\Cvmat -
\hc\trans\,\Ccmat] \,\Eun\,\Lmat = \hc\trans \,\Lmat.
\end{eqnarray}
In models without moiety conservation (i.e.~$\Lmat=\Imat$), this
implies that $\loadint = \hc$ and $\gc=0$.

\subsection{Economic variables in general}

\myparagraph{\ \\Economic {\fluxvalue}s can be obtained from local
  {\gain}s and {\price}s by projection} The formulae
Eqs~(\ref{eq:SIdefWcint}) and (\ref{eq:economicLoad}) for economic
variables show that the global flux and concentration {\myvalue}s can
be obtained from projections of local {\fluxgain}s and concentration
{\price}s: in models with flux objective ($\hc=0$),
Eq.~(\ref{eq:defGV}) shows that the {\fluxvalue} vector
$\gvtot = {\Cvmat}\trans\, \bvtot$ is obtained by applying the
transposed flux projector to the {\fluxgain} vector
$\bvtot$. Similarly Eq.~(\ref{eq:economicLoad2}) shows that the
concentration {\myvalue} vector is obtained as
$\gc = {\Cvmat_{\virtgamma}}\trans \,\bvtot -
{\Ccmat_{\virtgamma}}\trans \,\hc = -
{\Ccmat_{\virtgamma}}\trans\,\hctot$, i.e.~by applying the transposed
concentration projector to the effective proximal concentration
{\price} $\hctot = \hc - {\Eunint}\trans\,\bvtot$.  This holds for any
objective function.

\myparagraph{Potentials and loads can be defined for any state
  variables and functions} \co{gut in paper erwaehnt?} Also another
trick -- rewriting control coefficients as local differences -- works
not only in the case of flux values, but for any differentiable
function $f(\vv,\cintv)$ of the state variables -- including the state
variables themselves, any benefit functions, or even likelihood
functions that relate model predictions to experimental
data. Any such output
variable defines a set of economic potentials.  Given the function
$f(\cintv, \vv)$, we can write its control coefficients as
\begin{eqnarray}
 \Cmat^{\rm f}_{v} &=& ({\fv_{c}}\trans \Ccmat+{\fv_{v}}\trans \Cvmat) = \fv_{v} + ({\fv_{c}}\trans + {\fv_{v}}\trans \Eunint)\, \Ccmat \nonumber\\
&=& \fv_{v} + {\fv_{c*}}\trans\,\Ccmat_{\virtphiind}\,\NR = \fv_{v} + {\wv^{(f)}}\trans\, {\NR}
\end{eqnarray}
with $f_{v_{l}}= \partial f/\partial v_{l}$ and $f_{\cint_{i}}=
\partial f/\partial \cint_{i}$ (direct flux or concentration effects on
$f$), the proximal concentration effects $\fv_{c*}=\fv_{c}\trans +
\fv_{v}\trans \Eunint$, and  $\wv^{(f)} =
     {\Ccmat_{\virtphi}}\trans\,\fv_{c*}$ (internal potentials with
     respect to the variable $f$).  Analogous definitions can
      be given for  other economic variables, such as flux or
     concentration {\myvalue}s or economic loads.

     \co{emphasise likelihood this in paper?} \co{WO?  maybe as an
       example where the splitting of control coefficients is
       explained. // \textbf{Model fitting} In the economic balance
       equations, a global objective (e.g.~represented by flux
       {\gain}s in some distant reaction) is replaced by local proxy
       variables (e.g.~economics potentials). The same trick can also
       be used for model fitting. Imagine that we aim to fit our cell
       model to given flux, metabolite, and enzyme data \co{But what
         about enzyme cost - would it also arise from a least-squares
         fit?  is it a problem that the costs may be non-positive?}
       by maximising the negative weighted sum of squared residuals
\begin{eqnarray}
  \label{eq:fluxesclosetodata}
F(\vv,\cv,\esymbolv) =
    - \underbrace{\sum_{l} \frac{(v_{l}- v^{\rm exp}_{l})^{2}}{(\sigma^{\rm v}_{l})^{2}}}_{-\fluxcost(\vv)}
   - \underbrace{\sum_{i} \frac{(c_{i}- c^{\rm exp}_{i})^{2}}{(\sigma^{\rm c}_{i})^{2}}}_{\metcost(\cv)}
   - \underbrace{\sum_{l} \frac{(u_{l}- u^{\rm exp}_{l})^{2}}{(\sigma^{\rm u}_{l})^{2}}}_{\hminus(\esymbolv)}.
\end{eqnarray}
We can use this an a hypothetical fitess function! The only difference
is that now the ``enzyme {\price}s'' $\hul$ may not be strictly
positive; this means, for example, that the fluxes may also lead from
higher to lower economic potentials. Aside from this detail, all
economic variables can be defined (telling us how changes in the
simulated metabolic state would improve the fit), and the economic
balance equations will hold. The equations tell us about how different
model variables ``compete'' in contributing to the goodness of fit.}

\subsection{Reaction rule: writing control coefficients as differences
  along reactions}
\label{sec:SIderivationReactionRule}

To derive the reaction rule, we express the
economic variables by metabolic control coefficients:
\begin{eqnarray}
   \label{eq:enzymebalance0A}
\gu\trans\,  \diag(\enzymev/\vv)
&=& {\bvtot}\trans\, \Cvmat - \hc\trans \, \Ccmat  \nonumber \\
&=& {\bvtot}\trans\, (\Imat + \Eunc\, \Ccmat) - \hc\trans \, \Ccmat  \nonumber \\
&=& {\bvtot}\trans + ({\bvtot}\trans\,\Eunc - \hc\trans) \, \Ccmat \nonumber \\
&=& {\bvdir}\trans + \underbrace{{\bpsi}\trans}_{{\wext}\trans}\,\Next
    + \underbrace{({\bvtot}\trans\,\Eunc - \hc\trans) \, \Ccind_{\virtphi}}_{{\wint}\trans}\,\Nint  %\nonumber \\
%&=& {\bvdir}\trans + {\wint \choose \wext}\trans {\Nint \choose  \Next} \nonumber \\
= {\bvdir}\trans + \Deltar \wtot.
\end{eqnarray}
\co{die herleitung ist zu detailliert? formel ins SI, hier nur
  $\Ccmat = \Ccmat_{\virtphi}\,\Nint$ verraten} \co{ALLG: the fact
  that the indirect flux value can be written as a difference of
  production values comes from $\Ccmat = \Ccmat_{\virtphi}\,\Nint$}
\co{formel erklaeren, REF to SI} The same trick -- writing economic values
associated with reaction as a difference of economic values
associated with  metabolite production in that reaction
-- can be applied  generally, even if  $f$ is for instance a likelihood
function, scoring possible model states by comparing them to
experimentally measured state variables: \co{was kommt dabei raus?}
all control coefficients (for any differentiable function
$f(\vv,\cintv)$ of the state variables $\vv$ and $\cintv$) can be
written as local differences
\co{$\Cmat^{\rm a}_{v} = \av^{v} + \bv\trans\, {\NR}$} of ``compound
control coefficients''. \co{WORT!}  (see SI
\ref{sec:proofeconomicalternative}).  \co{kann man die metabolitregel
  mit einem aehnlichen {\MCA}-trick erklaeren?}


\subsection{Economic laws in their different forms}

\myparagraph{\ \\Different formulations of the economic balance
  equations} The economic balance equations describe how variations of
the metabolic state affect cell fitness. Variations can be described
in various ways, as differential or finite changes of state variables,
or directly in terms of fitness derivatives. Accordingly, the economic
laws can be given in different forms.  For example, the reaction
balance can be written in four different formulations, referring to
(i) enzyme {\myvalue} and enzyme {\price}, (ii) {\fluxvalue} and
{\fluxburden}, (iii) {\enzymecost} and {\enzymebenefit}, or (iv)
differential enzyme cost and differential enzyme benefit.  To derive
these formulations, we start from the enzyme {\myvalue}-{\price}
balance $\gu = \hu$. By inserting
$\gu\trans = \Cmat^{\rm g}\, \diag(\vv)\diag(\esymbolv)\inv$ and multiplying
with different variables from the right (and the symbols
$\odots$ and $\oslashs$ for componentwise vector multiplication and division)
\begin{eqnarray}
\Cmat^{\rm g}\, \diag(\vv\oslashs\esymbolv) &=& \hu\trans \nonumber \\
\Cmat^{\rm g} &=& \hu\trans \,\diag(\esymbolv\oslashs\vv)\nonumber \\
\Cmat^{\rm g}\, \diag(\vv) &=& \hu\trans \,\diag(\esymbolv) \nonumber \\
\Cmat^{\rm g}\, \diag(\delta \vv) &=& \hu\trans \,\diag(\esymbolv\oslashs\vv\odots\delta \vv) = \hu\trans \,\diag(\delta \esymbolv)
\end{eqnarray}
Similarly, starting from
${\Cmat^{\rm g}}\trans = \gvtot = \Deltar \wtot + \bvdir$, we obtain
four formulations of the reaction balance: \co{die formeln kommen
  jetzt auch in appendix; hier weg?}
\begin{eqnarray}
  \left[\Deltar \wtot + \bvdir\right] \odots \vv \oslashs \esymbolv &=&  \hu \quad\qquad\qquad\qquad\mbox{Enzyme \valueform}\nonumber \\
  \Deltar \wtot + \bvdir &=&  \hu \odots \esymbolv \oslashs \vv = \hvv \qquad\mbox{Flux \valueform}\nonumber \\
  \left[\Deltar \wtot + \bvdir\right] \odots \vv &=&  \hu \odots \esymbolv = \hudot \quad\qquad\mbox{Partial \pointbenefitform}\nonumber \\
  \left[\Deltar \wtot + \bvdir\right] \odots \delta \vv &=&  \hu  \odots \delta \esymbolv =\delta \hudot \qquad\mbox{Differential \pointbenefitform}
\end{eqnarray}
Given the reaction balance in \enzymevalueform, all other forms can
be simply obtained by multiplying with $u$, $u/v$, or $\delta
u$. \co{entsprechende formulierungen for
  other balance equations, rules, etc. // Example:
  $-\cintv \odots \hc = -\sum_l \Escint \hudot \hc = \cintv\inv \odots
  [\Escint\, \hudot] = \Eunint\,\acostv$ ???}

\section{Variants of the economic laws for more complicated models}
\label{sec:extensions}

In the article, we have made many simplifying assumptions about our kinetic
models (e.g.~each reaction must be catalysed by a specific enzyme) and
optimality problems  (e.g.~metabolite concentrations are scored by a cost, but are not
constrained by hard bounds).  We now drop some of these assumptions to make the theory
 applicable to a wider range of models or optimality problems.

\subsection{Isoenzymes and unspecific enzymes}
\label{sec:isoenzymes}
\label{sec:SIreactionBalanceNonUniqueEnzymes}

So far, we assumed that reactions are enzyme-catalysed and that
enzymes are fully specific (``unique enzyme assumption'').  In
reality, enzymes may catalyse several reactions, and reactions may be
catalysed by several enzymes. To consider this in models, we can split
each reaction into ``isoreactions'' (related to different isoenzymes)
and each enzyme into ``isoenzymes'' \co{schlechtes wort! ``enzyme
  subpools''? ueberall aendern} such that each enzyme subpool
catalyses, specifically, one single isoreaction.  Isoreactions have
identical reaction formulae and therefore identical
{\fluxvalue}s. Summing over their reaction balances (with indices $l$
for different isoenzymes), we obtain a joint reaction balance (index
$L$)
\begin{eqnarray}
 [w^{\rm v}_{L} + \Deltar w_{L}] \,v_{L} = \sum_{l \in L} \hul\,u_{l}.
\end{eqnarray}
The isoenzymes can
be replaced by a single enzyme with level $u_{L}=\sum_l u_{l}$ and
{{\enzymeprice}} $h^{u}_{L} = \frac{\sum_{l} \hul\,u_{l}}{\sum_{l}
  u_{l}}$.  

To describe unspecific or multifunctional enzymes, we need to modify  the
flux benefit balance equation. Consider an enzyme (index $l$) that
catalyses several reactions (indices $j \in J(l)$). In the reaction
balance, we sum the point benefits of all  reactions:
\begin{eqnarray}
 \label{eq.multifunctionalenzyme}
 \sum_{j \in J(l)} [\Deltar \wtotj + w^{\rm v}_{j}]\,v_{j} = \hul\, u_{l}.
\end{eqnarray}
This summation has two effects.  First, if all these reactions have
positive {{\enzymebenefit}}s, the {{\costshade}}s for all
multifunctional enzymes will be higher than for a monofunctional
enzyme.  This is plausible: if more substrates compete for the enzyme,
then more of the enzyme will be needed to catalyse all reactions
(which justifies the higher enzyme investment).  Second, there may
also be enzymes that co-catalyse deleterious side reactions.  Such
reactions would normally not occur, but if the overall enzyme benefit
remains positive, they can be active in optimal states, despite their
negative benefit, as an inevitable side effect.

%\subsection{Economic balance equations with unspecific enzymes and isoenzymes}

We have seen that we can satisfy the unique enzyme assumption by
splitting reactions and enzymes into separate ``isoreactions'' and
``isoenzymes'' with a unique mapping between them.  But this
duplication of network elements may cause problems: for example,
several copies of a reaction will have exactly the same kinetics, and
therefore the metabolite elasticity matrix will not have full column
rank.  Thus, alternatively we may keep our reactions and enzymes, with
the non-unique mapping between them. How can we derive the reaction
balance in such models? The elasticity matrix $\Eunu$ will not be
diagonal, and maybe not even quadratic. The benefit-cost condition for
enzyme levels reads
\begin{eqnarray}
\label{eq:BalanceNonUniqueCondition1}
\gvtot\trans \Eunu &=& \huv\trans.
\end{eqnarray}
Let us assume that the 
enzyme {\price} vector $\huv$ is predefined and that we search for a solution $\gvtot$.
For a solution to exist,
$\huv$ must be in the span of ${\Eunu}\trans$, and since $\huv$ can be
freely chosen, this means that $\Eunu$ must have full column
rank. \co{does this mean, if an enzyme catalyses no reaction, it must
  be switched off? or what does it mean precisely?} With the scaled
elasticity matrix $\Escu$, we can rewrite
Eq.~(\ref{eq:BalanceNonUniqueCondition1}) as
\begin{eqnarray}
\gvtot\trans \diag(\vv)\Escu &=& \huv\trans\,\diag(\esymbolv),
\end{eqnarray}
and by multiplying with the pseudoinverse
${\Escu}~^{+} = {\Escu}~\trans(\Escu\,{\Escu}~\trans)\inv$, and
redefining the {fluxburden}s\footnote{Instead of the pseudoinverse,
  we could also choose any matrix of the form
  ${\Escu}~^{+'} = {\Escu}~^{+'} + \mbox{Ker}(\Escu)\,\Amat$, with some
  arbitrary matrix $\Amat$. However, since we assumed that
  $\diag(\esymbolv)\, \huv$ is in the span of $\Escu$, it must be orthogonal
  to $\mbox{Ker}(\Escu)$ and therefore this extra term has no effect.}
as $\acostv = \huv\trans\,\diag(\esymbolv)\,{\Escu}~^{+}\, \diag(\vv)\inv$,
we obtain the well-known equality
\begin{eqnarray}
\gvtot\trans &=& \acostv.
\end{eqnarray}

\subsection{Bounds on the state variables give rise
  to shadow {\gain}s and shadow {\price}s}
\label{sec:inequality constraints}

In metabolic value theory, we assume that $u_{l} \ge 0$, i.e.~that enzyme
levels cannot be negative. Similar constraints may be imposed, for
instance, to keep metabolite concentrations in physiological ranges, to
enforce some basal rate in ATP-consuming maintenance reactions, or to limit
the total enzyme density in compartments or on cellular membranes
\cite{zhvm:11}. \co{another case?: impose dilution, by setting
  $\Nint\,\vv \ge \lambda\,\cintv$} In a general form, these
constraints can be written as linear inequalities
\begin{eqnarray}
\label{eq:hardconstraints1}
\Amat_{\rm v}\, \vv + \Amat_{\rm c}\, \cintv + \Amat_{\rm u}\, \esymbolv \ge \bv, \qquad
\end{eqnarray}
In  enzyme optimisation, active inequalities are associated with 
Lagrange multipliers. To find an optimal state,  we can maximise the Lagrangian
\begin{eqnarray}
\label{eq:hardconstraints2}
{\mathcal L}(\esymbolv) = \ffit(\esymbolv) + \betav\trans \left[\Amat_{\rm v}\, \vvsteady(\esymbolv) 
+  \Amat_{\rm c}\, \cvsteady(\esymbolv) +  \Amat_{\rm u}\, \esymbolv \right]
\end{eqnarray}
with Lagrange multipliers in vectors $\betav$.  In the solution, the
Lagrange multipliers for active lower bounds will be positive , those
for active higher bounds will be negative, and those for inactive
bounds will vanish.  The resulting cost-benefit balance resembles
Eq.~(\ref{eq:fitnessbalanceeq}), but with the  effective  {\gain} and {\price} vectors
$\bvtot^{\rm eff} = \bvtot + \Amat_{\rm v}\trans \betav$,
$\hc^{\rm eff} = \hc - \Amat_{\rm c}\trans \betav$, and
$\hu^{\rm eff} = \hu - \Amat_{\rm u}\trans \betav$. These effective
vectors contain  the actual {\gain}s and
{\price}s, as well as  shadow {\myvalue}s and {\price}s due to 
constraints. If many variables hit their constraints, the effective
{\gain} and {\price} vectors will be less sparse than the original
ones. In practice, if the constraints are upper and lower bounds on
the single variables, a flux that hits a lower (or upper) bound will
have an extra positive (or negative) {\gain}. Likewise, each
metabolite or enzyme level that hits a lower (or upper) bound will
have an extra negative (or positive) {\price}.

\subsection{Constraints on enzyme profiles due to kinetics and steady-state condition}
\label{sec:importancereversible} 

So far, in our optimality problems we assumed that cells can freely
vary their enzyme levels and that any enzyme profile leads to a
feasible steady state. This is not always the case: for certain (not
very realistic) rate laws, there exist enzyme profiles that do not
lead to a steady state. This restricts the region of possible enzyme
profiles from which we can choose during optimisation. Figure
\ref{fig:unidirectional} (a) shows an example: in a metabolic pathway
model with irreversible rate laws, the maximal velocities
$k^{\rm cat}_l\,u_l$ must not decrease along the pathway because
otherwise intermediates might accumulate, thus preventing a steady
state. In this case, enzyme profiles will be restricted to some
feasible region in enzyme space. If the optimal enzyme profile is
located on the boundary of this feasible region,
we need to consider Lagrange multipliers  (shadow
{{\enzymeprice}}s) for the boundary constraints, which then appear as terms
in the economic balance
equations.  If one ignores this fact, paradoxical results may arise.
In the model in Figure \ref{fig:unidirectional}, for example, there
can  be enzymes that catalyse a reaction, but have no control over the reaction flux.
\coout{A reversible mass-action kinetics
  $v=u\,\cdot (k_{+} a- k_{-} b)$, for instance, would be allowed, but
  not the irreversible rate law $v = u\, k_{+}\, a$.}  Consider, for
example, a linear pathway with a flux objective (Figure
\ref{fig:unidirectional} (b) and (c)).  If the first reaction has an  
irreversible rate law (and no allosteric regulation), the downstream
enzymes have no flux control, and accordingly, vanishing  {{\enzymebenefit}}s.
Likewise, if one applies a virtual supply flux, this  would lead to an accumulation of
pathway intermediates, but due to irreversibility this would not
slow down the first reaction and so the supply fluxes would directly
add to the pathway flux; this means that all intermediates have the
same economic potential as the end product, which again amounts to vanishing
{\enzymebenefit}s.  This directly leads to a paradox: since
{{\enzymebenefit}}s and costs must be balanced, all enzyme levels
except for the first must vanish, so there cannot even be any flux. So
where is the mistake?

\co{we did not consider constraints on feasible states!} \co{the logic
  here is not so clear .. rewrite, keeping the necessary shadow values
  in mind! maybe this can be very short! jsut say that there is a
  fallacy, and how it can be fixed // and for the graphics, note that
  the constraints are actually EQUALITY, not inequality constraints!}
When numerically optimising an enzyme profile, we may encounter
candidate profiles that would lead to accumulation or depletion of
intermediates. To allow for a steady state, we need to exclude these
regions from enzyme space by applying constraints
(e.g.~$k^{\rm cat}_{i+1}\, u_{i+i} \ge k^{\rm cat}_{i}\,u_i$). The
resulting optimum may be located on the boundary of the allowed
region, as shown in Figure \ref{fig:unidirectional} (a), and the
constraints on this boundary will be associated with Lagrange
multipliers (``negative shadow {\price}s''), which need to be included
in the reaction balance. There are two important cases in which steady
fluxes require fine-tuned enzyme levels (thus constituting a
``kinetic'' enzyme constraint): (i) if an enzyme is fully
substrate-saturated (and so the flux is independent of the substrate
concentration); (ii) if a reaction is fully irreversible (and so the
flux is independent of the product concentration). These constraints
will affect the economic potentials. In case (i), all economic
potentials upstream of the reaction will vanish. In case (ii), all
economic potentials downstream of the reaction will be identical, so
the potential differences vanish. In both cases, a steady state
requires fine-tuned enzyme levels.  Since models with irreversible
rate laws typically show this problem, and since irreversible rate
laws are not physically justified anyway, they should be avoided in
metabolic value theory. In models with only reversible rate laws, these
problems do not arise: each enzyme will have some positive flux
control, and virtual supply fluxes of downstream metabolites
contribute more strongly to the production objective, so the economic
potentials increase along the pathway.

\begin{figure*}[t!]
 \begin{center}
  \includegraphics[width=15cm]{\psfileskinetic/unidirectional_reaction_in_pathway.eps}
 \end{center}
 \caption{\co{state clearly, here and in
     text, the paradox stems from the non-consideration of lagrange
     multipliers! THIS is the problem with irreversible reactions!}
   The usage of irreversible rate laws in models can lead to
   paradoxical results.  (a) Unbranched pathway with identical
   irreversible rate laws in all reactions. In the model, all enzyme
   levels must be fine-tuned to exactly the same level to enable a
   steady state. Any decrease of enzyme levels would lead to an
   infinite accumulation of the enzymes' substrates. Therefore, for a
   steady state to exist, enzyme profiles with decreasing enzyme
   levels along the pathway must be excluded: the remaining feasible
   enzyme profiles forms a polyhedron in enzyme space. \co{eigentlich
     INCREASE ist genauso schlimm. durchdenken!}  The optimal enzyme
   profile is a boundary optimum (red point) within the feasible
   subset, characterised by negative shadow {{\enzymeprice}}s. If one
   ignores this constraint, one may get to paradoxical results like
   the following.  (b) Simple pathway with a flux objective. If the
   first rate law is irreversible, the downstream enzymes have no flux
   control and cannot provide any benefit. In enzyme-optimal states,
   their levels means that there is no flux.  (c) At the same time,
   due to the irreversible reaction, supply fluxes would directly add
   to the pathway flux (instead of slowing down the upstream
   reactions, as usually).  All intermediates have the same economic
   potential as the end product, which again agrees with the vanishing
   enzyme {\myvalue}s between them.}  \coout{Some of these paradoxical
   effects can be prevented by banning irreversible rate laws.}
  \label{fig:unidirectional}
\end{figure*}

\subsection{Leaky expression and soft bounds on enzyme levels.}
\label{sec:boundaryoptimaavoidedleaky}

\co{is mentioned in appendix; also mention this in CBA optimility, bei
  constraints vs costs} In our optimal states, an inactive reaction is
a reaction with a vanishing flux $v_{l}=0$ and an enzyme level
$u_{l}=0$, hitting its lower bound (positivity constraint).  However,
inactive reactions can also be modelled differently. We assume that
enzyme levels cannot be shut down completely, but that, instead, leaky
enzyme expression leads to a small, positive enzyme level
$\varepsilon$, whose complete suppression would be costly.  In a
model, this is expressed by an extra cost term $h^{\rm leak}(\esymbolv)$,
which rises as the enzyme level becomes very small. For instance, we
may set $h^{\rm leak}(\esymbolv)=\sum_{l} \varepsilon^{2}/u_{l}$ yielding
the gradient $h^{\rm leak}_{u_{l}}=-(\varepsilon/u_{l})^{2}$. The new
fitness function, including this cost term, diverges at
$u_{l} \rightarrow 0$. Instead of a boundary optimum at $u_{l} = 0$,
it has an interior optimum with positive (possibly very small) enzyme
levels. This is an example of objective terms and constraints that
have similar effects and that can replace each other in models. Let us
see the resulting balance equation. From the optimality condition
$\mbox{max} \stackrel{!}{=} \gplus(\esymbolv)-\hminus(\esymbolv)-h^{\rm
  leak}(\esymbolv)$, we obtain the cost-benefit balance
\begin{eqnarray}
 \gplus_{u_{l}}-\hul = h^{\rm leak}_{u_{l}} = - (\varepsilon/u_{l})^{2}.
\end{eqnarray}
The cost on the right approaches zero if $u_{l} \gg \varepsilon$ and is
negative otherwise. The resulting flux benefit balance
\begin{eqnarray}
 [\Deltar \wtotl + \bvdirl]\, v_{l} = \hul\,u_{l} - \varepsilon^{2}/u_{l}
\end{eqnarray}
contains a new cost term, which replaces the Lagrange multiplier that would come
with the hard constraint $u_{l}>0$. For the active enzymes, the
cost term $\hul$ dominates, but for inactive enzymes the stress term
becomes important and prevents smaller enzyme levels.

\subsection{Non-optimal states and economic imbalance}
\label{sec:violationsnonenzymatic}

\co{call the imbalance ``opportunity cost''? (THANKS TO RON!) nur hier
  fuer die erklaerung, nicht allgemein!}  The flux benefit balance
equation (\ref{eq:reactionbalanceeq}) states that cost and benefit of
an active enzyme, in optimal states, must be balanced.  Can we use
similar balance equations to also model non-optimal states?  More
commonly, enzymes will show non-optimal levels directly after a
perturbation, when there has not been enough time for adaptation 8or
also after an enzyme knockdown.  To describe non-optimal states, we
assume that the enzymes satisfy an imbalance
\begin{eqnarray}
 \label{eq:knockdown1}
 [\Deltar \wtotl + \bvdirl]\, v_{l} =  \hudotl^{\rm opt} \neq  \hudotl^{\rm real},
\end{eqnarray}
where $\hudotl^{\rm opt}$ is the optimal {\costshade} that would be in
balance with the economic potentials, and $\hudotl^{\rm real}$ is the
actual point cost of the enzyme.  The mismatch -- the difference
$\hudotl^{\rm opt} - \hudotl^{\rm real}$ between optimal and actual
{\enzymecost} is called \emph{economic stress} \co{wort? uea}
$\fudotl$. It is given by
$\fudotl = \partial \ffit/\partial u_{l} = [\Deltar \wtotl +
\bvdirl]\,v_{l} - \hul\,u_{l}$.  Formally, we can replace the
inequality (\ref{eq:knockdown1}) by a reaction balance
\begin{eqnarray}
 \label{eq:knockdown2}
[\Deltar \wtotl + \bvdirl]\, v_{l} = \hudotl^{\rm real} + \fudotl
\end{eqnarray}
with $\fudotl$ as an extra term (Eq.~(\ref{eq:econForceEquation})
in the article.  The economic stress tells us how strongly the flux
benefit balance is violated.  If the enzyme level is too low, the
economic stress will be positive; if the level is too high, it is
negative.  Thus, the inequality states that a change in enzyme level
-- if it were possible -- would be profitable.  The imbalance equation
can also be used in \enzymevalueform
\begin{eqnarray}
\label{eq:econPressureEquation}
\left[ \Deltar \wtotl + \bvdirl \right] \frac{v_{l}}{u_{l}} &=& \hul + \ful
\end{eqnarray}
with enzyme {\myvalue}, enzyme {\price}), and the enzyme
\stress $\ful = \frac{\partial \ffit}{\partial u_{l}}$, and
in the  \fluxvalueform
\begin{eqnarray}
\label{eq:econPressureEquation2}
 \Deltar \wtotl + \bvdirl &=& \hvl + \fvl
\end{eqnarray}
with {\fluxvalue}, flux {\fluxburden}), and the flux
\stress
$\fvl = \frac{1}{v_{l}}\frac{\partial \ffit}{\partial \ln u_{l}}$.

\subsection{Non-enzymatic reactions}
\label{sec:nonenzymatic}

\myparagraph{\ \\Kinetic models with non-enzymatic reactions and
  dilution} So far, we assumed that all reactions are catalysed by
enzymes and are therefore directly controllable.  In reality, there
are also non-enzymatic reactions, ranging from the fast protonation of
acids to the damage of proteins or DNA by reactive oxygen species.
Even metabolites dilution in growing cells can be described as a
non-enzymatic degradation reaction, with linear kinetics and the cell
growth rate $\lambda$ as the rate constant.  In models with
non-enzymatic reactions, the rules of metabolic value theory seem to be
violated: for example, if a pathway product is diluted, and if this
product acts as a catalyst or contributes directly to cell fitness,
the cells needs to constantly reproduce it. In this case, however, the
economic potential rises along the pathway, but then suddenly drops to
zero. Metabolic value theory would normally exclude such behaviour, and
 to account for non-enzymatic reactions and dilution,
some equations need to
be changed. We
consider the system equations
\begin{eqnarray}
 \label{eq:nonenzymaticequations}
 \md \cintv / \md t = \Nenz\, \vvenz + \Nnon\, \vvnon - \lambda\, \cintv
\end{eqnarray}
with separate terms for enzymatic reactions, non-enzymatic reactions,
and dilution (here dilution fluxes are not included in the flux vector
$\vv$). Accordingly, we obtain the flux vector
$\vv = {\vvenz \choose \vvnon}$, the stoichiometric matrix
$\Nint = (\Nenz | \Nnon)$, and the internal elasticity matrix
$\Eunint = {\Eunint^{\rm enz} \choose \Eunint^{\rm non}}$.  The
Jacobian matrix can be split into
$\Mmat_{\lambda} = \Mmat^{\rm enz} + \Mmat^{\rm non} - \lambda\,
\Imat$, with the terms
$\Mmat^{\rm enz} = {\NR}^{\rm enz}\, \Eunint^{\rm enz}\, \Lmat$ (for
enzymatic reactions), $\Mmat^{\rm non} = \NRnon\, \Eunnon\,\Lmat$ (for
non-enzymatic reactions) and $-\lambda\, \Imat$ (for dilution).
Metabolic control coefficients for such models, as well as their
summation and elasticity theorems, are given in SI
\ref{sec:SIproofMCAwithDilution}.

\myparagraph{{\Summationconnectivitycondition} with dilution} In
models with dilution ($\md \cintv / \md t = \Nint\,\vv + \lambda\,\cintv$),
the {\summationconnectivitycondition} read (proof in section
\ref{sec:demandDilution})
\begin{eqnarray}
 \Kint\trans \,\bvtot 
 &=& \Kint\trans\, \hvv \nonumber \\
 \Lmat\trans\, \hc
 + \lambda\,(\Lmat\, {\Mmat_{\lambda}}\inv)\trans\,\hctot
 &=& (\Eunint\,\Lmat)\trans\, \hvv.
\end{eqnarray}
with the {fluxburden} vector $\hvv = \hu \odots \esymbolv \oslashs \vv$.
The {\summationcondition} remains unchanged. The second equation
contains the extra term
$\lambda\,(\Lmat\,{\Mmat_{\lambda}}\inv)\trans\,\hctot$ with the
proximal concentration {\price}
$\hctot = - {\Eunint}\trans\,\bvtot + \hc$.

\myparagraph{{\Summationconnectivitycondition} with non-enzymatic
  reactions} The \summationconnectivitycondition Eq.~(\ref{eq:fitnessbalance2})
and (\ref{eq:fitnessbalance3}) are only valid if all reactions are
active and enzyme-catalysed.  If reactions are inactive, we can simply
omit them from the model.  Non-enzymatic reactions, in contrast, may
considerably change the shape of enzyme-optimal states. On the one
hand, they may produce valuable compounds ``for free''. On the other
hand, they may degrade valuable metabolites, but cannot be simply
switched off by repressing an enzyme. Instead, the cell can compensate
their effects or may control their fluxes indirectly by changing
enzyme levels -- which may again lead to costs.  Even a single
non-enzymatic reaction can drastically change the enzyme-optimal
states in a model. Our \summationconnectivitycondition should capture this
effect, and we shall now see how these modified conditions look
like. For simplicity, we reorder the reactions (first the enzymatic
reactions, then the non-enzymatic reactions) and write the flux vector
as $\vv = {\vv_{\rm enz} \choose \vv_{\rm non} }$. From the
cost-benefit balance (\ref{eq:fitnessbalanceeq}), we obtain the
following \summationconnectivitycondition for active enzymatic reactions (proof
in section \ref{sec:proofnonenzymatic}):
\begin{eqnarray}
 \label{eq:nonenzymatic2}
 \kv \cdot \bvtot  - \kv_{\rm non} \cdot \gvnon &=& 
 \kv_{\rm enz}\trans (\hudotenz \oslashs  \vv_{\rm enz})\\
 \label{eq:nonenzymatic2conc}
\Lmat\trans\,\hc - (\Eunint\,\Lmat)_{{\rm non}}\trans\, \gvnon &=& 
((\Eunint\,\Lmat)_{{\rm enz}})\trans
 (\hudotenz \oslashs \vv_{\rm enz}).
\end{eqnarray}
In the stationary flux mode $\kv$, the subvector $\kv_{\rm enz}$ is
contains the enzymatic reactions.  The {{\enzymecost}} vector
$\hudotenz = \esymbolv \odots \hu)$ refers to enzymatic reactions, and
$\gvnon = [\Deltar {\wint}^{\rm non} + \bvtotnon]$ refers to
non-enzymatic reactions.  The {\summationcondition}
(\ref{eq:nonenzymatic2}) contains an additional term for active
non-enzymatic reactions.  By splitting
$\kv \cdot \bvtot = \kv_{\rm enz} \cdot \bvtotenz + \kv_{\rm non}
\cdot \bvtotnon$, we can rewrite it as
\begin{eqnarray}
 \label{eq:nonenzymatic2a}
 \kv_{\rm enz}\cdot \bvtotenz 
- \kv_{\rm non}\cdot \Deltar {\wint}^{\rm non} &=& 
 \kv_{\rm enz}\trans (\hudot \oslashs  \vv_{\rm enz}) \nonumber \\
\Rightarrow \kv\cdot {\bvtotenz \choose - \Deltar {\wint}^{\rm non}} &=& 
 \kv_{\rm enz}\trans (\hudot \oslashs  \vv_{\rm enz}). 
\end{eqnarray}
Equations (\ref{eq:nonenzymatic2}) and (\ref{eq:nonenzymatic2a})
differ from the usual {\summationcondition} by an extra term, which
describes the effects of non-enzymatic reactions.  here we consider
two special cases: (i) For any flux variation $\modevector$ consisting
of enzymatic reactions, we obtain the original summation
condition. (ii) If we insert a {\flow} $\vv$ as its own flux variation,
Eq.~(\ref{eq:nonenzymatic2}) yields the balance equation
\begin{eqnarray}
 \label{eq:nonenzymatic2b}
 \sum_{l} \hudotl &=& 
 \vv \cdot \bvtot - \vv_{\rm non}\cdot [\Deltar \wvsymbol_{\rm non} + \bvtotnon]\trans.
\end{eqnarray}
In this equation, the total {{\enzymecost}} is not balanced with the
total flux benefit, but with the {\fluxbenefit} minus the
{\fluxbenefit} caused by non-enzymatic reactions. If this extra
term is positive, it will decrease the {\enzymecost}; if it is
negative, the {\enzymecost} increases.  This formula is also valid for
models of growing cells: the dilution ``reactions'' can be treated as
non-enzymatic reactions and can be included into the vector
$\vv_{\rm non}$.

\coout{ \co{If k is {\futile}: $0= \kv_{\rm enz}\trans (\hudot \oslashs 
  \vv_{\rm enz}) + \kv_{\rm non}\trans
  [\Deltar \wvsymbol_{\rm non} + \bvdir_{\rm non}]$ 
 so $\kv_{\rm enz}\trans (\hudot \oslashs  \vv_{\rm enz}) = - \kv_{\rm
  non}\trans [\Deltar \wvsymbol_{\rm non} + \bvdir_{\rm non}]$}

\co{falls $k_{l}= v_{l}$ for all active reactions in $\kv$ then
$\sum_{l} \hudotl$ all active enz reactions in $\kv$ $=\kv_{\rm
 non}\trans [\Deltar \wvsymbol_{\rm non} + \bvdir_{\rm non}]$}

 \co{ALSO REDO THE FOLLOWING:
   \begin{itemize}[leftmargin=5mm]
\item futile submodes (definition and statements) WIE SONST, ABER TEST ODES NUR AUF ENZYMATISCHEN REAKTIONEN. STATEMENT: ECONOMICAL =>
 NO FUTILE SUBMODES. Umgekehrt unklar
\item Statements about flux cost minimisation
\item {\fluxvalue}s, economic potentials, economic loads
\item \co{STIMMT NICHT UNBEDINGT: FORMELN WO? 
Balance equations: show that flux benefit balance stays
  the same, and that the compound balance changes; explain how
  concentrations and fluxes, loads and potentials become entangled}
 \co{We now consider systems in which only some of the reactions are
  catalysed by enzyme and therefore directly controllable via gene
  expression.} \co{The economic imbalance can also be used in this
  case.} If a reaction shows a metabolic flux in the absence of
 enzyme, its balance reads
\begin{eqnarray}
 \label{eq:nonenzymatic4}
 v_{l} [\Deltar \wtotl + \bvdirl] \neq 0 
\end{eqnarray}
with a ``$>$'' sign for beneficial reactions and a ``$<$'' sign for
futile reactions. In both cases, we can replace the inequality by
\co{rename ``economic imbalance'' in the case of non-enzymatic
  reactions? or explain that it's related to a hypothetical case in
  which the reaction is enzymatic with enzyme level =1.}
\begin{eqnarray}
 \label{eq:nonenzymatic6}
 [\Deltar \wtotl + \bvdirl] \, v_{l}= \fudotl
\end{eqnarray}
with a positive or with a negative economic imbalance. \co{explain both cases verbally}
\item \co{Other stuff (see theorems, appendix, proofs ...)}
\end{itemize}
}
}

\section{Control coefficients for metabolite perturbations}
\label{sec:SIvirtualVariations}

Metabolic control coefficients \cite{Heinrich1996, rede:88} describe how
small, virtual perturbations of a reaction rate will affect the steady state of a metabolic system. Here, instead, I consider
virtual perturbations of metabolite concentrations (namely, their production rates
or their concentrations). I determine  control matrices for such
perturbations, show how they are related to the usual control
matrices, and demonstrate that they can be seen as non-orthogonal
projectors, projecting local, initial perturbations to the resulting
long-term changes in metabolic states.

\myparagraph{Control coefficients for perturbations of virtual supply
  fluxes} We consider a kinetic model with $n_{\rm int}$ internal
metabolites. If there are conserved moieties in the model, we choose a
set of $n_{\rm ind}$ independent metabolites and split the
stoichiometric matrix into $\Nint = \Lmat \, \NR$, with an
$n_{\rm int} \times n_{\rm ind}$ link matrix $\Lmat$ and a reduced
stoichiometric matrix $\NR$, whose and rows correspond to the
independent metabolites. We can write $\NR = \Lmatplus \Nint$, where
the matrix $\Lmatplus$ is obtained from an
$n_{\rm int} \times n_{\rm int}$ identity matrix $\Imat$ by selecting
the rows corresponding to independent metabolites; we note that
$\Lmatplus\,\Lmat = \Imat$. The effects of small, virtual supply
fluxes $\virtphiindm$ (for the independent internal metabolites) on
the steady-state concentrations
$\cint_{i}=\csteady_{i}(\esymbolv,\xv,\virtphiindv)$ and steady-state fluxes
$v_{l}=\vsteady_{l}(\esymbolv,\xv,\virtphiindv)$ are described by the new control
matrices $\Ccmat_{\virtphiindv} = \partial \cintv/\partial \virtphiindv$
and $\Cvmat_{\virtphiindv} =\partial \vv/\partial \virtphiindv$, which
can be computed as follows. In the presence of supply fluxes
$\virtphiindv$, the stationarity condition reads
\begin{eqnarray}
 0 &=& \NR \vv +  \virtphiindv.
\end{eqnarray}
By taking derivative with respect to $\virtphiindv$, we obtain
\begin{eqnarray}
\label{eq:statresp}
 0 &=& \NR \frac{\partial \ratev}{\partial \cintv}\, \frac{\partial \cvsteady}{\partial \virtphiindv} 
+ \Imat = \NR\,\Eunint\,\Lmat\,\Ccind_{\virtphiind} + \Imat,
\end{eqnarray}
where $\ratev(\cintv)$ describes the rate laws,
$\cvsteadyind(\virtphiindv)$ denotes the steady-state concentrations
of independent metabolites, and the control matrix
$\Ccind_{\virtphiind} = \partial \cvsteadyind(\virtphiindv)/ \partial
\virtphiindv$ contains their derivatives. The matrix
$\Mmat = \NR\,\Eunint\,\Lmat$, the Jacobian matrix for the independent
internal metabolites, is usually invertible (except for pathological
cases in which $\Eunint$ is rank-deficient). By solving
Eq.~(\ref{eq:statresp}) for $\Ccind_{\virtphiind}$, we obtain
\begin{eqnarray}
 \Ccind_{\virtphiind} = - \Mmat\inv
\end{eqnarray}
and therefore
\begin{eqnarray}
\label{eq:controlbysupplyproof-1}
 \Ccmat_{\virtphiind} &=& \Lmat\, \Ccind_{\virtphiind} = - \Lmat\,\Mmat\inv  \nonumber \\
 \Cvmat_{\virtphiind} &=& \Eunint\, \Ccmat_{\virtphiind} = - \Eunint\, \Lmat\,\Mmat\inv.
\end{eqnarray}
For convenience, we formally define the control
matrices
\begin{eqnarray}
\label{eq:controlbysupplyproof-3}
 \Ccmat_{\virtphi} &=&  \Ccmat_{\virtphiind}\, \Lmatplus \nonumber \\
 \Cvmat_{\virtphi} &=&  \Cvmat_{\virtphiind}\, \Lmatplus,
\end{eqnarray}
to describe  perturbations of all internal metabolites.
By comparing them  to the usual unscaled metabolic control matrices
\cite{rede:88}
\begin{eqnarray}
 \Ccmat &=& - \Lmat\,\Mmat\inv \NR \nonumber \\
 \Cvmat &=& \Imat - \Eunint\, \Lmat\,\Mmat\inv \NR,
\end{eqnarray}
we obtain  the relationships
\begin{eqnarray}
\label{eq:controlbysupplyproof1}
\Ccmat &=& \Ccmat_{\virtphi}\,\Nint \nonumber \\
\Cvmat &=& \Imat + \Cvmat_{\virtphi}\,\Nint.
\end{eqnarray}
\todo{Furthermore, the new control matrices satisfy the identities
\begin{eqnarray}
\label{eq:controlbysupplyproof-2}
 (-\Nint\,\Eunc)\,\Ccmat_{\virtphiind} &=& \Imat \nonumber \\
 (-\Nint)\,\Cvmat_{\virtphiind} &=& \Imat \nonumber.
\end{eqnarray}}

\myparagraph{Control coefficients for concentration perturbations}
Similarly, we can define control matrices for perturbations of
metabolite concentrations.  We consider a steady state with internal
metabolite concentrations $\cintv^{\rm init}$. After a variation of
the concentrations
$\cintv^{\rm init} \rightarrow \cintv^{\rm init}+\delta \virtgammav$,
the system will arrive at a new steady state with concentrations
$\cintv = \cintv^{\rm init}+\delta \cintv$. In models without moiety
conservation, the perturbation $\delta \virtgammav$ has no long-term
\co{sicher? multi-stability? gilt das auf jeden fall fuer dv
  ungefaehr=0?} effect, so $\delta \cintv=0$. In models with moiety
conservation, the perturbation will lead to a stationary concentration
change $\delta \cintv = \Ccmat_{\virtgamma}\,\delta \virtgammav$.  The
control matrix reads (proof in SI \ref{sec:ProofsimplegammaControl})
\begin{eqnarray}
\label{eq:simplegammaControl}
\Ccmat_{\virtgamma} = \Imat -
\Lmat\,(\NR\,\Eunint\,\Lmat)\inv\,\NR\,\Eunint = \Imat + \Ccmat\,\Eunint.
\end{eqnarray}

For the resulting flux changes, we obtain a similar control matrix
$\Cvmat_{\virtgamma} = \Eunint\,\Ccmat_{\virtgamma}$. From
Eq.~(\ref{eq:simplegammaControl}) and $\Gmat\,\Lmat = 0$, we can see
that $\Ccmat_{\virtgamma} \,\Lmat =0$ and
$\Cvmat_{\virtgamma} \,\Lmat =0$. Therefore, the only way in which
concentration perturbations can affect steady-state concentrations or
fluxes is by changing the conserved moiety concentrations.

\begin{figure*}[t!]
 \begin{center}
  \includegraphics[width=15.5cm]{\psfileskinetic/projectors.eps}
 \end{center}
 \caption{The effect of small perturbations on metabolic states can
   described by linear projections.  Vectors describing the initial
   perturbation in flux or concentration space are projected onto
   ``proper'' (i.e.~constraint-respecting) vectors that describe the
   remaining long-term effects. (a) Flux space. Since the matrix
   $(\Kmat | \Eunint\,\Lmat)$ is invertible, flux space can be split
   into the subspaces Im($\Kmat$) (subspace of stationary flux
   perturbations) and Im($\Eunint\,\Lmat$) (subspace of non-stationary
   flux perturbations, caused by concentration changes of independent
   metabolites). An initial (non-stationary) flux perturbation
   $\delta \vv$ can be projected to these two subspaces by the
   projection matrices $\Cvmat$ and $-\Eunint\,\Ccmat$, 
   yielding the components $\deltapar \vv=\Cvmat\,\delta \vv$ and
   $\deltaimproper \vv=- \Eunint \Ccmat\,\delta \vv$. (b) Similar
   projections exist in concentrations space (for details, see text).}
  \label{fig:projectors}
\end{figure*}


\myparagraph{The control coefficient matrices are projectors in flux
  and concentration space} The responses of metabolic systems to
perturbations can be described geometrically as projections in flux or
concentration space. The initial perturbation vectors are projected to
the resulting steady-state changes, and the projectors are related to
the control matrices (see Figure \ref{fig:projectors}). We assume that
the Jacobian matrix $\Mmat = \NR\,\Eunint\,\Lmat$ is invertible
(i.e.~that the elasticity matrix $\Eunint$ has full row rank). Flux
space can be split into the subspaces
${\mathcal M}_{\rm v\parallel} = \mbox{Span}(\Kint)$ spanned by
stationay flux modes and the linearly independent subspace
${\mathcal M}_{\rm v/} = \mbox{Span}(\Eunint\,\Lmat)$ spanned by
reaction velocity perturbations due to perturbations of independent
metabolites. Using the theorems of metabolic control theory,
\begin{eqnarray}
\label{eq:MCAtheorems}
{ \Cvmat \choose \Ccmat}\,(\Kint, \; \Eunint\, \Lmat ) = 
\left(\begin{array}{cc}
\Kint & 0 \\ 0 &  -\Lmat
\end{array}\right),
\end{eqnarray}
we can easily see that the matrices
$\Projvpar = \Cvmat = \Imat + \Eunint\,\Ccmat$ and
$\Projvimproper = -\Eunint\,\Ccmat$ are (non-orthogonal) projectors onto
these subspaces:
\begin{eqnarray}
\label{eq:projector1}
{ \Projvpar \choose \Projvimproper}\,(\Kint, \; \Eunint\, \Lmat ) = 
\left(\begin{array}{cc}
\Kint & 0 \\ 0 &  \Eunint\, \Lmat
\end{array}\right).
\end{eqnarray}
Since the sum of the two projectors yields an identity matrix $\Imat$,
the two subspaces must span the entire flux space. We can also see this
from the fact that the matrix $(\Kmat,\;\Eunc\,\Lmat)$ is quadratic
and all its columns are linearly independent (unless $\Eunc$ is
rank-deficient). A similar projection exists for concentration space.
\co{nee .. eigentlich will ich im konzentrationsraum einen unterraum SENKRECHT auf G und einen unterraum SENKRECHT auf NR E!} Concentration space can be split into subspaces
${\mathcal M}_{\rm c\parallel} = \mbox{Span}(\Gmat\trans)$, spanned by
the coeffient vectors defining the conserved moiety, and the linearly
independent subspace
${\mathcal M}_{\rm c/} = \mbox{Span}((\NR\,\Eunint)\trans)$.  The
matrices $\Projcpar = {\Ccmat_{\virtgamma}}\trans = [\Imat + \Ccmat\,\Eunint]\trans$ and
$\Projcimproper = -[\Ccmat\,\Eunint]\trans$, are (non-orthogonal)
projectors onto these subspaces: \co{beweis ist ok, einfach
  hinschreiben und ausrechnen.}
\begin{eqnarray}
\label{eq:projector1}
{ \Projcpar \choose \Projcimproper }\,(\Gmat\trans, \; (\NR\,\Eunint)\trans) = 
\left(\begin{array}{cc}
\Gmat\trans & 0 \\ 0 &  (\NR\,\Eunint)\trans
\end{array}\right).
\end{eqnarray}
Again, since the sum of the two projectors yields an identity matrix
$\Imat$, the two subspaces must span the entire flux space, and we can
also see this from the fact that the matrix
$(\Gmat\trans, \; (\NR\,\Eunint)\trans)$ is quadratic and has full
rank (unless $\Eunc$ is rank-deficient).  \co{NOCHMAL UEBERLEGEN! der
  projektor ist nicht die kontrollmatrix, sondern die TRANSPONIERTE
  KONTROLLMATRIX!  Similarly, consider a sudden metabolite change
  $\delta \cintv$.  The permanent concentration change (which accounts
  for the changes of conserved moieties) is given by the projection
  $\deltaimproper \cintv = \Projcimproper\,\delta \cintv$, while the
  projection $\deltapar \cintv = \Projcpar\,\delta \cintv$ describes
  the (moiety-conserving) part of the concentration change that will
  be cancelled.} \co{refer to usage in ME (relationships between
  direct and indirect values); or refer to here from there?}

What can we learn from these projections? First, we can apply
  the projections to (physical) perturbations,  splitting them into proper
  (constraint-preserving) and improper (constraint-violating)
  components. A flux perturbation $\delta \vv$ (e.g.~the immediate
  consequence of an enzyme level change) can be split into
\begin{eqnarray}
  \delta \vv = \underbrace{\Cvmat \,\delta \vv}_{\deltapar \vv}
  + \underbrace{(1-\Cvmat)\,\delta \vv}_{\deltaimproper \vv},
\end{eqnarray}
where $\deltapar \vv$ is stationary, i.e.~$\Nint\,\deltapar \vv=0$.
The projection
$\deltaimproper \vv = \Projvimproper\,\delta \vv$, in contrast,
describes the part of the initial flux change that is cancelled by the
system dynamics. 
Likewise a concentration perturbation $\delta \cv$ can can be split
into
\begin{eqnarray}
  \delta \cv = \underbrace{\Ccmat_{\virtgamma} \,\delta \cv}_{\deltapar \cv}
  + \underbrace{(1-\Ccmat_{\virtgamma})\,\delta \cv}_{\deltaimproper \cv},
\end{eqnarray}
where $\deltapar \cv$ is moiety-preserving,
i.e.~$\Gmat\,\deltapar \cv=0$.  Second, we can apply projections to
direct {\myvalue} vectors. The fitness effect of a (possibly
non-stationary) flux perturbation $\delta \vv$ is given by
$\delta \vv\cdot\gvtot$, where \co{note that wv ist auch av!!}
\begin{eqnarray}
\gvtot\trans &=& {\Ccmat}\trans \,\hc + {\Cvmat}\trans\,\bvtot.
\end{eqnarray}
We can see the two terms as projections of $\bvtot$ and
$\hc$. \co{bessere begruendungen, aus projektoreigenschaften!} Given
that $\Ccmat = -\Lmat(\Nint\,\Eunint\,\Lmat)\inv\,\Nint$, the result
of the first term must be in Im(${\Nint}\trans$), and therefore
orthogonal on all stationary flux vectors. On the contrary, given that
$\Cvmat=\Imat-\Eunint\,\Ccmat$, the second term, must be orthogonal on
Im(${\Nint}\trans$), and therefore in the space of stationary flux
vectors. \co{this can be used to correct wv or av obtained from
  empirical data} If we assume that $\delta \vv$ is a stationary flux
variation, the first term must disappear (no effect of metabolite
costs) and the second term is directly given by
$\delta \vv \cdot \bvtot$, because $\Cvmat$ projects $\delta \vv$ onto
itself. \co{entsprechend fur stoerung $\delta \cv$, mit fitness effect
  $\delta \cv \cdot \wtot$ und
  $\wtot\trans = {\Ccmat}\trans_{\virtgamma} \,\hc +
  {\Cvmat}\trans_{\virtgamma}\,\bvtot.$ und entsprechenden
  projektoreigenschaften!}


==> sec_supplement_cba_kinetic_model_construction.tex <==
\section{Computing enzyme-optimal states}

\subsection{Economical fluxes computed from {{\enzymecost}}s}
\label{sec:fluxesfromenzymecosts} 

\coout{What is the meaning of the two equations? (i) Stationarity (ii)
  Scaling of flux costs to match the predefined flux benefit (in
  linear chain: only one scaling factor is needed! It is NOT
  considered here in any way that u increases with v (in fact, given
  the overall benefit, a higher y leads to a LOWER v! (remember that y
  are ALREADY assumed to stem from an optimal state; this is where
  further smartness comes in.) A solution yields v, this yields Delta
  v.  If one does not fully trust the $y$ or the relative scaling of y
  and bz, then one can still use the relationship $v = u * kcat * ..$
  to formulate constraints vl <= u kcat, to be used when computing
  v. (if the relative scaling between y and bv is unknown, one may
  predefine y, relate v to y and bv, and treat bv as a variable to be
  minimised.}

If a pathway is known to be in a stationary, enzyme-beneficial state,
and if the {\enzymecost}s and the flux directions in the pathway are
known, this is sufficient information to compute all reaction
fluxes  (we require that the predefined flux signs must be realisable by a  steady
  state). No further knowledge about metabolite concentrations or
kinetics is needed!  The fluxes can be computed from the
{\summationcondition} and from stationarity (proof in
\ref{sec:UniquenessProof}).  In some cases, these equations can be
solved analytically. In Box 1, this is shown for two examples, an
unbranched pathway and a branch point.

\begin{figure*}[t!]
\mybox{
\textbf{Box 1: Computing the metabolic fluxes from {\enzymecost}s}\\

\textbf{Example 1: Linear chain of reactions}\\

\includegraphics[width=15cm]{\psfileskinetic/unbranchedflux.eps}

{\small
\co{symbol y falsch ?? use blue2 for blue text; formeln in c schoener
  (oder in caption?)}  (a) Simple linear chain (with external
metabolites A and B and internal metabolite X). (b) In steady state,
the reactions must show the same flux, $v_{1}=v_{2}$. (c)
{\summationcondition} $\hudotone/v_{1}+\hudottwo/v_{2} = b$ with
${\Kint}=(1,1)\trans$ (unitless) and $\bvtot=(0,b)\trans$, i.e.~a
demand for the production of X$_{2}$. The solutions $\vv$ form a
hyperbola with the asymptotic fluxes $\vv=(\hudotone/b, \infty)\trans$
and $\vv= (\infty, \hudottwo/b)\trans$.  (d) Together, the two
conditions determine the flux.  Two example cases with different
numerical values for {{\enzymecost}}s $\hudotl$ (dark and light blue)
are shown. The calculation for a longer pathway is similar: the
{\summationcondition} with the {\flow} $\kv=(1,1,...,1)\trans$ leads to
the sum rule $\sum_{l} \hudotl/v_{l}=b$. Since all reaction fluxes
must be equal, we obtain
the {\flow} $\vv=(\sum_{l} \hudotl)/b\,\cdot (1,1,...,1)\trans$.\\
 %\label{fig:unbranchedflux}
}

  \textbf{Example 2: Metabolic branch point}\\

  \includegraphics[width=15cm]{\psfileskinetic/branchflux.eps}

  {\small
  \co{in
    d and e, use different colour for the two constraints; give the
    constraints names (in the drawing b)} (a) Metabolic branch point
  (with external metabolites A, B, C and internal metabolite X). (b)
  The {\summationcondition} Eq.~(\ref{eq:fitnessbalance2}),
  $\kv\trans \diag(\hudot)\,\vv\inv = \kv \cdot \bvtot$ implies a
  linear relationship (with an offset) between the inverse fluxes
  $v_{1}\inv$ and $v_{2}\inv$. (c) This yields a nonlinear
  relationship between the fluxes themselves (hyperbola function). (d)
  In the branch point model, there are two such relationships
  (projections on the $v_{1}/v_{2}$ and $v_{1}/v_{3}$ planes shown in
  blue, resulting constraint curve shown in \todo{purple}). (e) By
  intersecting this curve with the plane of stationary fluxes (red),
  we obtain a unique {\flow} (black dot). In the example, we assume
  external metabolite {\myvalue}s $w_{\rm A}=0$,
  $w_{\rm B}=w_{\rm C}=1$ and {{\enzymecost}}s
  $\hudot=(1,1,1)\trans$. With the flux variations
  $\modevector^{(1)}=(1,1,0)\trans$ and
  $\modevector^{(2)}=(1,0,1)\trans$ the {\summationcondition}s read
  $1/v_{1}+1/v_{2} = 1$ and $1/v_{1}+1/v_{3} = 1$. By combining them
  with the stationarity condition $v_{1}=v_{2}+v_{3}$, we obtain the
  flux vector $\vv=(3,3/2,3/2)\trans$.}
 }
\end{figure*}

\subsection{Computing metabolic fluxes from enzyme {\costshade}s} 

If the {\summationcondition} and {\connectivitycondition} cannot be
solved analytically, the {\flow} $\vv$ can be numerically computed as
follows (again, we require that the predefined flux signs must be
realisable by a steady state). We first remove all inactive reactions
from the model (those with zero values in $\hudot$). Then we consider
the {\summationcondition} Eq.~(\ref{eq:fitnessbalance2}) in the form
\begin{eqnarray}
\label{eq:fromcoststofluxes}
 {\Kint}\trans \bvtot = {\Kint}\trans \diag(\hudot) \vv\inv, 
\end{eqnarray}
where the vector $\vv\inv$ contains the reciprocal elements of $\vv$.
The {\summationcondition} yields $n_{\rm st}$ linearly independent
equations for $\vv\inv$ (where $n_{\rm st}$ is the number of
independent stationary flux profiles).  From the stationarity
condition, we further obtain $n_{\rm ind}$ linearly independent
equations for $\vv$ (where $n_{\rm ind}$ is the number of independent
metabolites). So we obtain $n_{\rm ind}+n_{\rm st}$ equations in
total. Since the number of columns of the stoichiometric matrix is
given by the rank $n_{\rm ind}$ of the matrix plus the dimension
$n_{\rm st}$ of the right null space, this matches exactly the total
number of reactions. As shown in section \ref{sec:UniquenessProof},
these equations determine the flux vector $\vv$ uniquely.  To compute
the fluxes in practice, we can use one the two following
methods. 
\begin{enumerate}[leftmargin=5mm]
\item \textbf{Iterative projection} \co{check implementation} Our aim
  is to find a {\flow} with predefined flux directions that satisfies the
  {\summationcondition} Eq.~(\ref{eq:fromcoststofluxes}) and the
  stationarity condition $\Nmat \,\vv=0$. To find such a {\flow}, we
  guess an initial flux distribution (e.g.~with fluxes proportional
  to the enzyme levels), and project it to the nullspace of $\Nint$ to
  make it stationary, while enforcing the correct flux signs by
  constraints.  This operation is a quadratic minimisation problem
  with linear constraints. \co{details see matlab file} Next, we
  compute the reciprocal vector $1/\vv$ and project it to the solution
  space of the {\summationcondition} Eq.~(\ref{eq:fromcoststofluxes})
  \co{how?} to make it economical and compliant with the predefined
  enzyme costs.  This is again a quadratic minimisation problem with
  constraints. if we take the reciprocal values again, the resulting
  {\flow} will not be stationary anymore.  To find a {\flow} that satisfies
  both conditions, we iterate the entire procedure until
  convergence. \co{klappt das praktisch? will it converge? possible
    tricks?: (1) when it starts to converge, start to expand 1/v
    functions as (1-v) (in both spaces) (2) use relaxation terms}
\item \textbf{Minimising the mismatch} In a second, alternative
  method, we ensure stationarity by representing our {\flow} $\vv$
  directly as $\vv = {\Kint}\, \hat \vv$ with some vector $\hat \vv$
  of independent fluxes. We insert this expression into
  Eq.~(\ref{eq:fromcoststofluxes}) and  optimise $\hat \vv$
  numerically by minimising the mismatch between the two sides,
while imposing sign constraints on $\vv = {\Kint}\, \hat \vv$. We determine 
\begin{eqnarray}
\label{eq:fromcoststofluxes2}
 \hat \vv = \argmin_{\hat \vv'} \sum_{i} \left(a_{i} - \sum_{l} \frac{A_{il}}{\sum_{j} K_{lj}\, \hat v'_{j}} \right)^{2}
\end{eqnarray}
with the abbreviations $\av={\Kint}\trans\, \bvtot$ and
$\Amat=\Kmat\, \hudot$, \co{is this convex or anything? ich denke
  nicht} and from the solution we obtain our {\flow} $\vv$. As we saw
before, if Eq.~(\ref{eq:fromcoststofluxes2}) with predefined flux
directions has a solution $\vv$, this solution will be unique.  If our
predefined {{\enzymecost}}s are infeasible (i.e.~numerical values
that cannot be realised by any economical metabolic {\flow}s because
positive costs are assigned to pathways that cannot contribute to the
metabolic benefit or because predefined sign pattern implies that
futile submodes are used), there will be no exact solution, and a
mismatch on the right of Eq.~(\ref{eq:fromcoststofluxes2}) will
remain.
\end{enumerate}

\begin{figure*}[t!]
\begin{center}
\parbox{7cm}{(a)\\
  \includegraphics[width=7cm]{\psfileskinetic/modelreconstruction.eps}}\hspace{15mm}
\parbox{6cm}{(b)\\
    \includegraphics[width=5.7cm]{\psfileskinetic/ycm_pmf_model_construction_atp_prod_aerob_glucose_uniform_mu.eps}\\[3mm]
    \includegraphics[width=5.7cm]{\psfileskinetic/ycm_pmf_model_construction_atp_prod_aerob_glucose_uniform_w.eps}
}
\end{center}
\caption{\co{bild is schoen - in paper zeigen?} Constructing metabolic
  models in enzyme-balanced states.  (a) Algorithm for model
  construction. (i) Given the metabolic network, an economical,
  energetically feasible {\flow}  (e.g.~by applying flux cost
  minimisation). (ii) Consistent economic potentials and
  {{\enzymecost}}s (satisfying the reaction balance) and (iii)
  reaction elasticities and economic loads (satisfying the compound
  balance) are computed as described in SI
  \ref{sec:reconstructionbalanced} and in \cite{lieb:14b}. (iv) The rate
  constants are computed from the reaction elasticities.  (v) By checking solutions
  for dynamic
  and economic stability (the second-order conditions), enzyme-optimal states
  were obtained.   (b) Reconstructed chemical potentials (top)
  and economic potentials (bottom), in yeast central metabolism under
  aerobic conditions. Other ways to construct models in optimal
  states, are described in \cite{lieb:14b,nfbd:16,wnfb:18}.}
  \label{fig:reconstruction}
\end{figure*}

\subsection{Construction of models in enzyme-optimal states}
\label{sec:reconstruction}
\label{sec:reconstructionbalanced}

\coout{rolle von load in construction? o model construction: muss man
  wirklich loads samplen, oder geht es effektiv nur um constraints
  beim elastizitaetssamplen?  echtes samplen noetig, oder geht auch
  samplen von elastizitaeten, + automatisches berechnen von load aus
  potential? kann man mit anderen formeln beim potentialsuchen zc
  schon irgendwie einbeziehen?}

\myparagraph{\ \\Constructing kinetic models in enzyme-balanced
  states} Computing optimal enzyme levels in kinetic models can be
difficult, \co{generally, multiple local optima.  note that FCM with
  enzymetic cost can do this, but it is difficult itself} and it is
even more difficult to obtain solutions with plausible metabolite
concentrations and fluxes.  To construct an enzyme-optimal model with
predefined fluxes, we need to adapt the model parameters, which
drastically increases the numerical effort.  Here I propose an
alternative method: in a first phase, we determine a consistent set of
state variables ($v_{l}$, $\cint_{i}$, $\mu_{i}$, $\Escvlci$, $\bvtotl$,
$\hci$, and $\winti$) and then construct a kinetic model that realises
the state (see Figure \ref{fig:reconstruction}). In this construction,
the state variables $v_{l}$ and $\cint_{i}$, the economic potentials
$\wtoti$ and loads $\loadi$, and the {\gain} and {\price} vectors
$\bvtot$ and $\hc$ must satisfy various conditions, including the
cost-benefit balance, {\gain} conditions, absence of futile submodes,
and the economic balance equations.  In a second phase, we solve for
the necessary kinetic constants.

An algorithm for model construction, based on this concept, is shown
in Figure \ref{fig:reconstruction}. The matrices $\Kint$ and $\Lmat$
are defined by the network, and the {\gain} and {\price} vectors
$\bvtot$ and $\hc$ are also assumed to be predefined.  In the
algorithm, the state variables (fluxes, concentrations, economic
potentials, {{\enzymecost}}s, economic loads, and reaction
elasticities) are chosen step by step, each of them in agreement with
the previous ones. The following criteria must be satisfied: $\vv$
must be stationary, energetically feasible, and pervasive, the
elasticities $\Eunint$ must be consistent with $\vv$ and with the
chemical potentials \cite{liuk:10}, the {\enzymecost}s $\hudotl$ must
be positive, and all economic balance equations must be satisfied.
The algorithm works as follows (for details, see SI
\ref{sec:realisekineticmodels}):

\begin{enumerate}[leftmargin=5mm]
\item \textbf{Steady-state phase} In the steady-state phase, we
  compute an economical metabolic {\flow} $\vv$ together with metabolite
  levels $\cint_{i}$, and economic potentials $\wtoti$ satisfying the
  energetic constraints and the flux benefit balance
  $[\Deltar \wtotl + \bvdirl] \,v_l = \hudotl$. In models with a
  production objective (defined by a vector $\wext$), the {\flow} must be
  free of cyclic submodes; such {\flow}s can be found by
  flux cost minimisation.  Once a {\flow} has been found, the flux
  distribution defines linear constraints for feasible logarithmic
  concentrations and economic potentials. Using these constraints, we
  can use sampling or optimisation with heuristical criteria to determine
  a specific solution $\cintv$, i.e.~concentrations
  $\cint_{i}$, standard chemical potentials $\mu^\circ_{i}$, economic
  potentials $\wint$, and {{\enzymecost}}s $\hudot$ that comply with
  the {\flow}, satisfying the thermodynamic constraints and the economic
  reaction balance.
\item \textbf{Kinetic phase} In the kinetic phase, we choose  the
  economic loads and  kinetic constants in our model. Given  the
  previously determined metabolic state, we search for  reaction
  elasticities $\Escint$ and economic loads that satisfy a compound
  balance Eq.~(\ref{eq:metabolitebalanceequation}) of the form
  $0 = {\Escint}~\trans\, \hudot - \loadint$.  To ensure that our
  reaction elasticities are energetically feasible, we parametrise
  them by saturation values $\beta$ as described in \cite{liuk:10}, and  to
  avoid that  enzymes are fully saturated, we limit the saturation values to a
  certain range, e.g. $0\le \beta_{li}<0.9$.  Moreover, to ensure the
   condition $\Lmat\trans \,\hc = \Lmat\trans \,\loadint$, \co{symbol $\loadint$ gut?} we
  choose internal load vectors of the form
  $\loadint = -\hc + \Gmat\trans \pv^{\rm cm}$.  At first, we  try to
  satisfy these equations for the given vector $\hc$.  Due to our
  previous, arbitrary choice of economic potentials, this may not be
 possible, and if this is the case, we replace $\hc$ by a
  deviation vector $\hc+\hc^{\rm mis}$ and minimise the mismatch
  $\hc^{\rm mis}$ by quadratic programming.  From the resulting saturation
  values, we compute  the elasticities and, finally, all kinetic constants
  for a consistent model.
\end{enumerate}

 Any metabolic state with feasible economic potentials
(determined in the steady-state phase) can be reached by an
enzyme-balanced kinetic model (determined in the kinetic phase). This fact 
is an important theoretical insight. We know that kinetic models
with optimised enzyme levels will satisfy all optimality criteria
listed above. However, does the opposite hold as well?  Can any set of state
variables that satisfy these criteria be  realised by
enzyme-optimal metabolic models?  If this is true, we may choose
steady-state variables -- metabolic fluxes, economic potentials, and
so on -- and construct models that realise these variables.  The
construction algorithm for enzyme-balanced models shows that and how
economical flux distributions can be kinetically realised, and how
this is done in practice.

\myparagraph{Constructing enzyme-optimal models} Toprove that a
metabolic {\flow} is enzyme-optimal (and not only enzyme-balanced), we
need to realise it by a kinetic model in an enzyme-optimal state.  The
state of this model must be both dynamically stable (i.e.~the Jacobian
matrix for independent metabolites must be negative definite) and
economically stable (the fitness curvature matrix must be negative
definite). By sampling the elasticities in the kinetic phase, we
obtain an ensemble of enzyme-balanced models realising the same
metabolic state (see \cite{liuk:10}). If one of them satisfies the
second-order conditions, this proves that the {\flow} is enzyme-optimal,
otherwise the question remains open. The first criterion, dynamical
stability, is not guaranteed by our previous construction, we may
require it as an extra criterion when choosing the reaction
elasticities.  The second criterion, negative fitness curvatures, can
be satisfied by choosing a strongly curved {{\investment}} function
$\hminus(\uv)$, giving rise to a strongly negative curvature matrix
${\bf H}_{\rm uu}$; however, assuming large cost curvatures may be
biologically implausible.

\coout{\subsection{Model of yeast central metabolism}
\label{sec:SIyeast}
The network contains 57 reactions and 68 metabolites, 47 of which are
internal. SI???}


==> table_cba_symbols.tex <==
\co{define $\prodrate_{i}$ (net rate of change);  $\prodrate^{+}_{i}$  production rate;  $\prodrate^{-}_{i}$  consumption rate; }

\begin{table*}[h!]
\begin{center}
{\small
\begin{tabular}{lll}
 \cellcolor{cbatablecolor1} Network variables and kinetics &  \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\ \ \\
 $\cint_{i}$ & mM & Internal metabolite concentration\\
 $\cextj$ & mM & External metabolite concentration\\
 $\esymbol_{l}$ & mM & Enzyme concentration \\[2mm]
 $v_{l}$ & mM/s & Reaction rate\\
 $\rate_{l}(\esymbolv,\cv, \cextv) = \esymbol_{l}\,\ratelaw_{l}(\cv, \cextv)$ & mM/s & Rate law \\
 $\ratelaw_{l}(\cv, \cextv) = \rate_{l}/\esymbol_{l}$ & 1/s & Catalytic rate (also called ``apparent $k_{\rm cat}$'')\\[2mm]
 $\intprod_{i}$ & mM/s & Internal metabolite net production rate  \\
 $\extprod_{i}$ & mM/s & External metabolite net production rate  \\[2mm]
 $\lambda$ & 1/s & Cell growth rate or dilution rate  \\
 $\enzdegrate_{l}$ & 1/s & Rate constant for degradation of enzyme $l$ \\ \ \\
\cellcolor{cbatablecolor1}  Flux profiles &  \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\\ \\
 $\Nint, \Next, \Ntot$ & 1 & Stoichiometric matrix (internal $n_{il}$, external $n^{\rm x}_{jl}$, all $n^{\rm tot}_{il}$)\\
$\NR$ & 1 & Reduced stoichiometric matrix \\
 $\Lmat$ & 1 & Link matrix (satisfying $\Lmat\,\NR = \Nint$)\\
 $\Gmat$ & 1 & Left-kernel (conserved moiety) matrix (satisfying $\Gmat\,\Nint=0$)\\
 $\Kint, \Ktot$ & 1 & Right-kernel matrices (satisfying $\Nint\,\Kint=0$, $\Ntot\,\Ktot=0$)\\
 $\vv$ & mM/s & Stationary flux distribution\\
 $\modevector$ & mM/s & Test mode (stationary flux distribution on active region of $\vv$) \\
 $\fbaPolytope$ & & FBA flux polytope: $\Nint\,\vv=0$ and $\vv^{\rm min}\le \vv \le \vv^{\rm max}$\\ 
 $\fbabPolytope$ & & Objective-flux polytope, $\fbaPolytope$ with additional condition  $b = \bvtot \cdot\vv$\\ \ \\
 \cellcolor{cbatablecolor1} Flux cost minimisation & \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\  \ \\
  $\acost(\vv)$   & D& Flux cost function\\
   $\acost(\vv) = \acostvweight \cdot |\vv|$ & D & Linear flux cost function (with predefined cost weights $\acostvlweight$) \\
  $\fluxbene(\vv) = \bvtotweight \cdot \vv$ & D & Flux benefit function (with fixed flux benefit weights $\bvtotweightl$)\\
  $\acostvl = \partial \acost/\partial v_{l}$  & D s/mM &  Flux {\price}\\
  $\apointcostvl = \partial \acost/\ln \partial v_{l} = \acostvl \,v_{l}$  & D & {\Fluxcostshade} \\ \ \\
 \cellcolor{cbatablecolor1} Thermodynamics &  \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\ \ \\
 $\mu_{i}$ & kJ/mol & Chemical potential \\
 $\theta_{l}$ & 1 & Thermodynamic driving force $\theta_{l} = - \Deltar G_{l}/RT = -  \sum_{i} n_{il}\, \mu_{i}/RT$\\
 $\sigma_{l}$ & kJ/(s m$^{3}$) & Entropy production rate per volume $\sigma_{l} = R\,(\theta_{l}\cdot v_{l})$ \\ \ \\
\cellcolor{cbatablecolor1}  Metabolic control &  \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\ \ \\
 $\Eunvlci$ & 1/s & Metabolite elasticity (internal $\Eunvlci=\frac{\partial v_{l}}{\partial \cint_{i}}$, external $\Eunextlj=\frac{\partial v_{l}}{\partial \cext_{j}}$)\\
 $\Eunul$ & 1/s & Enzyme elasticity $\Eunul = \frac{v_{l}}{u_{l}} = \ratelaw_{l}$ \\
 $\Escvlci$ & 1 & Scaled metabolite elasticity 
 (int.~$\Escvlci=\frac{\cint_{i}}{v_{l}}\frac{\partial v_{l}}{\partial \cint_{i}}$, 
 ext.~$\Escextlj=\frac{\cext_{j}}{v_{l}}\frac{\partial v_{l}}{\partial \cext_{j}}$)\\
$\csteady_{i}(\esymbolv,\cextv)$ & mM & Steady-state internal metabolite concentration \\
$\vsteady_{l}(\esymbolv,\cextv)$ & mM/s & Steady-state flux \\
 $\Rc_{im},\Rv_{lm}$ &  & Response coefficient (internal conc.~$i$ and flux $l$) for enzyme $m$.\\
 $\Cc_{im}, \Cv_{lm}$ & 1, s & Control coefficient (internal conc.~$i$ and flux $l$) for reaction $m$.\\
 $\Cc_{\virtphiindi}, \Cv_{\virtphiindi}$ & 1, s &  Control coefficient with respect to independent supply rates (index $i$)\\
 \vspace{-5mm}
\end{tabular}
}
\end{center}
\caption{\co{mention F-polytope and B-polytope? think about names that
    distinguish between oriented and non-oriented!}  Mathematical
  symbols used in kinetic models. The symbol $\Deltar$ denotes
  differences along reactions, defined as
  $\Deltar\,\cextv = {\Ntot}\trans\,\cextv$. $R$ denotes the Boltzmann
  constant.  Reaction rates and enzyme levels are given in units of
  mM/s and mM. Other units (mol/s and mol) could also be used instead.
  Indices denote metabolites ($i$), external metabolites ($j$), and
  reactions ($l$). Note that the sensitivities used in {\MCA}
  (elasticities, response coefficients, control coefficients) are
  given in their unscaled form.}
\label{tab:listofsymbols}
\end{table*}


\begin{table*}[h!]
\begin{center}
{\footnotesize
\begin{tabular}{llll}
 \cellcolor{cbatablecolor1}  Metabolic objective &  \cellcolor{cbatablecolor1} & \cellcolor{cbatablecolor1} (``direct {\myvalue}s'') &  \cellcolor{cbatablecolor1} \\ \ \\
  $\bbenefit^{(v)}(\vv)$ \co{klammern weg?}  & D & Direct flux benefit  function\\
  $\bbenefit^{(\rm ext)}(\extprodv)$   & D & Production benefit  function\\
  $\metcostfun(\cv)$ & D & Metabolite cost  function& \\
  $\hminus(\esymbolv)$     & D & Enzyme cost function \\[2mm]
  $\fluxbene(\vv) = \bbenefit^{(v)}(\vv) + \bbenefit^{(\rm ext)}(\extprodv(\vv))$   & D & Flux benefit function & \co{effective, mediated, proximal?} \\
  $\gplus(\vv,\cv) = \fluxbene(\vv) - \metcostfun(\cv)$ & D & {\Metabolicobjective} & \\[2mm]
  $\bvdirl = \partial \bbenefit^{(v)}/\partial v_{l}$ & D s/mM & Direct {\fluxgain} & \\
  $\bpsij = \partial \bbenefit^{(\rm ext)}/\partial \extprod_{j}$ & D s/mM  & Production {\gain} &  \\
  $\bvtotl = \sum_{j} {\Next}_{lj}\,\bpsij + \bvdirl$ & D s/mM&  Total  {\fluxgain} & \co{also ``proximal''?}\\
  $\Nobj = {\bvtot\trans \choose \Nint}$ &  & Benefit-stoichiometry~matrix & Right-kernel matrix is called $\Kobj$ \\[2mm]
  $\hci = \partial \metcostfun/\partial c_{i}$ & D/mM&  Concentration {\price} & \\
%  $\bsr  = \partial \bbenefit/\partial s_r$ & ? &  Quantity {\gain} &  (if $\bbenefit$ depends on an extra dynamic quantity $s_r$) \\
  $\hctoti  = \hci - \sum_l \Eunvlci \,\bvtotl$ & D/mM & Effective concentration {\price} \co{or ``proximal''?}
&  \\[2mm]
  $\hul = \partial\hminus/\partial u_{l}$ & D & \Enzymeprice                & Direct {\enzymeprice} \\
 $\hvl = \hul \,u_l/v_{l}$ & D s/mM & Flux {\burden}  & $\hvl = \hudotl/v_{l}= \hul/\ratelaw_l$ \\
  $\hvlmin$ & D s/mM & Lowest possible {fluxburden}  &  Lower bound on $\hvl$  \\[2mm]
  \ \\
 \cellcolor{cbatablecolor1} Economic {\myvalue}s &  \cellcolor{cbatablecolor1} & \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\ \ \\

  $\gplus(\esymbolv,\cextv) = \bbenefit(\vvsteady(\esymbolv,\cextv),\cvsteady(\esymbolv,\cextv))$ & D &  {\Metabolicobjective} & $\vvsteady$ and $\cvsteady$  can  depend on $\virtphiindv,\virtgammav,\virtnuv,\virtpsiv$ \\[2mm]
  $\virtgammai$ & mM & Concentration variation & virtual, in  $\gplus(\esymbolv,\cextv,\virtphiindv,\virtgammav)$\\
  $\virtnu_{l}$ & mM/s & Flux variation & virtual, in  $\gplus(\esymbolv,\cextv,\virtphiindv,\virtgammav,\virtnuv)$\\
  $\virtphiindi$ & mM/s & Supply flux (ind.~metab.)& virtual, in  $\gplus(\esymbolv,\cextv,\virtphiindv)$\\[2mm]
  $\gul= \partial\gplus(\vv(\esymbolv)),\cv(\esymbolv)))/\partial u_{l}$ & D/mM &  Enzyme load \co{oder Enzyme {\myvalue}?} & \\
  $\gxj = \partial\gplus/\partial x_{j}$ & D/mM & External metabolite {\myvalue} &\\
  $\gvtotl= \partial\gplus/\partial \virtnu_{l}$ & D s/mM & Flux {\myvalue} or \emph{economic {\stress}} &   $\gul \,u_{l}/v_{l}= \bvtotl + \Deltar \wintl = \bvdirl + \Deltar \wtotl $ \\
%  $\gsr=\partial \gplus/\partial \virtpsi_{r}$ &  &  {\Value} of quantity $s_r$ &\\
  $\gci = \partial \gplus/\partial \virtgamma_{i}$ & D/mM &   Concentration {\myvalue} & $\gci=0$ in models without conserved moieties \\
  $\gphii = \partial \gplus/\partial \virtphiindi$ & D s/mM &  Production {\myvalue}  & (for indep.~metabolites $i$; otherwise 0)
 \ \\ \ \\
 \cellcolor{cbatablecolor1}  Indirect {\myvalue}s &  \cellcolor{cbatablecolor1} & \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\ \ \\
  $\wtoti$ & D/(mM/s) & Economic potential & Int.: $\wint = \Lmat\,\gphi$;  ext.:  $\wextj=\bpsij$  \\
  $\gvindl = \Deltar \wtotl$ & D s/mM & Conversion {\myvalue} \co{also ``flux load''} &   $\Deltar \wtot = {\Ntot}\trans\,\wtot$ \\
  $\loadi$ & D/mM &  Internal metabolite load & $\loadi = \gci-\bci$\\
  $\loadj$ & D/mM &  External metabolite load & $\loadj = \gxj$\\[2mm]
 \ \\
 \cellcolor{cbatablecolor1}  Derivatives of fitness function &  \cellcolor{cbatablecolor1} & \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\ \ \\
  $\ffit(\esymbolv,\cextv) = \gplus(\esymbolv,\cextv) - \hminus(\esymbolv)$ & D & Fitness function &  \\
  $\ful = \partial \ffit/\partial u_{l}$ & D/mM & Enzyme \stress & $\gul-\hul =  [\Deltar \wtotl + \bvdirl]\,\frac{v_{l}}{u_{l}} - \hul$\\
  $\fvl = (\partial \ffit/\partial \ln u_{l})/v_{l}$ & D\;s/mM & Flux \stress &  $\fvl =  \ful\,u_{l}/v_{l} = [\Deltar \wtotl + \bvdirl] - \hvl$\\
  $\fvldev = \gvtotl - \hvlmin$  & D\;s/mM &  Excess flux \stress \co{ist das gut?} &  \\
\ \\
 \cellcolor{cbatablecolor1}  {\Benefitshade} and {\costshade} &  \cellcolor{cbatablecolor1} & \cellcolor{cbatablecolor1} &  \cellcolor{cbatablecolor1} \\ \ \\
 $\ubenel= \partial\gplus(\vv(\esymbolv)),\cv(\esymbolv)))/\partial \ln u_{l}$ & D &  \Enzymebenefit &  $\ubenel=\gul\,u_{l}$\\
 $\vbenel = \bvtotl\,v_{l} = \gvtotl\,v_{l}$ & D & {\Fluxbenefit} & $\vbenel = [\Deltar \wtotl + \bvdirl]\,v_{l}$\\
\todo{$\bbci, \bbxj$}   & D &  \todo{Concentration  {\benefit}} \co{lieber point load?} &  \todo{$\bbci = \loadi\,c_{i}, {\bbj}^{\rm x}= \loadj\,\cextj$}\\[2mm]
% $\bbsr$  & D &  {\Benefit}\, of quantity $s_r$ & $\bbsr = \loads_{s_r}\,s_{r}$\\
 $\hudotl = \partial h/\partial \ln u_{l}$ & D & {\Enzymecost} &  $\hudotl = \hul\,u_{l} $\\
 $\yvcostl = \hvl\,v_{l}$ & D & {\Fluxcostshade} &  $\yvcostl = \hudotl $\\
 $\fudotl = \partial \ffit/\partial \ln u_{l}$ & D & Enzyme {\point} \stress \co{equal to flux point stress} & $\fudotl = \ful\,u_{l} = [\Deltar \wtotl + \bvdirl] \,v_{l} - \hudotl$
\end{tabular}
}
\end{center}
\caption{\co{make sure all economic variables are defined}
  Mathematical symbols for economic variables. Fitness, metabolic
  objectives, and {{\investment}}s are expressed in hypothetical units
  called Darwin (Dw).  For instance, if the fitness of microbes is
  defined as the  logarithmic growth rate, one Dw
  corresponds to an $e$-fold increase of the growth
  rate. ``{\Value}'' and ``{\burden}'' denote marginal benefit and
  marginal cost. The direct {\myvalue}s and {\burden}s are are also called
  ``{\gain}'' and ``{\price}''}
\label{tab:listofsymbols2}
\end{table*}


  \coout{move gamma formula $\partial \gplus/\partial
    \virtgamma_{i} = {\NR\,\Eun \choose \Gmat}\inv{0 \choose \Gmat}$
    to paper/SI?}  \coout{vollstaendige definitionen fuer andere
    groessen, variationen, loads ..} 

